Task-Guided Inverse Reinforcement Learning Under Partial Information

We study the problem of inverse reinforcement learning (IRL), where the learning agent recovers a reward function using expert demonstrations. Most of the existing IRL techniques make the often unrealistic assumption that the agent has access to full information about the environment. We remove this assumption by developing an algorithm for IRL in partially observable Markov decision processes (POMDPs). The algorithm addresses several limitations of existing techniques that do not take the information asymmetry between the expert and the learner into account. First, it adopts causal entropy as the measure of the likelihood of the expert demonstrations as opposed to entropy in most existing IRL techniques, and avoids a common source of algorithmic complexity. Second, it incorporates task specifications expressed in temporal logic into IRL. Such specifications may be interpreted as side information available to the learner a priori in addition to the demonstrations and may reduce the information asymmetry. Nevertheless, the resulting formulation is still nonconvex due to the intrinsic nonconvexity of the so-called forward problem, i.e., computing an optimal policy given a reward function, in POMDPs. We address this nonconvexity through sequential convex programming and introduce several extensions to solve the forward problem in a scalable manner. This scalability allows computing policies that incorporate memory at the expense of added computational cost yet also outperform memoryless policies. We demonstrate that, even with severely limited data, the algorithm learns reward functions and policies that satisfy the task and induce a similar behavior to the expert by leveraging the side information and incorporating memory into the policy.

==> avoid_sim_files/avoid_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.39999999999999963	3.885780586188048e-16
9	-0.39999999999999963	3.885780586188048e-16
10	-0.5	0.0
11	-0.5	0.0
12	-0.5999999999999699	3.008704396734174e-14
13	-0.5999999999999699	3.008704396734174e-14
14	-0.7000000000000268	2.6867397195928788e-14
15	-0.7000000000000268	2.6867397195928788e-14
16	-0.7999999999999993	6.661338147750939e-16
17	-0.7999999999999993	6.661338147750939e-16
18	-0.9000000000000503	5.040412531798211e-14
19	-0.9000000000000503	5.040412531798211e-14
20	-0.9999999999999999	0.0
21	4.216666666666667	15.284623718699379
22	4.1270999999998015	15.315192966136815
23	4.1270999999998015	15.315192966136815
24	4.037533333333222	15.345762213573702
25	4.037533333333222	15.345762213573702
26	3.9479666666667605	15.376331461011167
27	3.9479666666667605	15.376331461011167
28	3.8584000000001804	15.406900708449086
29	3.8584000000001804	15.406900708449086
30	3.7688333333333333	15.437469955886437
31	3.7688333333333333	15.437469955886437
32	3.679266666666489	15.468039203323741
33	7.295933333333473	19.20485867679233
34	7.213599999999688	19.242996519253754
35	7.213599999999688	19.242996519253754
36	7.131266666666994	19.281134364854225
37	7.364600000000338	19.473223671836084
38	7.282733333333232	19.511752232835693
39	7.282733333333232	19.511752232835693
40	7.200866666666679	19.550280797188247
41	7.200866666666679	19.550280797188247
42	7.119000000000095	19.588809364873068
43	7.119000000000095	19.588809364873068
44	7.037133333333032	19.627337935871175
45	8.80379999999965	20.923831999898454
46	8.725466666667044	20.96502734195376
47	8.725466666667044	20.96502734195376
48	8.64713333333313	21.00622269191227
49	9.547133333333008	21.57699125879707
50	9.470600000000012	21.619367604997617
51	9.470600000000012	21.619367604997617
52	9.394066666666994	21.661743961699365
53	9.410733333333662	21.671742080312242
54	9.334233333332973	21.71413928171088
55	9.334233333332973	21.71413928171088
56	9.257733333333713	21.756536493558535
57	9.941066666667068	22.148762949553944
58	9.865933333333	22.191983375283787
59	9.865933333333	22.191983375283787
60	9.790800000000017	22.23520381497126
61	10.92413333333336	22.82091214030526
62	10.851266666667092	22.865371599769453
63	10.851266666667092	22.865371599769453
64	10.77839999999964	22.909831079837016
65	10.861733333332971	22.949735270707162
66	10.789033333333741	22.994279935066917
67	10.789033333333741	22.994279935066917
68	10.716333333332965	23.03882462038547
69	11.032999999999612	23.18577475522424
70	10.960933333333356	23.23063581700308
71	10.960933333333356	23.23063581700308
72	10.88886666666708	23.275496902298222
73	11.888866666667175	23.701709278353185
74	11.818799999999825	23.747497269396394
75	11.818799999999825	23.747497269396394
76	11.748733333333615	23.793285293591598
77	11.848733333333607	23.832764808044498
78	11.77886666666626	23.878639688688377
79	11.77886666666626	23.878639688688377
80	11.70900000000004	23.92451460322601
81	11.842333333333382	23.975867475905833
82	11.77273333333383	24.021856503239526
83	11.77273333333383	24.021856503239526
84	11.703133333333133	24.067845565862527
85	12.836466666666645	24.466227951652893
86	12.769133333333476	24.51311391715803
87	12.769133333333476	24.51311391715803
88	12.701799999999587	24.559999934039283
89	13.051799999999568	24.66981630981423
90	12.985166666666716	24.716953762662012
91	12.985166666666716	24.716953762662012
92	12.918533333333857	24.764091271750107
93	12.985200000000523	24.784134057093507
94	12.918699999999987	24.831318134766764
95	12.918699999999987	24.831318134766764
96	12.852200000000119	24.878502269228065
97	13.435533333333364	25.043402938010484
98	13.370199999999572	25.090975906887362
99	13.370199999999572	25.090975906887362
100	13.304866666666719	25.138548943449695
101	13.90486666666672	25.290725631785246
102	13.840733333333873	25.33866546332328
103	13.840733333333873	25.33866546332328
104	13.776600000000132	25.38660537448865
105	13.876600000000161	25.410124211424577
106	13.812666666666619	25.458122074409353
107	13.812666666666619	25.458122074409353
108	13.748733333332902	25.50612001844912
109	14.448733333332882	25.65665472599395
110	14.386200000000043	25.705032378116428
111	14.386200000000043	25.705032378116428
112	14.323666666667194	25.753410128024633
113	14.75700000000055	25.835050693454203
114	14.695333333333606	25.88364164658597
115	14.695333333333606	25.88364164658597
116	14.633666666666516	25.932232708007042
117	14.85033333333316	25.969453078997194
118	14.789099999999559	26.018144524991246
119	14.789099999999559	26.018144524991246
120	14.727866666666719	26.066836084360155
121	14.994533333333392	26.109142143105935
122	14.933833333333887	26.157951473797816
123	14.933833333333887	26.157951473797816
124	14.873133333333623	26.206760925039955
125	15.473133333333658	26.28966637639658
126	15.413633333333145	26.33871809331002
127	15.413633333333145	26.33871809331002
128	15.35413333333289	26.387769949648483
129	15.53746666666621	26.409675176259963
130	15.478333333333396	26.458794956603334
131	15.478333333333396	26.458794956603334
132	15.419200000000567	26.507914881409196
133	15.719200000000587	26.539932768566192
134	15.660666666667021	26.589157430970193
135	15.660666666667021	26.589157430970193
136	15.60213333333313	26.638382247843754
137	16.23546666666642	26.69256317370438
138	16.178199999999535	26.74198393463005
139	16.178199999999535	26.74198393463005
140	16.120933333333394	26.79140487411781
141	16.370933333333394	26.807767688903112
142	16.31416666666724	26.85725679660666
143	16.31416666666724	26.85725679660666
144	16.257400000000366	26.906746091640493
145	16.42406666666704	26.915783612264363
146	16.36763333333309	26.96531542059622
147	16.36763333333309	26.96531542059622
148	16.311199999999552	27.014847421865518
149	16.827866666666218	27.034548207473936
150	16.772466666666727	27.084196780574835
151	16.772466666666727	27.084196780574835
152	16.71706666666724	27.13384556961199
153	17.067066666667245	27.140396620699214
154	17.012366666667095	27.190111874213535
155	17.012366666667095	27.190111874213535
156	16.957666666666377	27.23982735913603
157	17.140999999999696	27.240841378342417
158	17.086666666666222	27.290587673327067
159	17.086666666666222	27.290587673327067
160	17.032333333333394	27.340334207093658
161	17.39900000000006	27.337441705470813
162	17.345400000000566	27.387241168835867
163	17.345400000000566	27.387241168835867
164	17.291800000000432	27.43704088928008
165	17.725133333333794	27.4258492724579
166	17.67239999999969	27.47569722936968
167	17.67239999999969	27.47569722936968
168	17.619666666666234	27.525545466388635
169	17.769666666666232	27.519579452132454
170	17.7172333333334	27.56944092672601
171	17.7172333333334	27.56944092672601
172	17.664800000000568	27.61930268779442
173	17.9981333333339	27.602021118912745
174	17.946366666667142	27.6519051808775
175	17.946366666667142	27.6519051808775
176	17.894599999999677	27.701789548210385
177	18.211266666666315	27.680600060852445
178	18.160133333332915	27.730497122282483
179	18.160133333332915	27.730497122282483
180	18.10900000000007	27.78039450763793
181	18.37566666666674	27.758861790226373
182	18.32506666666723	27.808763456787357
183	18.32506666666723	27.808763456787357
184	18.274466666667173	27.858665463051125
185	18.657800000000524	27.821955463745986
186	18.607966666666293	27.871853183194833
187	18.607966666666293	27.871853183194833
188	18.55813333333292	27.92175126758525
189	18.874799999999585	27.886384341227885
190	18.825600000000065	27.9362698173297
191	18.825600000000065	27.9362698173297
192	18.776400000000553	27.986155679311814
193	18.92640000000055	27.96765077203822
194	18.877500000000513	28.01752791408783
195	18.877500000000513	28.01752791408783
196	18.828599999999625	28.067405450213037
197	18.995266666666286	28.045355009262376
198	18.946699999999588	28.09522051482501
199	18.946699999999588	28.09522051482501
200	18.898133333333398	28.145086424612444
201	19.081466666666735	28.11908539021509
202	19.033266666667213	28.168935253730954
203	19.033266666667213	28.168935253730954
204	18.985066666667183	28.218785533674744
205	19.18506666666719	28.18839886068139
206	19.137266666666296	28.23822830600816
207	19.137266666666296	28.23822830600816
208	19.08946666666627	28.28805818212938
209	19.289466666666268	28.25559146521044
210	19.242066666666737	28.30539707774583
211	19.242066666666737	28.30539707774583
212	19.194666666667207	28.355203136089
213	19.52800000000055	28.296819420799824
214	19.4812666666672	28.34657726067747
215	19.4812666666672	28.34657726067747
216	19.43453333333297	28.396335575484983
217	19.73453333333295	28.33939226792931
218	19.688399999999625	28.38909929485806
219	19.688399999999625	28.38909929485806
220	19.642266666666746	28.43880682322787
221	19.942266666666747	28.37763861791336
222	19.89673333333387	28.42728728989478
223	19.89673333333387	28.42728728989478
224	19.85120000000055	28.476936490664727
225	20.134533333333895	28.41525331194897
226	20.089566666666283	28.46483996931849
227	20.089566666666283	28.46483996931849
228	20.04459999999964	28.514427181808564
229	20.41126666666631	28.429070914509477
230	20.36703333333342	28.478566967672823
231	20.36703333333342	28.478566967672823
232	20.32280000000053	28.52806361275388
233	20.506133333333864	28.482950029486453
234	20.462266666667222	28.53239707529391
235	20.462266666667222	28.53239707529391
236	20.41839999999963	28.581844728895188
237	20.63506666666629	28.526249846919697
238	20.59163333333299	28.575634959388434
239	20.59163333333299	28.575634959388434
240	20.54820000000009	28.625020700312497
241	20.798200000000094	28.557927272358743
242	20.755266666667193	28.60723566271714
243	20.755266666667193	28.60723566271714
244	20.712333333333888	28.656544707196574
245	20.912333333333894	28.600570295401926
246	20.869799999999643	28.649813634530886
247	20.869799999999643	28.649813634530886
248	20.827266666666336	28.699057647634447
249	20.910599999999675	28.675037128252566
250	20.868233333333432	28.724253066219806
251	20.868233333333432	28.724253066219806
252	20.82586666666719	28.77346968271676
253	21.05920000000052	28.704111935864702
254	21.017300000000557	28.75324533642563
255	21.017300000000557	28.75324533642563
256	20.97539999999965	28.802379441752205
257	21.158733333332975	28.74588324836965
258	21.11719999999968	28.794948703316802
259	21.11719999999968	28.794948703316802
260	21.075666666666763	28.844014882736822
261	21.2090000000001	28.801722847774162
262	21.167733333333842	28.850737348097237
263	21.167733333333842	28.850737348097237
264	21.126466666667216	28.899752585715582
265	21.359800000000572	28.823408957998225
266	21.318999999999644	28.872329296404164
267	21.318999999999644	28.872329296404164
268	21.2781999999997	28.921250401045924
269	21.578199999999686	28.81912220661794
270	21.538000000000093	28.867913953037696
271	21.538000000000093	28.867913953037696
272	21.4978000000005	28.91670650610157
273	21.781133333333837	28.816202919808166
274	21.741500000000563	28.86486597491825
275	21.741500000000563	28.86486597491825
276	21.7018666666663	28.91352987528336
277	21.918533333332967	28.83391157154288
278	21.879333333333033	28.882471724021197
279	21.879333333333033	28.882471724021197
280	21.840133333333426	28.931032750011163
281	22.023466666666753	28.86167578841473
282	21.984633333333818	28.910145748489633
283	21.984633333333818	28.910145748489633
284	21.945800000000553	28.95861660531003
285	22.12913333333389	28.887386023122538
286	22.090666666666294	28.93576263995042
287	22.090666666666294	28.93576263995042
288	22.052199999999715	28.984140177459995
289	22.26886666666641	28.897591895904224
290	22.230833333333422	28.94585380739179
291	22.230833333333422	28.94585380739179
292	22.192800000000446	28.994116670340816
293	22.35946666666708	28.92576862215122
294	22.321766666667234	28.97393971966651
295	22.321766666667234	28.97393971966651
296	22.284066666666277	29.022111790763436
297	22.384066666666268	28.98027190110931
298	22.346566666666412	29.028387971297956
299	22.346566666666412	29.028387971297956


==> avoid_sim_files/avoid_mem1_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=1, N=10}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.39999999999999963	3.885780586188048e-16
9	-0.39999999999999963	3.885780586188048e-16
10	-0.5	0.0
11	-0.5	0.0
12	-0.5999999999999699	3.008704396734174e-14
13	-0.5999999999999699	3.008704396734174e-14
14	-0.7000000000000268	2.6867397195928788e-14
15	-0.7000000000000268	2.6867397195928788e-14
16	-0.7999999999999993	6.661338147750939e-16
17	-0.7999999999999993	6.661338147750939e-16
18	-0.9000000000000503	5.040412531798211e-14
19	-0.9000000000000503	5.040412531798211e-14
20	-0.9999999999999999	0.0
21	4.816666666666666	16.031210878228386
22	4.728299999999797	16.063273299984356
23	4.728299999999797	16.063273299984356
24	4.639933333333165	16.095335721740945
25	4.639933333333165	16.095335721740945
26	4.551566666666829	16.12739814349742
27	4.551566666666829	16.12739814349742
28	4.463200000000186	16.159460565253866
29	4.463200000000186	16.159460565253866
30	4.374833333333333	16.191522987010206
31	4.374833333333333	16.191522987010206
32	4.286466666666483	16.2235854087666
33	8.053133333333546	19.82436792222083
34	7.972299999999685	19.86372831847039
35	7.972299999999685	19.86372831847039
36	7.8914666666670215	19.903088717974214
37	8.158133333333696	20.105381879376502
38	8.077833333333173	20.145154222266154
39	8.077833333333173	20.145154222266154
40	7.997533333333357	20.18492656866016
41	7.997533333333357	20.18492656866016
42	7.917233333333519	20.224698918538657
43	7.917233333333519	20.224698918538657
44	7.836933333333026	20.264471271881504
45	9.520266666666323	21.40539283908461
46	9.443333333333712	21.447516768977806
47	9.443333333333712	21.447516768977806
48	9.366399999999729	21.489640706784023
49	9.99973333333303	21.86700954853142
50	9.92406666666668	21.909916494490684
51	9.92406666666668	21.909916494490684
52	9.848400000000325	21.952823450298844
53	9.848400000000325	21.952823450298844
54	9.77273333333298	21.99573041589865
55	9.77273333333298	21.99573041589865
56	9.697066666667048	22.038637391231816
57	10.463733333333737	22.45628920211232
58	10.389599999999692	22.50007581853896
59	10.389599999999692	22.50007581853896
60	10.315466666666687	22.543862448914496
61	11.282133333333363	23.01915262230344
62	11.209933333333732	23.0639488089578
63	11.209933333333732	23.0639488089578
64	11.137733333333056	23.108745015590216
65	11.137733333333056	23.108745015590216
66	11.06553333333368	23.153541242083826
67	11.06553333333368	23.153541242083826
68	10.993333333333004	23.198337488324555
69	11.359999999999658	23.362505002674638
70	11.28853333333336	23.40765633681048
71	11.28853333333336	23.40765633681048
72	11.217066666667058	23.452807693938976
73	12.217066666667122	23.862105007637695
74	12.147599999999919	23.908151209158266
75	12.147599999999919	23.908151209158266
76	12.078133333333524	23.95419744391766
77	12.144800000000178	23.97947830180409
78	12.075466666666333	24.025580494871107
79	12.075466666666333	24.025580494871107
80	12.006133333333384	24.071682721590335
81	12.172800000000052	24.133298299789875
82	12.103800000000431	24.179538296391268
83	12.103800000000431	24.179538296391268
84	12.01813333333325	24.25412441590588
85	13.101466666666765	24.585557776512815
86	13.034633333333389	24.632590143931687
87	13.034633333333389	24.632590143931687
88	12.967799999999631	24.679622697548474
89	13.18446666666629	24.745587863608495
90	13.118066666666733	24.79277247362422
91	13.118066666666733	24.79277247362422
92	13.051666666667169	24.839957270941774
93	13.135000000000506	24.86445766551161
94	13.068766666666747	24.911699817800624
95	13.068766666666747	24.911699817800624
96	13.002533333333403	24.958942156714723
97	13.935866666666643	25.209382253086737
98	13.871499999999617	25.2572203092502
99	13.871499999999617	25.2572203092502
100	13.807133333333399	25.3050585677162
101	14.42380000000007	25.44805651177867
102	14.360666666667187	25.496244551349882
103	14.360666666667187	25.496244551349882
104	14.297533333333515	25.544432803429196
105	14.39753333333354	25.565768922177877
106	14.334599999999933	25.614010804765655
107	14.334599999999933	25.614010804765655
108	14.271666666666281	25.662252899714748
109	14.788333333332949	25.764126685934457
110	14.726433333333395	25.812630589414358
111	14.726433333333395	25.812630589414358
112	14.66453333333384	25.861134715673828
113	15.197866666667192	25.953131001522607
114	15.137033333333587	26.001880672986605
115	15.137033333333587	26.001880672986605
116	15.07619999999989	26.05063057893213
117	15.159533333333213	26.063685639516684
118	15.098866666666286	26.11247183592961
119	15.098866666666286	26.11247183592961
120	15.038200000000073	26.1612582666308
121	15.288200000000069	26.197897512840928
122	15.22803333333385	26.246788580679635
123	15.22803333333385	26.246788580679635
124	15.167866666666908	26.295679888190957
125	15.917866666666972	26.38841565502196
126	15.859199999999847	26.437588178450504
127	15.859199999999847	26.437588178450504
128	15.800533333332947	26.48676096434281
129	16.083866666666264	26.5151766550569
130	16.02576666666674	26.564443392353283
131	16.02576666666674	26.564443392353283
132	15.967666666667217	26.613710399382388
133	16.15100000000055	26.629829621434993
134	16.09326666666699	26.679153809585756
135	16.09326666666699	26.679153809585756
136	16.03553333333316	26.7284782716034
137	16.51886666666647	26.76322584036178
138	16.462099999999598	26.812686927211466
139	16.462099999999598	26.812686927211466
140	16.405333333333413	26.86214830492085
141	16.63866666666675	26.874983625834975
142	16.582366666667227	26.924504063502035
143	16.582366666667227	26.924504063502035
144	16.52606666666702	26.974024799095798
145	16.809400000000366	26.98591543083165
146	16.753666666666483	27.035501596151867
147	16.753666666666483	27.035501596151867
148	16.697933333332948	27.085088069431926
149	17.164599999999588	27.096607662952575
150	17.10980000000008	27.146287111868077
151	17.10980000000008	27.146287111868077
152	17.05500000000057	27.195966888493288
153	17.42166666666725	27.198146454410335
154	17.367600000000422	27.247886711449414
155	17.367600000000422	27.247886711449414
156	17.313533333333098	27.29762731170744
157	17.530199999999756	27.295866255289766
158	17.476566666666265	27.345637449976344
159	17.476566666666265	27.345637449976344
160	17.42293333333342	27.395408996075055
161	17.672933333333425	27.390408310128713
162	17.619800000000584	27.440210178252546
163	17.619800000000584	27.440210178252546
164	17.566666666667093	27.490012408549486
165	17.983333333333785	27.47523033974859
166	17.931033333333094	27.52507136410196
167	17.931033333333094	27.52507136410196
168	17.87873333333295	27.574912772220245
169	18.07873333333294	27.564911047602358
170	18.026833333333432	27.614766158203015
171	18.026833333333432	27.614766158203015
172	17.974933333333922	27.66462166128824
173	18.208266666667257	27.650350419639647
174	18.156833333333793	27.700217567838106
175	18.156833333333793	27.700217567838106
176	18.105399999999754	27.750085120109908
177	18.388733333333064	27.729176326188913
178	18.337866666666287	27.77905180975178
179	18.337866666666287	27.77905180975178
180	18.287000000000102	27.828927713202866
181	18.587000000000103	27.80264407689808
182	18.536733333333917	27.852521082699322
183	18.536733333333917	27.852521082699322
184	18.48646666666714	27.90239852621152
185	18.75313333333381	27.875436322723814
186	18.703399999999743	27.925308505129586
187	18.703399999999743	27.925308505129586
188	18.653666666666297	27.975181141306063
189	19.103666666666292	27.92239172937851
190	19.054833333333434	27.972241895116092
191	19.054833333333434	27.972241895116092
192	19.006000000000576	28.022092546179778
193	19.172666666667247	28.00014094408967
194	19.124166666667136	28.04997931025185
195	19.124166666667136	28.04997931025185
196	19.075666666666407	28.099818170625902
197	19.258999999999737	28.073921926466465
198	19.210866666666302	28.12374445047373
199	19.210866666666302	28.12374445047373
200	19.16273333333344	28.173567479623664
201	19.429400000000104	28.132875234737615
202	19.381800000000563	28.18266917971647
203	19.381800000000563	28.18266917971647
204	19.33420000000046	28.232463649022357
205	19.58420000000047	28.191175989896667
206	19.537099999999754	28.240937784063544
207	19.537099999999754	28.240937784063544
208	19.489999999999654	28.290700120946788
209	19.706666666666322	28.252394038185813
210	19.66000000000011	28.302123830789164
211	19.66000000000011	28.302123830789164
212	19.613333333333895	28.351854181967745
213	19.796666666667228	28.317529357076467
214	19.75036666666714	28.367229095070616
215	19.75036666666714	28.367229095070616
216	19.70406666666642	28.416929404768002
217	20.05406666666641	28.346896305043618
218	20.008466666666326	28.396529746588552
219	20.008466666666326	28.396529746588552
220	19.962866666666773	28.44616379143095
221	20.196200000000108	28.396251845856575
222	20.151066666667216	28.4458357619452
223	20.151066666667216	28.4458357619452
224	20.105933333333795	28.49542030096861
225	20.322600000000467	28.44660722429569
226	20.277899999999747	28.496141053190293
227	20.277899999999747	28.496141053190293
228	20.23319999999967	28.545675523507157
229	20.366533333332995	28.514364099208
230	20.322100000000102	28.5638655458842
231	20.322100000000102	28.5638655458842
232	20.27766666666721	28.613367643268813
233	20.47766666666721	28.564553930040987
234	20.4336333333338	28.61400319422097
235	20.4336333333338	28.61400319422097
236	20.38959999999975	28.66345312716744
237	20.622933333333076	28.603915012847963
238	20.579366666666335	28.653298779237318
239	20.579366666666335	28.653298779237318
240	20.5358000000001	28.702683237402812
241	20.7858000000001	28.635880028849325
242	20.74273333333386	28.685188289351554
243	20.74273333333386	28.685188289351554
244	20.699666666667124	28.73449726760871
245	21.049666666667143	28.63597504111836
246	21.007299999999738	28.685168003284424
247	21.007299999999738	28.685168003284424
248	20.964933333333022	28.734361723592144
249	21.16493333333302	28.675382653574268
250	21.12296666666677	28.724505609883273
251	21.12296666666677	28.724505609883273
252	21.08100000000052	28.773629344708368
253	21.331000000000525	28.697016319935916
254	21.289533333333814	28.74604640263081
255	21.289533333333814	28.74604640263081
256	21.24806666666641	28.79507729217312
257	21.46473333333307	28.7260979412258
258	21.423699999999695	28.77504326628636
259	21.423699999999695	28.77504326628636
260	21.382666666666772	28.823989422393236
261	21.599333333333437	28.752558139329874
262	21.55873333333384	28.801414497593996
263	21.55873333333384	28.801414497593996
264	21.518133333333815	28.850271711872974
265	21.834800000000484	28.741661091407227
266	21.79483333333307	28.790379121717287
267	21.79483333333307	28.790379121717287
268	21.75486666666638	28.839098049619157
269	21.95486666666637	28.767892339358205
270	21.9153000000001	28.816519034111852
271	21.9153000000001	28.816519034111852
272	21.875733333333827	28.865146650049578
273	22.075733333333808	28.791776565463483
274	22.036566666667134	28.84030824290136
275	22.036566666667134	28.84030824290136
276	21.99739999999973	28.888840865866424
277	22.214066666666394	28.806931610213976
278	22.17533333333306	28.855356028916905
279	22.17533333333306	28.855356028916905
280	22.136600000000087	28.90378142112241
281	22.253266666666764	28.858559030708403
282	22.214766666667124	28.906924751903322
283	22.214766666667124	28.906924751903322
284	22.17626666666713	28.955291457616866
285	22.426266666667125	28.855818651741835
286	22.3882666666664	28.90405200536538
287	22.3882666666664	28.90405200536538
288	22.35026666666644	28.9522863794129
289	22.700266666666458	28.807762841443957
290	22.662966666666758	28.855800431320922
291	22.662966666666758	28.855800431320922
292	22.625666666667065	28.90383909717794
293	22.759000000000377	28.84707886424557
294	22.72196666666713	28.89504018798994
295	22.72196666666713	28.89504018798994
296	22.684933333333056	28.94300260273994
297	22.90159999999971	28.848575657040637
298	22.864999999999817	28.896407994766136
299	22.864999999999817	28.896407994766136


==> avoid_sim_files/avoid_mem1_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.39999999999999963	3.885780586188048e-16
9	-0.39999999999999963	3.885780586188048e-16
10	-0.5	0.0
11	-0.5	0.0
12	-0.5999999999999699	3.008704396734174e-14
13	-0.5999999999999699	3.008704396734174e-14
14	-0.716666666666688	0.9127187713395325
15	-0.716666666666688	0.9127187713395325
16	-0.8333333333333375	1.2905640455070582
17	-0.8333333333333375	1.2905640455070582
18	-0.9333333333333836	1.2905640455070575
19	-0.9333333333333836	1.2905640455070575
20	-1.0333333333333332	1.2905640455070582
21	-1.0333333333333332	1.2905640455070582
22	-1.1666666666666077	1.8245242911205517
23	-1.1666666666666077	1.8245242911205517
24	-1.2666666666666015	1.8245242911205521
25	-1.2666666666666015	1.8245242911205521
26	-1.3666666666667384	1.824524291120547
27	-1.3666666666667384	1.824524291120547
28	-1.483333333333361	2.0395397084200897
29	-1.483333333333361	2.0395397084200897
30	-1.616666666666667	2.4124100443793086
31	-1.616666666666667	2.4124100443793086
32	-1.71666666666669	2.4124100443793073
33	-1.71666666666669	2.4124100443793073
34	-1.816666666666569	2.412410044379313
35	-1.816666666666569	2.412410044379313
36	-1.9166666666667689	2.4124100443793037
37	-1.9166666666667689	2.4124100443793037
38	-2.016666666666595	2.412410044379312
39	-2.016666666666595	2.412410044379312
40	-2.166666666666667	2.88193607763171
41	-2.2	3.409789827345278
42	-2.333333333333447	4.275381724348123
43	-2.333333333333447	4.275381724348123
44	-2.4333333333332097	4.275381724348134
45	-2.4333333333332097	4.275381724348134
46	-2.550000000000126	4.370831347314445
47	-2.550000000000126	4.370831347314445
48	-2.6499999999998582	4.37083134731446
49	-2.6499999999998582	4.37083134731446
50	-2.7500000000000004	4.370831347314452
51	-2.7500000000000004	4.370831347314452
52	-2.900000000000163	4.645069070171564
53	-2.900000000000163	4.645069070171564
54	-2.9999999999999565	4.6450690701715756
55	-2.9999999999999565	4.6450690701715756
56	-3.10000000000002	4.645069070171572
57	-3.10000000000002	4.645069070171572
58	-3.1999999999998185	4.645069070171584
59	-3.1999999999998185	4.645069070171584
60	-3.3000000000000007	4.645069070171574
61	-3.3000000000000007	4.645069070171574
62	-3.4166666666668624	4.732834480754702
63	-3.4166666666668624	4.732834480754702
64	-3.5500000000000704	4.903485155138638
65	-3.5500000000000704	4.903485155138638
66	-3.6499999999999098	4.903485155138633
67	-3.666666666666572	4.9865374314805315
68	-3.799999999999787	5.307855813163431
69	-3.799999999999787	5.307855813163431
70	-3.933333333333333	5.460056979759873
71	-3.933333333333333	5.460056979759873
72	-4.050000000000225	5.5345129264762525
73	-4.050000000000225	5.5345129264762525
74	-4.150000000000175	5.534512926476254
75	-4.150000000000175	5.534512926476254
76	-4.24999999999981	5.534512926476271
77	-4.24999999999981	5.534512926476271
78	-4.349999999999764	5.534512926476275
79	-4.349999999999764	5.534512926476275
80	-4.466666666666668	5.60793089195031
81	-4.466666666666668	5.60793089195031
82	-4.583333333333577	5.680351123732425
83	-4.583333333333577	5.680351123732425
84	-4.73333333333357	5.891990797307522
85	-4.73333333333357	5.891990797307522
86	-4.8666666666664185	6.028727523744708
87	-4.8666666666664185	6.028727523744708
88	-4.983333333333078	6.095877477625753
89	-4.983333333333078	6.095877477625753
90	-5.083333333333333	6.095877477625731
91	-5.083333333333333	6.095877477625731
92	-5.200000000000259	6.162250671088736
93	-5.200000000000259	6.162250671088736
94	-5.300000000000284	6.162250671088732
95	-5.300000000000284	6.162250671088732
96	-5.399999999999706	6.16225067108877
97	-5.399999999999706	6.16225067108877
98	-5.516666666666411	6.227871939024338
99	-5.516666666666411	6.227871939024338
100	-5.616666666666666	6.227871939024316
101	-5.616666666666666	6.227871939024316
102	-5.716666666666856	6.227871939024301
103	-5.716666666666856	6.227871939024301
104	-5.833333333333663	6.292764804828801
105	-5.833333333333663	6.292764804828801
106	-5.933333333332996	6.292764804828854
107	-5.933333333332996	6.292764804828854
108	-6.03333333333324	6.292764804828831
109	-6.03333333333324	6.292764804828831
110	-6.15	6.356951575506441
111	-6.15	6.356951575506441
112	-6.250000000000036	6.356951575506439
113	-6.250000000000036	6.356951575506439
114	-6.36666666666703	6.420453428085771
115	-6.36666666666703	6.420453428085771
116	-6.499999999999628	6.54548190229996
117	-6.499999999999628	6.54548190229996
118	-6.600000000000049	6.545481902299937
119	-6.600000000000049	6.545481902299937
120	-6.699999999999998	6.545481902299943
121	-6.699999999999998	6.545481902299943
122	-6.81666666666657	6.607045902334344
123	-6.81666666666657	6.607045902334344
124	-6.916666666667057	6.607045902334312
125	-6.916666666667057	6.607045902334312
126	-7.033333333332935	6.667999866693244
127	-7.033333333332935	6.667999866693244
128	-7.1333333333334785	6.6679998666932025
129	-7.1333333333334785	6.6679998666932025
130	-7.25	6.728360374811483
131	-7.25	6.728360374811483
132	-7.366666666666475	6.788143257834933
133	-7.366666666666475	6.788143257834933
134	-7.500000000000416	6.906036007242794
135	-7.500000000000416	6.906036007242794
136	-7.599999999999578	6.906036007242629
137	-7.599999999999578	6.906036007242629
138	-7.700000000000242	6.906036007242815
139	-7.716666666666913	6.964174195281136
140	-7.85	7.195658413237989
141	-7.85	7.195658413237989
142	-7.983333333333048	7.30659899603724
143	-7.983333333333048	7.30659899603724
144	-8.083333333333773	7.306598996037183
145	-8.100000000000438	7.36138573911174
146	-8.216666666666224	7.527265255205525
147	-8.216666666666224	7.527265255205525
148	-8.316666666666983	7.527265255205523
149	-8.316666666666983	7.527265255205523
150	-8.416666666666666	7.52726525520555
151	-8.416666666666666	7.52726525520555
152	-8.566666666666313	7.685411866358129
153	-8.566666666666313	7.685411866358129
154	-8.666666666667126	7.685411866358066
155	-8.666666666667126	7.685411866358066
156	-8.766666666666204	7.685411866358142
157	-8.766666666666204	7.685411866358142
158	-8.866666666667058	7.685411866358071
159	-8.866666666667058	7.685411866358071
160	-8.983333333333333	7.73733732552046
161	-8.983333333333333	7.73733732552046
162	-9.08333333333291	7.737337325520085
163	-9.08333333333291	7.737337325520085
164	-9.200000000000477	7.788880963698561
165	-9.216666666667143	7.840050311629862
166	-9.333333333332853	7.995762766754942
167	-9.333333333332853	7.995762766754942
168	-9.43333333333379	7.9957627667548445
169	-9.43333333333379	7.9957627667548445
170	-9.533333333333333	7.995762766754887
171	-9.533333333333333	7.995762766754887
172	-9.633333333332855	7.995762766754942
173	-9.633333333332855	7.995762766754942
174	-9.766666666667158	8.094991592885474
175	-9.766666666667158	8.094991592885474
176	-9.866666666666172	8.094991592885581
177	-9.866666666666172	8.094991592885581
178	-9.966666666667177	8.094991592885474
179	-9.966666666667177	8.094991592885474
180	-10.066666666666665	8.09499159288552
181	-10.066666666666665	8.09499159288552
182	-10.166666666666137	8.094991592885584
183	-10.166666666666137	8.094991592885584
184	-10.300000000000505	8.192883090422628
185	-10.300000000000505	8.192883090422628
186	-10.416666666666156	8.241342258529649
187	-10.416666666666156	8.241342258529649
188	-10.533333333333893	8.289484637512373
189	-10.533333333333893	8.289484637512373
190	-10.649999999999999	8.337315715104818
191	-10.649999999999999	8.337315715104818
192	-10.749999999999421	8.33731571510489
193	-10.766666666666087	8.384840818737095
194	-10.88333333333385	8.53032173419553
195	-10.88333333333385	8.53032173419553
196	-10.983333333332824	8.530321734195631
197	-10.983333333332824	8.530321734195631
198	-11.08333333333393	8.530321734195518
199	-11.08333333333393	8.530321734195518
200	-11.183333333333332	8.530321734195594
201	-11.199999999999998	8.576712656956728
202	-11.316666666666054	8.718928960727952
203	-11.316666666666054	8.718928960727952
204	-11.416666666667028	8.718928960727865
205	-11.416666666667028	8.718928960727865
206	-11.516666666666334	8.718928960727931
207	-11.516666666666334	8.718928960727931
208	-11.633333333333969	8.764258224300438
209	-11.633333333333969	8.764258224300438
210	-11.749999999999998	8.809322713277487
211	-11.749999999999998	8.809322713277487
212	-11.849999999999348	8.80932271327757
213	-11.849999999999348	8.80932271327757
214	-11.966666666666885	8.854126470496833
215	-11.966666666666885	8.854126470496833
216	-12.083333333333147	8.898673434219804
217	-12.083333333333147	8.898673434219804
218	-12.18333333333401	8.898673434220015
219	-12.18333333333401	8.898673434220015
220	-12.316666666666665	8.987012233712115
221	-12.316666666666665	8.987012233712115
222	-12.416666666665973	8.987012233712193
223	-12.433333333332639	9.030811456096263
224	-12.566666666666734	9.117687328605967
225	-12.566666666666734	9.117687328605967
226	-12.666666666666618	9.11768732860598
227	-12.666666666666618	9.11768732860598
228	-12.766666666667374	9.1176873286059
229	-12.766666666667374	9.1176873286059
230	-12.866666666666664	9.117687328605976
231	-12.866666666666664	9.117687328605976
232	-12.983333333332608	9.160770831225193
233	-12.983333333332608	9.160770831225193
234	-13.09999999999994	9.203622475235841
235	-13.09999999999994	9.203622475235841
236	-13.233333333333418	9.288643005783474
237	-13.233333333333418	9.288643005783474
238	-13.36666666666741	9.372773809758034
239	-13.36666666666741	9.372773809758034
240	-13.499999999999998	9.456038635002853
241	-13.499999999999998	9.456038635002853
242	-13.616666666665905	9.497353432521095
243	-13.616666666665905	9.497353432521095
244	-13.716666666666482	9.497353432521031
245	-13.733333333333146	9.538460159911834
246	-13.86666666666687	9.706298069924692
247	-13.86666666666687	9.706298069924692
248	-13.96666666666744	9.706298069924628
249	-13.96666666666744	9.706298069924628
250	-14.08333333333333	9.746438095814842
251	-14.08333333333333	9.746438095814842
252	-14.216666666665878	9.826141437795108
253	-14.216666666665878	9.826141437795108
254	-14.349999999999726	9.905091283442747
255	-14.349999999999726	9.905091283442747
256	-14.483333333333622	9.983305509142884
257	-14.483333333333622	9.983305509142884
258	-14.600000000000804	10.022142152920091
259	-14.600000000000804	10.022142152920091
260	-14.733333333333333	10.099284903177677
261	-14.733333333333333	10.099284903177677
262	-14.833333333332513	10.09928490317761
263	-14.849999999999177	10.137595046821291
264	-14.949999999999614	10.137595046821243
265	-14.949999999999614	10.137595046821243
266	-15.050000000000399	10.137595046821117
267	-15.050000000000399	10.137595046821117
268	-15.150000000000826	10.137595046821067
269	-15.150000000000826	10.137595046821067
270	-15.266666666666664	10.175733661783525
271	-15.266666666666664	10.175733661783525
272	-15.383333333332489	10.213702669562313
273	-15.383333333332489	10.213702669562313
274	-15.48333333333286	10.21370266956227
275	-15.48333333333286	10.21370266956227
276	-15.633333333333825	10.326610716440022
277	-15.633333333333825	10.326610716440022
278	-15.73333333333418	10.326610716439983
279	-15.73333333333418	10.326610716439983
280	-15.83333333333333	10.326610716440085
281	-15.83333333333333	10.326610716440085
282	-15.93333333333247	10.3266107164397
283	-15.93333333333247	10.3266107164397
284	-16.033333333332774	10.32661071643965
285	-16.033333333332774	10.32661071643965
286	-16.150000000000567	10.363919786129909
287	-16.150000000000567	10.363919786129909
288	-16.250000000000867	10.363919786129879
289	-16.250000000000867	10.363919786129879
290	-16.43333333333333	10.548090927851284
291	-16.43333333333333	10.548090927851284
292	-16.54999999999911	10.584461882085888
293	-16.54999999999911	10.584461882085888
294	-16.649999999999366	10.584461882085835
295	-16.649999999999366	10.584461882085835
296	-16.78333333333398	10.65675320577941
297	-16.78333333333398	10.65675320577941
298	-16.900000000000894	10.692676621563507
299	-16.900000000000894	10.692676621563507


==> avoid_sim_files/avoid_mem1_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.39999999999999963	3.885780586188048e-16
9	-0.39999999999999963	3.885780586188048e-16
10	-0.5	0.0
11	-0.5	0.0
12	-0.5999999999999699	3.008704396734174e-14
13	-0.5999999999999699	3.008704396734174e-14
14	-0.716666666666688	0.9127187713395325
15	-0.716666666666688	0.9127187713395325
16	-0.8333333333333375	1.2905640455070582
17	-0.8333333333333375	1.2905640455070582
18	-0.9333333333333836	1.2905640455070575
19	-0.9333333333333836	1.2905640455070575
20	-1.0333333333333332	1.2905640455070582
21	-1.0333333333333332	1.2905640455070582
22	-1.1666666666666077	1.8245242911205517
23	-1.1666666666666077	1.8245242911205517
24	-1.2666666666666015	1.8245242911205521
25	-1.2666666666666015	1.8245242911205521
26	-1.3666666666667384	1.824524291120547
27	-1.3666666666667384	1.824524291120547
28	-1.483333333333361	2.0395397084200897
29	-1.483333333333361	2.0395397084200897
30	-1.616666666666667	2.4124100443793086
31	-1.616666666666667	2.4124100443793086
32	-1.71666666666669	2.4124100443793073
33	-1.71666666666669	2.4124100443793073
34	-1.816666666666569	2.412410044379313
35	-1.816666666666569	2.412410044379313
36	-1.9166666666667689	2.4124100443793037
37	-1.9166666666667689	2.4124100443793037
38	-2.016666666666595	2.412410044379312
39	-2.016666666666595	2.412410044379312
40	-2.166666666666667	2.88193607763171
41	-2.2	3.409789827345278
42	-2.333333333333447	4.275381724348123
43	-2.333333333333447	4.275381724348123
44	-2.4333333333332097	4.275381724348134
45	-2.4333333333332097	4.275381724348134
46	-2.550000000000126	4.370831347314445
47	-2.550000000000126	4.370831347314445
48	-2.6499999999998582	4.37083134731446
49	-2.6499999999998582	4.37083134731446
50	-2.7500000000000004	4.370831347314452
51	-2.7500000000000004	4.370831347314452
52	-2.900000000000163	4.645069070171564
53	-2.900000000000163	4.645069070171564
54	-2.9999999999999565	4.6450690701715756
55	-2.9999999999999565	4.6450690701715756
56	-3.1166666666666822	4.732834480754701
57	-3.1166666666666822	4.732834480754701
58	-3.216666666666483	4.732834480754715
59	-3.216666666666483	4.732834480754715
60	-3.3166666666666673	4.732834480754701
61	-3.3166666666666673	4.732834480754701
62	-3.416666666666862	4.73283448075469
63	-3.416666666666862	4.73283448075469
64	-3.550000000000069	4.903485155138617
65	-3.550000000000069	4.903485155138617
66	-3.6499999999999106	4.903485155138621
67	-3.666666666666573	4.9865374314805315
68	-3.799999999999787	5.307855813163431
69	-3.799999999999787	5.307855813163431
70	-3.933333333333333	5.460056979759867
71	-3.933333333333333	5.460056979759867
72	-4.0500000000002245	5.534512926476245
73	-4.0500000000002245	5.534512926476245
74	-4.150000000000174	5.534512926476247
75	-4.150000000000174	5.534512926476247
76	-4.249999999999811	5.534512926476271
77	-4.249999999999811	5.534512926476271
78	-4.349999999999764	5.534512926476274
79	-4.349999999999764	5.534512926476274
80	-4.466666666666668	5.607930891950306
81	-4.466666666666668	5.607930891950306
82	-4.583333333333577	5.680351123732423
83	-4.583333333333577	5.680351123732423
84	-4.733333333333569	5.891990797307524
85	-4.733333333333569	5.891990797307524
86	-4.866666666666419	6.028727523744709
87	-4.866666666666419	6.028727523744709
88	-4.9833333333330785	6.095877477625753
89	-4.9833333333330785	6.095877477625753
90	-5.083333333333333	6.095877477625731
91	-5.083333333333333	6.095877477625731
92	-5.183333333333593	6.095877477625712
93	-5.183333333333593	6.095877477625712
94	-5.283333333333617	6.09587747762571
95	-5.283333333333617	6.09587747762571
96	-5.38333333333304	6.095877477625758
97	-5.38333333333304	6.095877477625758
98	-5.499999999999739	6.162250671088782
99	-5.499999999999739	6.162250671088782
100	-5.6	6.162250671088756
101	-5.6	6.162250671088756
102	-5.7000000000001965	6.162250671088745
103	-5.7000000000001965	6.162250671088745
104	-5.816666666666997	6.227871939024287
105	-5.816666666666997	6.227871939024287
106	-5.9166666666663295	6.227871939024347
107	-5.9166666666663295	6.227871939024347
108	-6.016666666666567	6.2278719390243245
109	-6.016666666666567	6.2278719390243245
110	-6.133333333333334	6.29276480482883
111	-6.133333333333334	6.29276480482883
112	-6.233333333333376	6.292764804828825
113	-6.233333333333376	6.292764804828825
114	-6.350000000000364	6.356951575506412
115	-6.350000000000364	6.356951575506412
116	-6.483333333332961	6.483290488290338
117	-6.483333333332961	6.483290488290338
118	-6.583333333333377	6.483290488290298
119	-6.583333333333377	6.483290488290298
120	-6.683333333333334	6.483290488290301
121	-6.683333333333334	6.483290488290301
122	-6.799999999999909	6.545481902299957
123	-6.799999999999909	6.545481902299957
124	-6.90000000000039	6.54548190229991
125	-6.90000000000039	6.54548190229991
126	-7.0166666666662705	6.6070459023343595
127	-7.0166666666662705	6.6070459023343595
128	-7.116666666666806	6.607045902334306
129	-7.116666666666806	6.607045902334306
130	-7.233333333333333	6.667999866693223
131	-7.233333333333333	6.667999866693223
132	-7.349999999999813	6.728360374811505
133	-7.349999999999813	6.728360374811505
134	-7.483333333333749	6.847363645147488
135	-7.483333333333749	6.847363645147488
136	-7.583333333332913	6.8473636451475715
137	-7.583333333332913	6.8473636451475715
138	-7.68333333333357	6.847363645147507
139	-7.70000000000024	6.90603600724281
140	-7.833333333333333	7.139483330201035
141	-7.833333333333333	7.139483330201035
142	-7.966666666666382	7.251360025693163
143	-7.966666666666382	7.251360025693163
144	-8.066666666667105	7.251360025693114
145	-8.083333333333771	7.306598996037186
146	-8.199999999999557	7.473731776473208
147	-8.199999999999557	7.473731776473208
148	-8.300000000000315	7.4737317764731515
149	-8.300000000000315	7.4737317764731515
150	-8.4	7.4737317764731825
151	-8.416666666666666	7.52726525520555
152	-8.58333333333298	7.844300832805489
153	-8.58333333333298	7.844300832805489
154	-8.683333333333794	7.844300832805812
155	-8.683333333333794	7.844300832805812
156	-8.78333333333287	7.844300832805502
157	-8.78333333333287	7.844300832805502
158	-8.883333333333724	7.844300832805817
159	-8.883333333333724	7.844300832805817
160	-9.0	7.895146188218006
161	-9.0	7.895146188218006
162	-9.099999999999577	7.895146188218056
163	-9.099999999999577	7.895146188218056
164	-9.216666666667143	7.945631224487712
165	-9.23333333333381	7.995762766754796
166	-9.349999999999518	8.14846611332458
167	-9.349999999999518	8.14846611332458
168	-9.450000000000456	8.148466113324977
169	-9.450000000000456	8.148466113324977
170	-9.55	8.148466113324552
171	-9.55	8.148466113324552
172	-9.649999999999523	8.148466113324579
173	-9.649999999999523	8.148466113324579
174	-9.783333333333825	8.245790171691091
175	-9.783333333333825	8.245790171691091
176	-9.883333333332839	8.245790171691187
177	-9.883333333332839	8.245790171691187
178	-9.983333333333842	8.245790171691093
179	-9.983333333333842	8.245790171691093
180	-10.083333333333332	8.245790171691128
181	-10.083333333333332	8.245790171691128
182	-10.183333333332804	8.24579017169119
183	-10.183333333332804	8.24579017169119
184	-10.316666666667171	8.341845652425587
185	-10.316666666667171	8.341845652425587
186	-10.433333333332824	8.389411315594314
187	-10.433333333332824	8.389411315594314
188	-10.550000000000558	8.436675885679122
189	-10.550000000000558	8.436675885679122
190	-10.666666666666666	8.48364439508312
191	-10.666666666666666	8.48364439508312
192	-10.766666666666088	8.483644395083187
193	-10.783333333332754	8.530321734195645
194	-10.900000000000517	8.673330771201314
195	-10.900000000000517	8.673330771201314
196	-10.999999999999496	8.673330771201428
197	-10.999999999999496	8.673330771201428
198	-11.100000000000597	8.673330771201307
199	-11.100000000000597	8.673330771201307
200	-11.199999999999998	8.673330771201362
201	-11.216666666666665	8.718928960727892
202	-11.333333333332723	8.858831124301155
203	-11.333333333332723	8.858831124301155
204	-11.43333333333369	8.858831124301053
205	-11.43333333333369	8.858831124301053
206	-11.533333333333008	8.85883112430112
207	-11.533333333333008	8.85883112430112
208	-11.666666666667304	8.947749561885313
209	-11.666666666667304	8.947749561885313
210	-11.783333333333331	8.991832713944106
211	-11.783333333333331	8.991832713944106
212	-11.88333333333268	8.991832713944172
213	-11.88333333333268	8.991832713944172
214	-12.000000000000208	9.035670054474926
215	-12.000000000000208	9.035670054474926
216	-12.116666666666491	9.079265144027792
217	-12.116666666666491	9.079265144027792
218	-12.216666666667345	9.079265144027715
219	-12.216666666667345	9.079265144027715
220	-12.33333333333333	9.122621455602811
221	-12.33333333333333	9.122621455602811
222	-12.433333333332639	9.122621455602886
223	-12.449999999999307	9.165742377643824
224	-12.583333333333407	9.25129120117249
225	-12.583333333333407	9.25129120117249
226	-12.68333333333328	9.251291201172492
227	-12.68333333333328	9.251291201172492
228	-12.783333333334042	9.251291201172425
229	-12.783333333334042	9.251291201172425
230	-12.883333333333331	9.251291201172503
231	-12.883333333333331	9.251291201172503
232	-12.999999999999275	9.293725481922134
233	-12.999999999999275	9.293725481922134
234	-13.11666666666661	9.33593713679658
235	-13.11666666666661	9.33593713679658
236	-13.25000000000008	9.419704524736126
237	-13.25000000000008	9.419704524736126
238	-13.383333333334075	9.502616598717394
239	-13.383333333334075	9.502616598717394
240	-13.516666666666667	9.584695555357257
241	-13.516666666666667	9.584695555357257
242	-13.633333333332573	9.625429283356311
243	-13.633333333332573	9.625429283356311
244	-13.733333333333153	9.625429283356244
245	-13.749999999999815	9.66596261803928
246	-13.883333333333535	9.831567638083806
247	-13.883333333333535	9.831567638083806
248	-13.983333333334107	9.831567638083943
249	-13.983333333334107	9.831567638083943
250	-14.1	9.871170143402358
251	-14.1	9.871170143402358
252	-14.233333333332546	9.9498185354752
253	-14.233333333332546	9.9498185354752
254	-14.366666666666395	10.027739304327534
255	-14.366666666666395	10.027739304327534
256	-14.483333333333617	10.066432116472514
257	-14.483333333333617	10.066432116472514
258	-14.600000000000804	10.104949282406334
259	-14.600000000000804	10.104949282406334
260	-14.733333333333333	10.181464640326517
261	-14.733333333333333	10.181464640326517
262	-14.833333333332513	10.181464640326451
263	-14.849999999999177	10.219466717984965
264	-14.94999999999962	10.219466717984908
265	-14.94999999999962	10.219466717984908
266	-15.050000000000395	10.219466717984785
267	-15.050000000000395	10.219466717984785
268	-15.150000000000826	10.219466717984728
269	-15.150000000000826	10.219466717984728
270	-15.266666666666667	10.257300922865658
271	-15.266666666666667	10.257300922865658
272	-15.383333333332489	10.294969105776424
273	-15.383333333332489	10.294969105776424
274	-15.483333333332865	10.29496910577638
275	-15.483333333332865	10.29496910577638
276	-15.633333333333821	10.406995510499677
277	-15.633333333333821	10.406995510499677
278	-15.73333333333418	10.406995510499648
279	-15.73333333333418	10.406995510499648
280	-15.83333333333333	10.406995510499744
281	-15.83333333333333	10.406995510499744
282	-15.93333333333247	10.406995510499344
283	-15.93333333333247	10.406995510499344
284	-16.033333333332774	10.406995510499296
285	-16.033333333332774	10.406995510499296
286	-16.150000000000563	10.444017426259004
287	-16.150000000000563	10.444017426259004
288	-16.250000000000867	10.444017426258968
289	-16.250000000000867	10.444017426258968
290	-16.43333333333333	10.626800501039119
291	-16.43333333333333	10.626800501039119
292	-16.54999999999911	10.662902981833595
293	-16.54999999999911	10.662902981833595
294	-16.649999999999366	10.662902981833541
295	-16.649999999999366	10.662902981833541
296	-16.783333333333978	10.734666066327183
297	-16.783333333333978	10.734666066327183
298	-16.900000000000894	10.770329614268892
299	-16.900000000000894	10.770329614268892


==> evade_sim_files/evade_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.39999999999999963	3.885780586188048e-16
9	-0.39999999999999963	3.885780586188048e-16
10	-0.5066666666666667	0.25811280910140844
11	-0.5066666666666667	0.25811280910140844
12	-0.6099999999999688	0.31606961258558514
13	-0.6099999999999688	0.31606961258558514
14	-0.7233333333333534	0.4824820088758875
15	-0.7233333333333534	0.4824820088758875
16	-0.8800000000000133	0.9275056154367393
17	7.993333333333767	9.936999323515675
18	7.904366666666711	10.039134969320036
19	9.364366666666639	10.066969765801211
20	9.302700000000176	10.140061606157449
21	11.829366666666731	9.652659094720535
22	11.780333333333656	9.724734437962114
23	12.58700000000025	9.4343067754517
24	12.538666666666645	9.513291660735723
25	13.925333333333278	8.790789017804697
26	13.88726666666652	8.863851938946121
27	14.460599999999777	8.502416968525353
28	14.432066666666332	8.563325195013705
29	15.378733333332917	7.792666278552477
30	15.35493333333307	7.852523734160584
31	15.734933333333036	7.468242519420952
32	15.706366666666513	7.542990750727092
33	16.32636666666647	6.888571317689043
34	16.307566666666425	6.947323663029454
35	16.647566666666403	6.504195626328869
36	16.633799999999606	6.54578115226383
37	17.08046666666625	5.8918201869673315
38	17.072266666666227	5.918215175390517
39	17.305599999999544	5.53628352838502
40	17.298566666666286	5.560747666656208
41	17.578566666666276	5.050047915174217
42	17.572933333333	5.071893209531221
43	17.759599999999658	4.6987261933421465
44	17.75156666666631	4.7361916007367615
45	17.998233333332962	4.162678650287119
46	17.99476666666624	4.1795058653971475
47	18.054766666666236	4.028560199238545
48	18.05159999999956	4.044566409394263
49	18.158266666666226	3.757321518789068
50	18.15563333333292	3.7717363285657077
51	18.182299999999586	3.6955356007846727
52	18.179799999999613	3.709533478305156
53	18.27313333333294	3.4263242961258733
54	18.26776666666627	3.46380008260032
55	18.287766666666265	3.3801578383593065
56	18.282499999999565	3.417704456210369
57	18.36916666666623	3.1014339649409233
58	18.364333333332894	3.139690200570107
59	18.404333333332893	2.9701135593703727
60	18.403033333332907	2.979445272567047
61	18.449699999999574	2.7947510163399647
62	18.448633333332918	2.8029445467619163
63	18.508633333332913	2.5430419053217035
64	18.50453333333292	2.5842431739722476
65	18.531199999999583	2.460357675894558
66	18.53056666666623	2.466093201581992
67	18.550566666666228	2.36812014311401
68	18.550033333332898	2.3731877293819226
69	18.570033333332898	2.2405993243376026
70	18.569599999999568	2.2448539314025306
71	18.576266666666235	2.2087092902618495
72	18.57586666666624	2.212712720219754
73	18.589199999999572	2.138043504390537
74	18.58886666666624	2.1415078913907335
75	18.595533333332906	2.1028932566559146
76	18.595233333332896	2.106078649739556
77	18.601899999999564	2.066459062422182
78	18.6016333333329	2.069354327374172
79	18.61496666666623	1.9871267361584128
80	18.614766666666235	1.9893965447396766
81	18.6214333333329	1.9466528398481442
82	18.614599999999566	2.0412218987655604
83	18.634599999999566	1.8414494761826363
84	18.6345333333329	1.8422741694860367
85	18.6345333333329	1.8422741694860367
86	18.63446666666623	1.8431021084633887
87	18.63446666666623	1.8431021084633887
88	18.634399999999566	1.8439332887426703
89	18.634399999999566	1.8439332887426703
90	18.6343333333329	1.8447677059426413
91	18.6343333333329	1.8447677059426413
92	18.63426666666623	1.845605355673017
93	18.63426666666623	1.845605355673017
94	18.634199999999566	1.8464462335343754
95	18.64086666666623	1.7976456590651118
96	18.6408333333329	1.7980793379479865
97	18.6408333333329	1.7980793379479865
98	18.640799999999565	1.7985147650213977
99	18.640799999999565	1.7985147650213977
100	18.64076666666623	1.798951939015846
101	18.647433333332895	1.7476575023600955
102	18.647433333332895	1.7476575023600955
103	18.647433333332895	1.7476575023600955
104	18.647433333332895	1.7476575023600955
105	18.647433333332895	1.7476575023600955
106	18.647433333332895	1.7476575023600955
107	18.647433333332895	1.7476575023600955
108	18.647433333332895	1.7476575023600955
109	18.647433333332895	1.7476575023600955
110	18.647433333332895	1.7476575023600955
111	18.647433333332895	1.7476575023600955
112	18.647433333332895	1.7476575023600955
113	18.647433333332895	1.7476575023600955
114	18.647433333332895	1.7476575023600955
115	18.647433333332895	1.7476575023600955
116	18.647433333332895	1.7476575023600955
117	18.647433333332895	1.7476575023600955
118	18.647433333332895	1.7476575023600955
119	18.647433333332895	1.7476575023600955
120	18.647433333332895	1.7476575023600955
121	18.647433333332895	1.7476575023600955
122	18.647433333332895	1.7476575023600955
123	18.647433333332895	1.7476575023600955
124	18.647433333332895	1.7476575023600955
125	18.647433333332895	1.7476575023600955
126	18.647433333332895	1.7476575023600955
127	18.647433333332895	1.7476575023600955
128	18.647433333332895	1.7476575023600955
129	18.647433333332895	1.7476575023600955
130	18.647433333332895	1.7476575023600955
131	18.647433333332895	1.7476575023600955
132	18.647433333332895	1.7476575023600955
133	18.647433333332895	1.7476575023600955
134	18.647433333332895	1.7476575023600955
135	18.647433333332895	1.7476575023600955
136	18.647433333332895	1.7476575023600955
137	18.647433333332895	1.7476575023600955
138	18.647433333332895	1.7476575023600955
139	18.647433333332895	1.7476575023600955
140	18.647433333332895	1.7476575023600955
141	18.647433333332895	1.7476575023600955
142	18.647433333332895	1.7476575023600955
143	18.647433333332895	1.7476575023600955
144	18.647433333332895	1.7476575023600955
145	18.647433333332895	1.7476575023600955
146	18.647433333332895	1.7476575023600955
147	18.647433333332895	1.7476575023600955
148	18.647433333332895	1.7476575023600955
149	18.647433333332895	1.7476575023600955
150	18.647433333332895	1.7476575023600955
151	18.647433333332895	1.7476575023600955
152	18.647433333332895	1.7476575023600955
153	18.647433333332895	1.7476575023600955
154	18.647433333332895	1.7476575023600955
155	18.647433333332895	1.7476575023600955
156	18.647433333332895	1.7476575023600955
157	18.647433333332895	1.7476575023600955
158	18.647433333332895	1.7476575023600955
159	18.647433333332895	1.7476575023600955
160	18.647433333332895	1.7476575023600955
161	18.647433333332895	1.7476575023600955
162	18.647433333332895	1.7476575023600955
163	18.647433333332895	1.7476575023600955
164	18.647433333332895	1.7476575023600955
165	18.647433333332895	1.7476575023600955
166	18.647433333332895	1.7476575023600955
167	18.647433333332895	1.7476575023600955
168	18.647433333332895	1.7476575023600955
169	18.647433333332895	1.7476575023600955
170	18.647433333332895	1.7476575023600955
171	18.647433333332895	1.7476575023600955
172	18.647433333332895	1.7476575023600955
173	18.647433333332895	1.7476575023600955
174	18.647433333332895	1.7476575023600955
175	18.647433333332895	1.7476575023600955
176	18.647433333332895	1.7476575023600955
177	18.647433333332895	1.7476575023600955
178	18.647433333332895	1.7476575023600955
179	18.647433333332895	1.7476575023600955
180	18.647433333332895	1.7476575023600955
181	18.647433333332895	1.7476575023600955
182	18.647433333332895	1.7476575023600955
183	18.647433333332895	1.7476575023600955
184	18.647433333332895	1.7476575023600955
185	18.647433333332895	1.7476575023600955
186	18.647433333332895	1.7476575023600955
187	18.647433333332895	1.7476575023600955
188	18.647433333332895	1.7476575023600955
189	18.647433333332895	1.7476575023600955
190	18.647433333332895	1.7476575023600955
191	18.647433333332895	1.7476575023600955
192	18.647433333332895	1.7476575023600955
193	18.647433333332895	1.7476575023600955
194	18.647433333332895	1.7476575023600955
195	18.647433333332895	1.7476575023600955
196	18.647433333332895	1.7476575023600955
197	18.647433333332895	1.7476575023600955
198	18.647433333332895	1.7476575023600955
199	18.647433333332895	1.7476575023600955
200	18.647433333332895	1.7476575023600955
201	18.647433333332895	1.7476575023600955
202	18.647433333332895	1.7476575023600955
203	18.647433333332895	1.7476575023600955
204	18.647433333332895	1.7476575023600955
205	18.647433333332895	1.7476575023600955
206	18.647433333332895	1.7476575023600955
207	18.647433333332895	1.7476575023600955
208	18.647433333332895	1.7476575023600955
209	18.647433333332895	1.7476575023600955
210	18.647433333332895	1.7476575023600955
211	18.647433333332895	1.7476575023600955
212	18.647433333332895	1.7476575023600955
213	18.647433333332895	1.7476575023600955
214	18.647433333332895	1.7476575023600955
215	18.647433333332895	1.7476575023600955
216	18.647433333332895	1.7476575023600955
217	18.647433333332895	1.7476575023600955
218	18.647433333332895	1.7476575023600955
219	18.647433333332895	1.7476575023600955
220	18.647433333332895	1.7476575023600955
221	18.647433333332895	1.7476575023600955
222	18.647433333332895	1.7476575023600955
223	18.647433333332895	1.7476575023600955
224	18.647433333332895	1.7476575023600955
225	18.647433333332895	1.7476575023600955
226	18.647433333332895	1.7476575023600955
227	18.647433333332895	1.7476575023600955
228	18.647433333332895	1.7476575023600955
229	18.647433333332895	1.7476575023600955
230	18.647433333332895	1.7476575023600955
231	18.647433333332895	1.7476575023600955
232	18.647433333332895	1.7476575023600955
233	18.647433333332895	1.7476575023600955
234	18.647433333332895	1.7476575023600955
235	18.647433333332895	1.7476575023600955
236	18.647433333332895	1.7476575023600955
237	18.647433333332895	1.7476575023600955
238	18.647433333332895	1.7476575023600955
239	18.647433333332895	1.7476575023600955
240	18.647433333332895	1.7476575023600955
241	18.647433333332895	1.7476575023600955
242	18.647433333332895	1.7476575023600955
243	18.647433333332895	1.7476575023600955
244	18.647433333332895	1.7476575023600955
245	18.647433333332895	1.7476575023600955
246	18.647433333332895	1.7476575023600955
247	18.647433333332895	1.7476575023600955
248	18.647433333332895	1.7476575023600955
249	18.647433333332895	1.7476575023600955
250	18.647433333332895	1.7476575023600955
251	18.647433333332895	1.7476575023600955
252	18.647433333332895	1.7476575023600955
253	18.647433333332895	1.7476575023600955
254	18.647433333332895	1.7476575023600955
255	18.647433333332895	1.7476575023600955
256	18.647433333332895	1.7476575023600955
257	18.647433333332895	1.7476575023600955
258	18.647433333332895	1.7476575023600955
259	18.647433333332895	1.7476575023600955
260	18.647433333332895	1.7476575023600955
261	18.647433333332895	1.7476575023600955
262	18.647433333332895	1.7476575023600955
263	18.647433333332895	1.7476575023600955
264	18.647433333332895	1.7476575023600955
265	18.647433333332895	1.7476575023600955
266	18.647433333332895	1.7476575023600955
267	18.647433333332895	1.7476575023600955
268	18.647433333332895	1.7476575023600955
269	18.647433333332895	1.7476575023600955
270	18.647433333332895	1.7476575023600955
271	18.647433333332895	1.7476575023600955
272	18.647433333332895	1.7476575023600955
273	18.647433333332895	1.7476575023600955
274	18.647433333332895	1.7476575023600955
275	18.647433333332895	1.7476575023600955
276	18.647433333332895	1.7476575023600955
277	18.647433333332895	1.7476575023600955
278	18.647433333332895	1.7476575023600955
279	18.647433333332895	1.7476575023600955
280	18.647433333332895	1.7476575023600955
281	18.647433333332895	1.7476575023600955
282	18.647433333332895	1.7476575023600955
283	18.647433333332895	1.7476575023600955
284	18.647433333332895	1.7476575023600955
285	18.647433333332895	1.7476575023600955
286	18.647433333332895	1.7476575023600955
287	18.647433333332895	1.7476575023600955
288	18.647433333332895	1.7476575023600955
289	18.647433333332895	1.7476575023600955
290	18.647433333332895	1.7476575023600955
291	18.647433333332895	1.7476575023600955
292	18.647433333332895	1.7476575023600955
293	18.647433333332895	1.7476575023600955
294	18.647433333332895	1.7476575023600955
295	18.647433333332895	1.7476575023600955
296	18.647433333332895	1.7476575023600955
297	18.647433333332895	1.7476575023600955
298	18.647433333332895	1.7476575023600955
299	18.647433333332895	1.7476575023600955


==> evade_sim_files/evade_mem1_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=1, N=10}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.09999999999999991	9.71445146547012e-17
4	-0.19999999999999982	1.942890293094024e-16
5	-0.19999999999999982	1.942890293094024e-16
6	-0.29999999999998495	1.509903313490213e-14
7	-0.29999999999998495	1.509903313490213e-14
8	-0.43000000000000577	0.5469003565550136
9	-0.43000000000000577	0.5469003565550136
10	-0.53	0.5469003565550139
11	-0.53	0.5469003565550139
12	-0.6333333333332998	0.5763872155263312
13	-0.6333333333332998	0.5763872155263312
14	-0.7733333333333411	0.8914158525751367
15	-0.7733333333333411	0.8914158525751367
16	-0.9166666666666903	1.134190852056567
17	7.363333333333734	9.899157652155312
18	7.281400000000073	9.978986289866059
19	8.428066666666664	10.10128600371709
20	8.341866666666832	10.204410509622283
21	11.315200000000138	9.838850659163926
22	11.237200000000371	9.960214329688801
23	11.957166666666973	9.735986954193299
24	11.89613333333335	9.838851476784246
25	13.596099999999964	9.00669018692959
26	13.550233333333255	9.097119321277185
27	14.16353333333319	8.719679859311773
28	14.134066666666394	8.791523159397457
29	15.247399999999626	7.8906387514995435
30	15.226833333333106	7.936513296502078
31	15.646833333333067	7.542853348626758
32	15.6250333333332	7.597144858359001
33	16.36503333333317	6.758399267989112
34	16.350266666666478	6.8003029292001145
35	16.590266666666462	6.495310508016836
36	16.566699999999663	6.571930800254604
37	17.0733666666663	5.847105323624209
38	17.055666666666287	5.912970028298489
39	17.24899999999962	5.585365908634111
40	17.23893333333301	5.629187406919622
41	17.512266666666324	5.08878730107238
42	17.506899999999703	5.109569034990419
43	17.64689999999969	4.823362975145085
44	17.638899999999683	4.859682786972825
45	17.845566666666343	4.40155961134483
46	17.841933333332957	4.418266054561358
47	17.941933333332948	4.181230472267899
48	17.935466666666283	4.216644256066926
49	18.06879999999961	3.839208237818472
50	18.062999999999633	3.8745112810090645
51	18.156333333332963	3.609898413467561
52	18.15433333333298	3.6215357546519202
53	18.234333333332977	3.3548613317922804
54	18.232733333332977	3.3649054264405613
55	18.279399999999644	3.2093647824245393
56	18.27136666666629	3.2719764871132235
57	18.32469999999962	3.042264492665493
58	18.32359999999962	3.050020170425109
59	18.390266666666285	2.793152089585407
60	18.389499999999625	2.799122436883819
61	18.40949999999963	2.7164510701771865
62	18.408833333332964	2.7218349151915615
63	18.442166666666296	2.576823361988348
64	18.438333333332963	2.615315893390754
65	18.478333333332962	2.4028893487262977
66	18.478033333332956	2.4057391377472337
67	18.49136666666629	2.3395132254856312
68	18.491133333332957	2.3418329108248312
69	18.511133333332957	2.207895540000777
70	18.510999999999623	2.209221356043808
71	18.510999999999623	2.209221356043808
72	18.510866666666292	2.210552400545066
73	18.510866666666292	2.210552400545066
74	18.510733333332958	2.2118886640656528
75	18.510733333332958	2.2118886640656528
76	18.510599999999624	2.213230137152515
77	18.510599999999624	2.213230137152515
78	18.51046666666629	2.2145768103384738
79	18.517133333332957	2.1768861053246775
80	18.517033333332957	2.17791793514405
81	18.52369999999962	2.1392494735303793
82	18.523633333332956	2.139952834111568
83	18.53029999999962	2.100247265601502
84	18.530266666666286	2.100607196873227
85	18.530266666666286	2.100607196873227
86	18.53023333333295	2.1009686525240934
87	18.53023333333295	2.1009686525240934
88	18.530199999999617	2.101331631767503
89	18.536866666666285	2.059890170750784
90	18.536866666666285	2.059890170750784
91	18.536866666666285	2.059890170750784
92	18.536866666666285	2.059890170750784
93	18.536866666666285	2.059890170750784
94	18.536866666666285	2.059890170750784
95	18.536866666666285	2.059890170750784
96	18.536866666666285	2.059890170750784
97	18.536866666666285	2.059890170750784
98	18.536866666666285	2.059890170750784
99	18.536866666666285	2.059890170750784
100	18.536866666666285	2.059890170750784
101	18.536866666666285	2.059890170750784
102	18.536866666666285	2.059890170750784
103	18.536866666666285	2.059890170750784
104	18.536866666666285	2.059890170750784
105	18.536866666666285	2.059890170750784
106	18.536866666666285	2.059890170750784
107	18.536866666666285	2.059890170750784
108	18.536866666666285	2.059890170750784
109	18.536866666666285	2.059890170750784
110	18.536866666666285	2.059890170750784
111	18.536866666666285	2.059890170750784
112	18.536866666666285	2.059890170750784
113	18.536866666666285	2.059890170750784
114	18.536866666666285	2.059890170750784
115	18.536866666666285	2.059890170750784
116	18.536866666666285	2.059890170750784
117	18.536866666666285	2.059890170750784
118	18.536866666666285	2.059890170750784
119	18.536866666666285	2.059890170750784
120	18.536866666666285	2.059890170750784
121	18.536866666666285	2.059890170750784
122	18.536866666666285	2.059890170750784
123	18.536866666666285	2.059890170750784
124	18.536866666666285	2.059890170750784
125	18.536866666666285	2.059890170750784
126	18.536866666666285	2.059890170750784
127	18.536866666666285	2.059890170750784
128	18.536866666666285	2.059890170750784
129	18.536866666666285	2.059890170750784
130	18.536866666666285	2.059890170750784
131	18.536866666666285	2.059890170750784
132	18.536866666666285	2.059890170750784
133	18.536866666666285	2.059890170750784
134	18.536866666666285	2.059890170750784
135	18.536866666666285	2.059890170750784
136	18.536866666666285	2.059890170750784
137	18.536866666666285	2.059890170750784
138	18.536866666666285	2.059890170750784
139	18.536866666666285	2.059890170750784
140	18.536866666666285	2.059890170750784
141	18.536866666666285	2.059890170750784
142	18.536866666666285	2.059890170750784
143	18.536866666666285	2.059890170750784
144	18.536866666666285	2.059890170750784
145	18.536866666666285	2.059890170750784
146	18.536866666666285	2.059890170750784
147	18.536866666666285	2.059890170750784
148	18.536866666666285	2.059890170750784
149	18.536866666666285	2.059890170750784
150	18.536866666666285	2.059890170750784
151	18.536866666666285	2.059890170750784
152	18.536866666666285	2.059890170750784
153	18.536866666666285	2.059890170750784
154	18.536866666666285	2.059890170750784
155	18.536866666666285	2.059890170750784
156	18.536866666666285	2.059890170750784
157	18.536866666666285	2.059890170750784
158	18.536866666666285	2.059890170750784
159	18.536866666666285	2.059890170750784
160	18.536866666666285	2.059890170750784
161	18.536866666666285	2.059890170750784
162	18.536866666666285	2.059890170750784
163	18.536866666666285	2.059890170750784
164	18.536866666666285	2.059890170750784
165	18.536866666666285	2.059890170750784
166	18.536866666666285	2.059890170750784
167	18.536866666666285	2.059890170750784
168	18.536866666666285	2.059890170750784
169	18.536866666666285	2.059890170750784
170	18.536866666666285	2.059890170750784
171	18.536866666666285	2.059890170750784
172	18.536866666666285	2.059890170750784
173	18.536866666666285	2.059890170750784
174	18.536866666666285	2.059890170750784
175	18.536866666666285	2.059890170750784
176	18.536866666666285	2.059890170750784
177	18.536866666666285	2.059890170750784
178	18.536866666666285	2.059890170750784
179	18.536866666666285	2.059890170750784
180	18.536866666666285	2.059890170750784
181	18.536866666666285	2.059890170750784
182	18.536866666666285	2.059890170750784
183	18.536866666666285	2.059890170750784
184	18.536866666666285	2.059890170750784
185	18.536866666666285	2.059890170750784
186	18.536866666666285	2.059890170750784
187	18.536866666666285	2.059890170750784
188	18.536866666666285	2.059890170750784
189	18.536866666666285	2.059890170750784
190	18.536866666666285	2.059890170750784
191	18.536866666666285	2.059890170750784
192	18.536866666666285	2.059890170750784
193	18.536866666666285	2.059890170750784
194	18.536866666666285	2.059890170750784
195	18.536866666666285	2.059890170750784
196	18.536866666666285	2.059890170750784
197	18.536866666666285	2.059890170750784
198	18.536866666666285	2.059890170750784
199	18.536866666666285	2.059890170750784
200	18.536866666666285	2.059890170750784
201	18.536866666666285	2.059890170750784
202	18.536866666666285	2.059890170750784
203	18.536866666666285	2.059890170750784
204	18.536866666666285	2.059890170750784
205	18.536866666666285	2.059890170750784
206	18.536866666666285	2.059890170750784
207	18.536866666666285	2.059890170750784
208	18.536866666666285	2.059890170750784
209	18.536866666666285	2.059890170750784
210	18.536866666666285	2.059890170750784
211	18.536866666666285	2.059890170750784
212	18.536866666666285	2.059890170750784
213	18.536866666666285	2.059890170750784
214	18.536866666666285	2.059890170750784
215	18.536866666666285	2.059890170750784
216	18.536866666666285	2.059890170750784
217	18.536866666666285	2.059890170750784
218	18.536866666666285	2.059890170750784
219	18.536866666666285	2.059890170750784
220	18.536866666666285	2.059890170750784
221	18.536866666666285	2.059890170750784
222	18.536866666666285	2.059890170750784
223	18.536866666666285	2.059890170750784
224	18.536866666666285	2.059890170750784
225	18.536866666666285	2.059890170750784
226	18.536866666666285	2.059890170750784
227	18.536866666666285	2.059890170750784
228	18.536866666666285	2.059890170750784
229	18.536866666666285	2.059890170750784
230	18.536866666666285	2.059890170750784
231	18.536866666666285	2.059890170750784
232	18.536866666666285	2.059890170750784
233	18.536866666666285	2.059890170750784
234	18.536866666666285	2.059890170750784
235	18.536866666666285	2.059890170750784
236	18.536866666666285	2.059890170750784
237	18.536866666666285	2.059890170750784
238	18.536866666666285	2.059890170750784
239	18.536866666666285	2.059890170750784
240	18.536866666666285	2.059890170750784
241	18.536866666666285	2.059890170750784
242	18.536866666666285	2.059890170750784
243	18.536866666666285	2.059890170750784
244	18.536866666666285	2.059890170750784
245	18.536866666666285	2.059890170750784
246	18.536866666666285	2.059890170750784
247	18.536866666666285	2.059890170750784
248	18.536866666666285	2.059890170750784
249	18.536866666666285	2.059890170750784
250	18.536866666666285	2.059890170750784
251	18.536866666666285	2.059890170750784
252	18.536866666666285	2.059890170750784
253	18.536866666666285	2.059890170750784
254	18.536866666666285	2.059890170750784
255	18.536866666666285	2.059890170750784
256	18.536866666666285	2.059890170750784
257	18.536866666666285	2.059890170750784
258	18.536866666666285	2.059890170750784
259	18.536866666666285	2.059890170750784
260	18.536866666666285	2.059890170750784
261	18.536866666666285	2.059890170750784
262	18.536866666666285	2.059890170750784
263	18.536866666666285	2.059890170750784
264	18.536866666666285	2.059890170750784
265	18.536866666666285	2.059890170750784
266	18.536866666666285	2.059890170750784
267	18.536866666666285	2.059890170750784
268	18.536866666666285	2.059890170750784
269	18.536866666666285	2.059890170750784
270	18.536866666666285	2.059890170750784
271	18.536866666666285	2.059890170750784
272	18.536866666666285	2.059890170750784
273	18.536866666666285	2.059890170750784
274	18.536866666666285	2.059890170750784
275	18.536866666666285	2.059890170750784
276	18.536866666666285	2.059890170750784
277	18.536866666666285	2.059890170750784
278	18.536866666666285	2.059890170750784
279	18.536866666666285	2.059890170750784
280	18.536866666666285	2.059890170750784
281	18.536866666666285	2.059890170750784
282	18.536866666666285	2.059890170750784
283	18.536866666666285	2.059890170750784
284	18.536866666666285	2.059890170750784
285	18.536866666666285	2.059890170750784
286	18.536866666666285	2.059890170750784
287	18.536866666666285	2.059890170750784
288	18.536866666666285	2.059890170750784
289	18.536866666666285	2.059890170750784
290	18.536866666666285	2.059890170750784
291	18.536866666666285	2.059890170750784
292	18.536866666666285	2.059890170750784
293	18.536866666666285	2.059890170750784
294	18.536866666666285	2.059890170750784
295	18.536866666666285	2.059890170750784
296	18.536866666666285	2.059890170750784
297	18.536866666666285	2.059890170750784
298	18.536866666666285	2.059890170750784
299	18.536866666666285	2.059890170750784


==> evade_sim_files/evade_mem1_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.10960000000000135	0.02945912422323493
4	-0.20110000000000006	0.010430244484190982
5	-0.21896666666666958	0.03928866107274251
6	-0.32613333333331496	0.4826286172847893
7	-0.35063333333331465	0.4833076303510753
8	-0.48850000000001675	0.9451725151173822
9	-0.5284333333333483	0.994921209052336
10	-0.7013999999999975	1.4700084036040764
11	-0.7690333333333181	1.5948597845021621
12	-0.9382333333332885	1.9718320277233423
13	-1.0484666666666225	2.1684735757875435
14	-1.2415999999999567	2.5129510089401217
15	-1.345333333333335	2.6472321813966326
16	-1.5889666666667384	2.9711223915475307
17	-0.257966666666658	6.019802588032947
18	2.1035333333333788	8.531828693128551
19	4.652400000000101	9.930114512934944
20	6.8638000000000305	10.421683304213957
21	8.741666666666731	10.45597168554356
22	10.484733333333391	10.230127740920603
23	12.143199999999982	9.694480238431133
24	13.371899999999988	9.073528919701959
25	14.206033333333243	8.51373206055289
26	14.976066666666517	7.766648388819651
27	15.553833333333179	7.198139016826144
28	16.063633333333193	6.567356200599746
29	16.410366666666544	6.106672514462208
30	16.641399999999887	5.7404273394931025
31	16.829466666666562	5.40129290530417
32	16.991266666666558	5.099495765487213
33	17.10353333333321	4.892593809240887
34	17.19579999999985	4.696017003092481
35	17.285199999999847	4.533083677439302
36	17.317999999999852	4.467646211000406
37	17.344133333333186	4.399480149088306
38	17.377099999999853	4.329923662529495
39	17.416799999999856	4.21190745703969
40	17.443233333333193	4.152226817691396
41	17.45643333333319	4.122081829879416
42	17.469599999999854	4.091832821609399
43	17.48616666666652	4.0646162556329735
44	17.486099999999855	4.064940769146178
45	17.485999999999855	4.065509890120401
46	17.492599999999854	4.0330921024279345
47	17.499233333333187	4.017032413638531
48	17.49916666666652	4.017364306634639
49	17.512499999999854	3.984017287864066
50	17.512466666666523	3.9841859790370755
51	17.512466666666523	3.9841859790370755
52	17.512433333333185	3.9843554993945287
53	17.512433333333185	3.9843554993945287
54	17.512399999999854	3.9845258488306805
55	17.512399999999854	3.9845258488306805
56	17.51236666666652	3.984697027239187
57	17.51236666666652	3.984697027239187
58	17.519033333333187	3.967064540129851
59	17.519033333333187	3.967064540129851
60	17.519033333333187	3.967064540129851
61	17.519033333333187	3.967064540129851
62	17.519033333333187	3.967064540129851
63	17.519033333333187	3.967064540129851
64	17.519033333333187	3.967064540129851
65	17.519033333333187	3.967064540129851
66	17.519033333333187	3.967064540129851
67	17.519033333333187	3.967064540129851
68	17.519033333333187	3.967064540129851
69	17.519033333333187	3.967064540129851
70	17.519033333333187	3.967064540129851
71	17.519033333333187	3.967064540129851
72	17.519033333333187	3.967064540129851
73	17.519033333333187	3.967064540129851
74	17.519033333333187	3.967064540129851
75	17.519033333333187	3.967064540129851
76	17.519033333333187	3.967064540129851
77	17.519033333333187	3.967064540129851
78	17.519033333333187	3.967064540129851
79	17.519033333333187	3.967064540129851
80	17.519033333333187	3.967064540129851
81	17.519033333333187	3.967064540129851
82	17.519033333333187	3.967064540129851
83	17.519033333333187	3.967064540129851
84	17.519033333333187	3.967064540129851
85	17.519033333333187	3.967064540129851
86	17.519033333333187	3.967064540129851
87	17.519033333333187	3.967064540129851
88	17.519033333333187	3.967064540129851
89	17.519033333333187	3.967064540129851
90	17.519033333333187	3.967064540129851
91	17.519033333333187	3.967064540129851
92	17.519033333333187	3.967064540129851
93	17.519033333333187	3.967064540129851
94	17.519033333333187	3.967064540129851
95	17.519033333333187	3.967064540129851
96	17.519033333333187	3.967064540129851
97	17.519033333333187	3.967064540129851
98	17.519033333333187	3.967064540129851
99	17.519033333333187	3.967064540129851
100	17.519033333333187	3.967064540129851
101	17.519033333333187	3.967064540129851
102	17.519033333333187	3.967064540129851
103	17.519033333333187	3.967064540129851
104	17.519033333333187	3.967064540129851
105	17.519033333333187	3.967064540129851
106	17.519033333333187	3.967064540129851
107	17.519033333333187	3.967064540129851
108	17.519033333333187	3.967064540129851
109	17.519033333333187	3.967064540129851
110	17.519033333333187	3.967064540129851
111	17.519033333333187	3.967064540129851
112	17.519033333333187	3.967064540129851
113	17.519033333333187	3.967064540129851
114	17.519033333333187	3.967064540129851
115	17.519033333333187	3.967064540129851
116	17.519033333333187	3.967064540129851
117	17.519033333333187	3.967064540129851
118	17.519033333333187	3.967064540129851
119	17.519033333333187	3.967064540129851
120	17.519033333333187	3.967064540129851


==> evade_sim_files/evade_mem1_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	0.0	0.0
2	-0.09999999999999991	9.71445146547012e-17
3	-0.1116333333333346	0.03206242175645628
4	-0.20166666666666677	0.012801909579781171
5	-0.22306666666666913	0.042598069857162184
6	-0.31723333333331627	0.36527571169674805
7	-0.35279999999998274	0.44942054544343035
8	-0.4710000000000116	0.7931450056578294
9	-0.5119666666666781	0.8338625779400866
10	-0.6784999999999962	1.3048733335717315
11	-0.7535999999999808	1.432931856951591
12	-0.9262999999999526	1.8437023376890518
13	-1.016999999999955	1.9986572992887146
14	-1.197833333333297	2.337894773556335
15	-1.2902333333333424	2.4709973584679266
16	-1.4924000000000703	2.7829329085217664
17	-0.6800666666666789	5.030654960230174
18	0.6743999999999811	7.245235076011321
19	2.3725000000000187	8.679550703617377
20	4.23046666666665	9.661388363768225
21	6.167299999999982	10.274993627410941
22	7.812733333333364	10.401025167207731
23	9.29493333333332	10.353066904491946
24	10.735400000000002	10.025018046866581
25	11.961433333333337	9.640546454716935
26	12.998266666666588	9.11008289363432
27	13.875933333333249	8.576810642398188
28	14.681233333333271	7.897417160833214
29	15.105166666666637	7.5182003590546564
30	15.603233333333323	7.0145272740854425
31	15.925799999999988	6.619307694917958
32	16.255599999999976	6.175023506567946
33	16.473099999999967	5.843198871907997
34	16.69403333333327	5.544827114727987
35	16.886233333333262	5.228102314628358
36	17.01149999999993	4.975609619266054
37	17.084099999999935	4.831508100307151
38	17.143166666666605	4.693413111892967
39	17.182399999999944	4.604039918738049
40	17.22183333333328	4.510454519471679
41	17.29476666666661	4.34217640654495
42	17.321066666666614	4.27024935207403
43	17.344099999999944	4.23083110708365
44	17.35719999999994	4.201238090531593
45	17.37029999999994	4.171638516218783
46	17.376766666666608	4.140871511999467
47	17.38996666666661	4.10989326692991
48	17.396499999999943	4.0947874690472394
49	17.402999999999942	4.079453925874563
50	17.402933333333273	4.079781619427932
51	17.40939999999994	4.064057698081257
52	17.409366666666607	4.064223041643025
53	17.415866666666602	4.048598306684513
54	17.42253333333327	4.0317356372769355
55	17.422399999999936	4.032408491212213
56	17.422399999999936	4.032408491212213
57	17.428966666666607	4.015644107598301
58	17.428966666666607	4.015644107598301
59	17.435566666666606	3.9984628311667745
60	17.435566666666606	3.9984628311667745
61	17.43549999999994	3.998806874139634
62	17.43549999999994	3.998806874139634
63	17.435433333333272	3.9991525534237615
64	17.435433333333272	3.9991525534237615
65	17.435366666666603	3.999499868594706
66	17.435366666666603	3.999499868594706
67	17.43529999999994	3.9998488192264214
68	17.43529999999994	3.9998488192264214
69	17.435233333333272	4.000199404890813
70	17.44189999999994	3.9815927788595964
71	17.448566666666604	3.963055800627658
72	17.448566666666604	3.963055800627658
73	17.448566666666604	3.963055800627658
74	17.448566666666604	3.963055800627658
75	17.448566666666604	3.963055800627658
76	17.448566666666604	3.963055800627658
77	17.448566666666604	3.963055800627658
78	17.448566666666604	3.963055800627658
79	17.448566666666604	3.963055800627658
80	17.448566666666604	3.963055800627658
81	17.448566666666604	3.963055800627658
82	17.448566666666604	3.963055800627658
83	17.448566666666604	3.963055800627658
84	17.448566666666604	3.963055800627658
85	17.448566666666604	3.963055800627658
86	17.448566666666604	3.963055800627658
87	17.448566666666604	3.963055800627658
88	17.448566666666604	3.963055800627658
89	17.448566666666604	3.963055800627658
90	17.448566666666604	3.963055800627658
91	17.448566666666604	3.963055800627658
92	17.448566666666604	3.963055800627658
93	17.448566666666604	3.963055800627658
94	17.448566666666604	3.963055800627658
95	17.448566666666604	3.963055800627658
96	17.448566666666604	3.963055800627658
97	17.448566666666604	3.963055800627658
98	17.448566666666604	3.963055800627658
99	17.448566666666604	3.963055800627658
100	17.448566666666604	3.963055800627658
101	17.448566666666604	3.963055800627658
102	17.448566666666604	3.963055800627658
103	17.448566666666604	3.963055800627658
104	17.448566666666604	3.963055800627658
105	17.448566666666604	3.963055800627658
106	17.448566666666604	3.963055800627658
107	17.448566666666604	3.963055800627658
108	17.448566666666604	3.963055800627658
109	17.448566666666604	3.963055800627658
110	17.448566666666604	3.963055800627658
111	17.448566666666604	3.963055800627658
112	17.448566666666604	3.963055800627658
113	17.448566666666604	3.963055800627658
114	17.448566666666604	3.963055800627658
115	17.448566666666604	3.963055800627658
116	17.448566666666604	3.963055800627658
117	17.448566666666604	3.963055800627658
118	17.448566666666604	3.963055800627658
119	17.448566666666604	3.963055800627658
120	17.448566666666604	3.963055800627658


==> intercept_sim_files/intercept_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29999999999998495	1.509903313490213e-14
4	-0.39999999999999963	3.885780586188048e-16
5	3.258700000000034	7.8372217213753785
6	4.142199999999869	8.556138098464624
7	8.382399999999787	10.04118868660459
8	9.875100000000238	10.113725821377614
9	13.806599999999817	9.05095334426155
10	14.616633333333285	8.608538009764189
11	17.068166666666656	6.379252566371325
12	17.49939999999995	5.800029279236462
13	18.165133333333202	4.656017359169612
14	18.414366666666517	4.153159873183606
15	18.831066666666512	2.9399333658359152
16	18.92956666666652	2.574574879901954
17	19.041466666666523	2.0659397818480043
18	19.107533333333183	1.6901173279456587
19	19.14679999999984	1.414103871715222
20	19.166499999999843	1.2530314241869684
21	19.20629999999984	0.8244090671505128
22	19.206199999999843	0.8269955018015558
23	19.206099999999843	0.8295859147791915
24	19.20599999999984	0.8321802689321398
25	19.219299999999837	0.6199173412641474
26	19.219266666666506	0.6210867858484624
27	19.22593333333317	0.4776129488287438
28	19.22593333333317	0.4776129488287438
29	19.22593333333317	0.4776129488287438
30	19.22593333333317	0.4776129488287438
31	19.22593333333317	0.4776129488287438
32	19.22593333333317	0.4776129488287438
33	19.22593333333317	0.4776129488287438
34	19.22593333333317	0.4776129488287438
35	19.22593333333317	0.4776129488287438
36	19.22593333333317	0.4776129488287438
37	19.22593333333317	0.4776129488287438
38	19.22593333333317	0.4776129488287438
39	19.22593333333317	0.4776129488287438
40	19.22593333333317	0.4776129488287438
41	19.22593333333317	0.4776129488287438
42	19.22593333333317	0.4776129488287438
43	19.22593333333317	0.4776129488287438
44	19.22593333333317	0.4776129488287438
45	19.22593333333317	0.4776129488287438
46	19.22593333333317	0.4776129488287438
47	19.22593333333317	0.4776129488287438
48	19.22593333333317	0.4776129488287438
49	19.22593333333317	0.4776129488287438
50	19.22593333333317	0.4776129488287438
51	19.22593333333317	0.4776129488287438
52	19.22593333333317	0.4776129488287438
53	19.22593333333317	0.4776129488287438
54	19.22593333333317	0.4776129488287438
55	19.22593333333317	0.4776129488287438
56	19.22593333333317	0.4776129488287438
57	19.22593333333317	0.4776129488287438
58	19.22593333333317	0.4776129488287438
59	19.22593333333317	0.4776129488287438
60	19.22593333333317	0.4776129488287438
61	19.22593333333317	0.4776129488287438
62	19.22593333333317	0.4776129488287438
63	19.22593333333317	0.4776129488287438
64	19.22593333333317	0.4776129488287438
65	19.22593333333317	0.4776129488287438
66	19.22593333333317	0.4776129488287438
67	19.22593333333317	0.4776129488287438
68	19.22593333333317	0.4776129488287438
69	19.22593333333317	0.4776129488287438
70	19.22593333333317	0.4776129488287438
71	19.22593333333317	0.4776129488287438
72	19.22593333333317	0.4776129488287438
73	19.22593333333317	0.4776129488287438
74	19.22593333333317	0.4776129488287438
75	19.22593333333317	0.4776129488287438
76	19.22593333333317	0.4776129488287438
77	19.22593333333317	0.4776129488287438
78	19.22593333333317	0.4776129488287438
79	19.22593333333317	0.4776129488287438
80	19.22593333333317	0.4776129488287438
81	19.22593333333317	0.4776129488287438
82	19.22593333333317	0.4776129488287438
83	19.22593333333317	0.4776129488287438
84	19.22593333333317	0.4776129488287438
85	19.22593333333317	0.4776129488287438
86	19.22593333333317	0.4776129488287438
87	19.22593333333317	0.4776129488287438
88	19.22593333333317	0.4776129488287438
89	19.22593333333317	0.4776129488287438
90	19.22593333333317	0.4776129488287438
91	19.22593333333317	0.4776129488287438
92	19.22593333333317	0.4776129488287438
93	19.22593333333317	0.4776129488287438
94	19.22593333333317	0.4776129488287438
95	19.22593333333317	0.4776129488287438
96	19.22593333333317	0.4776129488287438
97	19.22593333333317	0.4776129488287438
98	19.22593333333317	0.4776129488287438
99	19.22593333333317	0.4776129488287438
100	19.22593333333317	0.4776129488287438
101	19.22593333333317	0.4776129488287438
102	19.22593333333317	0.4776129488287438
103	19.22593333333317	0.4776129488287438
104	19.22593333333317	0.4776129488287438
105	19.22593333333317	0.4776129488287438
106	19.22593333333317	0.4776129488287438
107	19.22593333333317	0.4776129488287438
108	19.22593333333317	0.4776129488287438
109	19.22593333333317	0.4776129488287438
110	19.22593333333317	0.4776129488287438
111	19.22593333333317	0.4776129488287438
112	19.22593333333317	0.4776129488287438
113	19.22593333333317	0.4776129488287438
114	19.22593333333317	0.4776129488287438
115	19.22593333333317	0.4776129488287438
116	19.22593333333317	0.4776129488287438
117	19.22593333333317	0.4776129488287438
118	19.22593333333317	0.4776129488287438
119	19.22593333333317	0.4776129488287438
120	19.22593333333317	0.4776129488287438
121	19.22593333333317	0.4776129488287438
122	19.22593333333317	0.4776129488287438
123	19.22593333333317	0.4776129488287438
124	19.22593333333317	0.4776129488287438
125	19.22593333333317	0.4776129488287438
126	19.22593333333317	0.4776129488287438
127	19.22593333333317	0.4776129488287438
128	19.22593333333317	0.4776129488287438
129	19.22593333333317	0.4776129488287438
130	19.22593333333317	0.4776129488287438
131	19.22593333333317	0.4776129488287438
132	19.22593333333317	0.4776129488287438
133	19.22593333333317	0.4776129488287438
134	19.22593333333317	0.4776129488287438
135	19.22593333333317	0.4776129488287438
136	19.22593333333317	0.4776129488287438
137	19.22593333333317	0.4776129488287438
138	19.22593333333317	0.4776129488287438
139	19.22593333333317	0.4776129488287438
140	19.22593333333317	0.4776129488287438
141	19.22593333333317	0.4776129488287438
142	19.22593333333317	0.4776129488287438
143	19.22593333333317	0.4776129488287438
144	19.22593333333317	0.4776129488287438
145	19.22593333333317	0.4776129488287438
146	19.22593333333317	0.4776129488287438
147	19.22593333333317	0.4776129488287438
148	19.22593333333317	0.4776129488287438
149	19.22593333333317	0.4776129488287438
150	19.22593333333317	0.4776129488287438
151	19.22593333333317	0.4776129488287438
152	19.22593333333317	0.4776129488287438
153	19.22593333333317	0.4776129488287438
154	19.22593333333317	0.4776129488287438
155	19.22593333333317	0.4776129488287438
156	19.22593333333317	0.4776129488287438
157	19.22593333333317	0.4776129488287438
158	19.22593333333317	0.4776129488287438
159	19.22593333333317	0.4776129488287438
160	19.22593333333317	0.4776129488287438
161	19.22593333333317	0.4776129488287438
162	19.22593333333317	0.4776129488287438
163	19.22593333333317	0.4776129488287438
164	19.22593333333317	0.4776129488287438
165	19.22593333333317	0.4776129488287438
166	19.22593333333317	0.4776129488287438
167	19.22593333333317	0.4776129488287438
168	19.22593333333317	0.4776129488287438
169	19.22593333333317	0.4776129488287438
170	19.22593333333317	0.4776129488287438
171	19.22593333333317	0.4776129488287438
172	19.22593333333317	0.4776129488287438
173	19.22593333333317	0.4776129488287438
174	19.22593333333317	0.4776129488287438
175	19.22593333333317	0.4776129488287438
176	19.22593333333317	0.4776129488287438
177	19.22593333333317	0.4776129488287438
178	19.22593333333317	0.4776129488287438
179	19.22593333333317	0.4776129488287438
180	19.22593333333317	0.4776129488287438
181	19.22593333333317	0.4776129488287438
182	19.22593333333317	0.4776129488287438
183	19.22593333333317	0.4776129488287438
184	19.22593333333317	0.4776129488287438
185	19.22593333333317	0.4776129488287438
186	19.22593333333317	0.4776129488287438
187	19.22593333333317	0.4776129488287438
188	19.22593333333317	0.4776129488287438
189	19.22593333333317	0.4776129488287438
190	19.22593333333317	0.4776129488287438
191	19.22593333333317	0.4776129488287438
192	19.22593333333317	0.4776129488287438
193	19.22593333333317	0.4776129488287438
194	19.22593333333317	0.4776129488287438
195	19.22593333333317	0.4776129488287438
196	19.22593333333317	0.4776129488287438
197	19.22593333333317	0.4776129488287438
198	19.22593333333317	0.4776129488287438
199	19.22593333333317	0.4776129488287438
200	19.22593333333317	0.4776129488287438
201	19.22593333333317	0.4776129488287438
202	19.22593333333317	0.4776129488287438
203	19.22593333333317	0.4776129488287438
204	19.22593333333317	0.4776129488287438
205	19.22593333333317	0.4776129488287438
206	19.22593333333317	0.4776129488287438
207	19.22593333333317	0.4776129488287438
208	19.22593333333317	0.4776129488287438
209	19.22593333333317	0.4776129488287438
210	19.22593333333317	0.4776129488287438
211	19.22593333333317	0.4776129488287438
212	19.22593333333317	0.4776129488287438
213	19.22593333333317	0.4776129488287438
214	19.22593333333317	0.4776129488287438
215	19.22593333333317	0.4776129488287438
216	19.22593333333317	0.4776129488287438
217	19.22593333333317	0.4776129488287438
218	19.22593333333317	0.4776129488287438
219	19.22593333333317	0.4776129488287438
220	19.22593333333317	0.4776129488287438
221	19.22593333333317	0.4776129488287438
222	19.22593333333317	0.4776129488287438
223	19.22593333333317	0.4776129488287438
224	19.22593333333317	0.4776129488287438
225	19.22593333333317	0.4776129488287438
226	19.22593333333317	0.4776129488287438
227	19.22593333333317	0.4776129488287438
228	19.22593333333317	0.4776129488287438
229	19.22593333333317	0.4776129488287438
230	19.22593333333317	0.4776129488287438
231	19.22593333333317	0.4776129488287438
232	19.22593333333317	0.4776129488287438
233	19.22593333333317	0.4776129488287438
234	19.22593333333317	0.4776129488287438
235	19.22593333333317	0.4776129488287438
236	19.22593333333317	0.4776129488287438
237	19.22593333333317	0.4776129488287438
238	19.22593333333317	0.4776129488287438
239	19.22593333333317	0.4776129488287438
240	19.22593333333317	0.4776129488287438
241	19.22593333333317	0.4776129488287438
242	19.22593333333317	0.4776129488287438
243	19.22593333333317	0.4776129488287438
244	19.22593333333317	0.4776129488287438
245	19.22593333333317	0.4776129488287438
246	19.22593333333317	0.4776129488287438
247	19.22593333333317	0.4776129488287438
248	19.22593333333317	0.4776129488287438
249	19.22593333333317	0.4776129488287438
250	19.22593333333317	0.4776129488287438
251	19.22593333333317	0.4776129488287438
252	19.22593333333317	0.4776129488287438
253	19.22593333333317	0.4776129488287438
254	19.22593333333317	0.4776129488287438
255	19.22593333333317	0.4776129488287438
256	19.22593333333317	0.4776129488287438
257	19.22593333333317	0.4776129488287438
258	19.22593333333317	0.4776129488287438
259	19.22593333333317	0.4776129488287438
260	19.22593333333317	0.4776129488287438
261	19.22593333333317	0.4776129488287438
262	19.22593333333317	0.4776129488287438
263	19.22593333333317	0.4776129488287438
264	19.22593333333317	0.4776129488287438
265	19.22593333333317	0.4776129488287438
266	19.22593333333317	0.4776129488287438
267	19.22593333333317	0.4776129488287438
268	19.22593333333317	0.4776129488287438
269	19.22593333333317	0.4776129488287438
270	19.22593333333317	0.4776129488287438
271	19.22593333333317	0.4776129488287438
272	19.22593333333317	0.4776129488287438
273	19.22593333333317	0.4776129488287438
274	19.22593333333317	0.4776129488287438
275	19.22593333333317	0.4776129488287438
276	19.22593333333317	0.4776129488287438
277	19.22593333333317	0.4776129488287438
278	19.22593333333317	0.4776129488287438
279	19.22593333333317	0.4776129488287438
280	19.22593333333317	0.4776129488287438
281	19.22593333333317	0.4776129488287438
282	19.22593333333317	0.4776129488287438
283	19.22593333333317	0.4776129488287438
284	19.22593333333317	0.4776129488287438
285	19.22593333333317	0.4776129488287438
286	19.22593333333317	0.4776129488287438
287	19.22593333333317	0.4776129488287438
288	19.22593333333317	0.4776129488287438
289	19.22593333333317	0.4776129488287438
290	19.22593333333317	0.4776129488287438
291	19.22593333333317	0.4776129488287438
292	19.22593333333317	0.4776129488287438
293	19.22593333333317	0.4776129488287438
294	19.22593333333317	0.4776129488287438
295	19.22593333333317	0.4776129488287438
296	19.22593333333317	0.4776129488287438
297	19.22593333333317	0.4776129488287438
298	19.22593333333317	0.4776129488287438
299	19.22593333333317	0.4776129488287438


==> intercept_sim_files/intercept_mem1_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=1, N=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29999999999998495	1.509903313490213e-14
4	-0.39999999999999963	3.885780586188048e-16
5	3.258700000000034	7.8372217213753785
6	4.142199999999869	8.556138098464624
7	8.382399999999787	10.04118868660459
8	9.875100000000238	10.113725821377614
9	13.806599999999817	9.05095334426155
10	14.616633333333285	8.608538009764189
11	17.068166666666656	6.379252566371325
12	17.49939999999995	5.800029279236462
13	18.165133333333202	4.656017359169612
14	18.414366666666517	4.153159873183606
15	18.831066666666512	2.9399333658359152
16	18.92956666666652	2.574574879901954
17	19.041466666666523	2.0659397818480043
18	19.107533333333183	1.6901173279456587
19	19.14679999999984	1.414103871715222
20	19.166499999999843	1.2530314241869684
21	19.20629999999984	0.8244090671505128
22	19.206199999999843	0.8269955018015558
23	19.206099999999843	0.8295859147791915
24	19.20599999999984	0.8321802689321398
25	19.219299999999837	0.6199173412641474
26	19.219266666666506	0.6210867858484624
27	19.22593333333317	0.4776129488287438
28	19.22593333333317	0.4776129488287438
29	19.22593333333317	0.4776129488287438
30	19.22593333333317	0.4776129488287438
31	19.22593333333317	0.4776129488287438
32	19.22593333333317	0.4776129488287438
33	19.22593333333317	0.4776129488287438
34	19.22593333333317	0.4776129488287438
35	19.22593333333317	0.4776129488287438
36	19.22593333333317	0.4776129488287438
37	19.22593333333317	0.4776129488287438
38	19.22593333333317	0.4776129488287438
39	19.22593333333317	0.4776129488287438
40	19.22593333333317	0.4776129488287438
41	19.22593333333317	0.4776129488287438
42	19.22593333333317	0.4776129488287438
43	19.22593333333317	0.4776129488287438
44	19.22593333333317	0.4776129488287438
45	19.22593333333317	0.4776129488287438
46	19.22593333333317	0.4776129488287438
47	19.22593333333317	0.4776129488287438
48	19.22593333333317	0.4776129488287438
49	19.22593333333317	0.4776129488287438
50	19.22593333333317	0.4776129488287438
51	19.22593333333317	0.4776129488287438
52	19.22593333333317	0.4776129488287438
53	19.22593333333317	0.4776129488287438
54	19.22593333333317	0.4776129488287438
55	19.22593333333317	0.4776129488287438
56	19.22593333333317	0.4776129488287438
57	19.22593333333317	0.4776129488287438
58	19.22593333333317	0.4776129488287438
59	19.22593333333317	0.4776129488287438
60	19.22593333333317	0.4776129488287438
61	19.22593333333317	0.4776129488287438
62	19.22593333333317	0.4776129488287438
63	19.22593333333317	0.4776129488287438
64	19.22593333333317	0.4776129488287438
65	19.22593333333317	0.4776129488287438
66	19.22593333333317	0.4776129488287438
67	19.22593333333317	0.4776129488287438
68	19.22593333333317	0.4776129488287438
69	19.22593333333317	0.4776129488287438
70	19.22593333333317	0.4776129488287438
71	19.22593333333317	0.4776129488287438
72	19.22593333333317	0.4776129488287438
73	19.22593333333317	0.4776129488287438
74	19.22593333333317	0.4776129488287438
75	19.22593333333317	0.4776129488287438
76	19.22593333333317	0.4776129488287438
77	19.22593333333317	0.4776129488287438
78	19.22593333333317	0.4776129488287438
79	19.22593333333317	0.4776129488287438
80	19.22593333333317	0.4776129488287438
81	19.22593333333317	0.4776129488287438
82	19.22593333333317	0.4776129488287438
83	19.22593333333317	0.4776129488287438
84	19.22593333333317	0.4776129488287438
85	19.22593333333317	0.4776129488287438
86	19.22593333333317	0.4776129488287438
87	19.22593333333317	0.4776129488287438
88	19.22593333333317	0.4776129488287438
89	19.22593333333317	0.4776129488287438
90	19.22593333333317	0.4776129488287438
91	19.22593333333317	0.4776129488287438
92	19.22593333333317	0.4776129488287438
93	19.22593333333317	0.4776129488287438
94	19.22593333333317	0.4776129488287438
95	19.22593333333317	0.4776129488287438
96	19.22593333333317	0.4776129488287438
97	19.22593333333317	0.4776129488287438
98	19.22593333333317	0.4776129488287438
99	19.22593333333317	0.4776129488287438
100	19.22593333333317	0.4776129488287438
101	19.22593333333317	0.4776129488287438
102	19.22593333333317	0.4776129488287438
103	19.22593333333317	0.4776129488287438
104	19.22593333333317	0.4776129488287438
105	19.22593333333317	0.4776129488287438
106	19.22593333333317	0.4776129488287438
107	19.22593333333317	0.4776129488287438
108	19.22593333333317	0.4776129488287438
109	19.22593333333317	0.4776129488287438
110	19.22593333333317	0.4776129488287438
111	19.22593333333317	0.4776129488287438
112	19.22593333333317	0.4776129488287438
113	19.22593333333317	0.4776129488287438
114	19.22593333333317	0.4776129488287438
115	19.22593333333317	0.4776129488287438
116	19.22593333333317	0.4776129488287438
117	19.22593333333317	0.4776129488287438
118	19.22593333333317	0.4776129488287438
119	19.22593333333317	0.4776129488287438
120	19.22593333333317	0.4776129488287438
121	19.22593333333317	0.4776129488287438
122	19.22593333333317	0.4776129488287438
123	19.22593333333317	0.4776129488287438
124	19.22593333333317	0.4776129488287438
125	19.22593333333317	0.4776129488287438
126	19.22593333333317	0.4776129488287438
127	19.22593333333317	0.4776129488287438
128	19.22593333333317	0.4776129488287438
129	19.22593333333317	0.4776129488287438
130	19.22593333333317	0.4776129488287438
131	19.22593333333317	0.4776129488287438
132	19.22593333333317	0.4776129488287438
133	19.22593333333317	0.4776129488287438
134	19.22593333333317	0.4776129488287438
135	19.22593333333317	0.4776129488287438
136	19.22593333333317	0.4776129488287438
137	19.22593333333317	0.4776129488287438
138	19.22593333333317	0.4776129488287438
139	19.22593333333317	0.4776129488287438
140	19.22593333333317	0.4776129488287438
141	19.22593333333317	0.4776129488287438
142	19.22593333333317	0.4776129488287438
143	19.22593333333317	0.4776129488287438
144	19.22593333333317	0.4776129488287438
145	19.22593333333317	0.4776129488287438
146	19.22593333333317	0.4776129488287438
147	19.22593333333317	0.4776129488287438
148	19.22593333333317	0.4776129488287438
149	19.22593333333317	0.4776129488287438
150	19.22593333333317	0.4776129488287438
151	19.22593333333317	0.4776129488287438
152	19.22593333333317	0.4776129488287438
153	19.22593333333317	0.4776129488287438
154	19.22593333333317	0.4776129488287438
155	19.22593333333317	0.4776129488287438
156	19.22593333333317	0.4776129488287438
157	19.22593333333317	0.4776129488287438
158	19.22593333333317	0.4776129488287438
159	19.22593333333317	0.4776129488287438
160	19.22593333333317	0.4776129488287438
161	19.22593333333317	0.4776129488287438
162	19.22593333333317	0.4776129488287438
163	19.22593333333317	0.4776129488287438
164	19.22593333333317	0.4776129488287438
165	19.22593333333317	0.4776129488287438
166	19.22593333333317	0.4776129488287438
167	19.22593333333317	0.4776129488287438
168	19.22593333333317	0.4776129488287438
169	19.22593333333317	0.4776129488287438
170	19.22593333333317	0.4776129488287438
171	19.22593333333317	0.4776129488287438
172	19.22593333333317	0.4776129488287438
173	19.22593333333317	0.4776129488287438
174	19.22593333333317	0.4776129488287438
175	19.22593333333317	0.4776129488287438
176	19.22593333333317	0.4776129488287438
177	19.22593333333317	0.4776129488287438
178	19.22593333333317	0.4776129488287438
179	19.22593333333317	0.4776129488287438
180	19.22593333333317	0.4776129488287438
181	19.22593333333317	0.4776129488287438
182	19.22593333333317	0.4776129488287438
183	19.22593333333317	0.4776129488287438
184	19.22593333333317	0.4776129488287438
185	19.22593333333317	0.4776129488287438
186	19.22593333333317	0.4776129488287438
187	19.22593333333317	0.4776129488287438
188	19.22593333333317	0.4776129488287438
189	19.22593333333317	0.4776129488287438
190	19.22593333333317	0.4776129488287438
191	19.22593333333317	0.4776129488287438
192	19.22593333333317	0.4776129488287438
193	19.22593333333317	0.4776129488287438
194	19.22593333333317	0.4776129488287438
195	19.22593333333317	0.4776129488287438
196	19.22593333333317	0.4776129488287438
197	19.22593333333317	0.4776129488287438
198	19.22593333333317	0.4776129488287438
199	19.22593333333317	0.4776129488287438
200	19.22593333333317	0.4776129488287438
201	19.22593333333317	0.4776129488287438
202	19.22593333333317	0.4776129488287438
203	19.22593333333317	0.4776129488287438
204	19.22593333333317	0.4776129488287438
205	19.22593333333317	0.4776129488287438
206	19.22593333333317	0.4776129488287438
207	19.22593333333317	0.4776129488287438
208	19.22593333333317	0.4776129488287438
209	19.22593333333317	0.4776129488287438
210	19.22593333333317	0.4776129488287438
211	19.22593333333317	0.4776129488287438
212	19.22593333333317	0.4776129488287438
213	19.22593333333317	0.4776129488287438
214	19.22593333333317	0.4776129488287438
215	19.22593333333317	0.4776129488287438
216	19.22593333333317	0.4776129488287438
217	19.22593333333317	0.4776129488287438
218	19.22593333333317	0.4776129488287438
219	19.22593333333317	0.4776129488287438
220	19.22593333333317	0.4776129488287438
221	19.22593333333317	0.4776129488287438
222	19.22593333333317	0.4776129488287438
223	19.22593333333317	0.4776129488287438
224	19.22593333333317	0.4776129488287438
225	19.22593333333317	0.4776129488287438
226	19.22593333333317	0.4776129488287438
227	19.22593333333317	0.4776129488287438
228	19.22593333333317	0.4776129488287438
229	19.22593333333317	0.4776129488287438
230	19.22593333333317	0.4776129488287438
231	19.22593333333317	0.4776129488287438
232	19.22593333333317	0.4776129488287438
233	19.22593333333317	0.4776129488287438
234	19.22593333333317	0.4776129488287438
235	19.22593333333317	0.4776129488287438
236	19.22593333333317	0.4776129488287438
237	19.22593333333317	0.4776129488287438
238	19.22593333333317	0.4776129488287438
239	19.22593333333317	0.4776129488287438
240	19.22593333333317	0.4776129488287438
241	19.22593333333317	0.4776129488287438
242	19.22593333333317	0.4776129488287438
243	19.22593333333317	0.4776129488287438
244	19.22593333333317	0.4776129488287438
245	19.22593333333317	0.4776129488287438
246	19.22593333333317	0.4776129488287438
247	19.22593333333317	0.4776129488287438
248	19.22593333333317	0.4776129488287438
249	19.22593333333317	0.4776129488287438
250	19.22593333333317	0.4776129488287438
251	19.22593333333317	0.4776129488287438
252	19.22593333333317	0.4776129488287438
253	19.22593333333317	0.4776129488287438
254	19.22593333333317	0.4776129488287438
255	19.22593333333317	0.4776129488287438
256	19.22593333333317	0.4776129488287438
257	19.22593333333317	0.4776129488287438
258	19.22593333333317	0.4776129488287438
259	19.22593333333317	0.4776129488287438
260	19.22593333333317	0.4776129488287438
261	19.22593333333317	0.4776129488287438
262	19.22593333333317	0.4776129488287438
263	19.22593333333317	0.4776129488287438
264	19.22593333333317	0.4776129488287438
265	19.22593333333317	0.4776129488287438
266	19.22593333333317	0.4776129488287438
267	19.22593333333317	0.4776129488287438
268	19.22593333333317	0.4776129488287438
269	19.22593333333317	0.4776129488287438
270	19.22593333333317	0.4776129488287438
271	19.22593333333317	0.4776129488287438
272	19.22593333333317	0.4776129488287438
273	19.22593333333317	0.4776129488287438
274	19.22593333333317	0.4776129488287438
275	19.22593333333317	0.4776129488287438
276	19.22593333333317	0.4776129488287438
277	19.22593333333317	0.4776129488287438
278	19.22593333333317	0.4776129488287438
279	19.22593333333317	0.4776129488287438
280	19.22593333333317	0.4776129488287438
281	19.22593333333317	0.4776129488287438
282	19.22593333333317	0.4776129488287438
283	19.22593333333317	0.4776129488287438
284	19.22593333333317	0.4776129488287438
285	19.22593333333317	0.4776129488287438
286	19.22593333333317	0.4776129488287438
287	19.22593333333317	0.4776129488287438
288	19.22593333333317	0.4776129488287438
289	19.22593333333317	0.4776129488287438
290	19.22593333333317	0.4776129488287438
291	19.22593333333317	0.4776129488287438
292	19.22593333333317	0.4776129488287438
293	19.22593333333317	0.4776129488287438
294	19.22593333333317	0.4776129488287438
295	19.22593333333317	0.4776129488287438
296	19.22593333333317	0.4776129488287438
297	19.22593333333317	0.4776129488287438
298	19.22593333333317	0.4776129488287438
299	19.22593333333317	0.4776129488287438


==> intercept_sim_files/intercept_mem1_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29999999999998495	1.509903313490213e-14
4	-0.39999999999999963	3.885780586188048e-16
5	3.319000000000036	7.885248188865231
6	4.108999999999876	8.535808046108007
7	8.543799999999774	10.056040053619386
8	9.883200000000237	10.114628898778077
9	13.842299999999787	9.034982053662201
10	14.59899999999992	8.669119851519
11	17.245099999999944	6.151370253041248
12	17.684099999999916	5.520302273426617
13	18.27719999999982	4.430864493527175
14	18.41326666666648	4.165912944628313
15	18.817366666666484	3.0026480089339813
16	18.916033333333157	2.6451842277786484
17	19.00799999999983	2.249813918231146
18	19.013866666666473	2.2847467508578463
19	19.079999999999803	1.8779652108953677
20	19.10636666666647	1.794735671964588
21	19.12603333333314	1.822042516579179
22	19.132566666666477	1.6255633112520689
23	19.145799999999806	1.5315620653437487
24	19.14573333333314	1.5324974591242289
25	19.152366666666474	1.481891043753037
26	19.152333333333143	1.4823791312915906
27	19.158999999999807	1.4285326970940044
28	19.158999999999807	1.4285326970940044
29	19.158999999999807	1.4285326970940044
30	19.158999999999807	1.4285326970940044
31	19.158999999999807	1.4285326970940044
32	19.158999999999807	1.4285326970940044
33	19.158999999999807	1.4285326970940044
34	19.158999999999807	1.4285326970940044
35	19.158999999999807	1.4285326970940044
36	19.158999999999807	1.4285326970940044
37	19.158999999999807	1.4285326970940044
38	19.158999999999807	1.4285326970940044
39	19.158999999999807	1.4285326970940044
40	19.158999999999807	1.4285326970940044
41	19.158999999999807	1.4285326970940044
42	19.158999999999807	1.4285326970940044
43	19.158999999999807	1.4285326970940044
44	19.158999999999807	1.4285326970940044
45	19.158999999999807	1.4285326970940044
46	19.158999999999807	1.4285326970940044
47	19.158999999999807	1.4285326970940044
48	19.158999999999807	1.4285326970940044
49	19.158999999999807	1.4285326970940044
50	19.158999999999807	1.4285326970940044
51	19.158999999999807	1.4285326970940044
52	19.158999999999807	1.4285326970940044
53	19.158999999999807	1.4285326970940044
54	19.158999999999807	1.4285326970940044
55	19.158999999999807	1.4285326970940044
56	19.158999999999807	1.4285326970940044
57	19.158999999999807	1.4285326970940044
58	19.158999999999807	1.4285326970940044
59	19.158999999999807	1.4285326970940044
60	19.158999999999807	1.4285326970940044
61	19.158999999999807	1.4285326970940044
62	19.158999999999807	1.4285326970940044
63	19.158999999999807	1.4285326970940044
64	19.158999999999807	1.4285326970940044
65	19.158999999999807	1.4285326970940044
66	19.158999999999807	1.4285326970940044
67	19.158999999999807	1.4285326970940044
68	19.158999999999807	1.4285326970940044
69	19.158999999999807	1.4285326970940044
70	19.158999999999807	1.4285326970940044
71	19.158999999999807	1.4285326970940044
72	19.158999999999807	1.4285326970940044
73	19.158999999999807	1.4285326970940044
74	19.158999999999807	1.4285326970940044
75	19.158999999999807	1.4285326970940044
76	19.158999999999807	1.4285326970940044
77	19.158999999999807	1.4285326970940044
78	19.158999999999807	1.4285326970940044
79	19.158999999999807	1.4285326970940044
80	19.158999999999807	1.4285326970940044
81	19.158999999999807	1.4285326970940044
82	19.158999999999807	1.4285326970940044
83	19.158999999999807	1.4285326970940044
84	19.158999999999807	1.4285326970940044
85	19.158999999999807	1.4285326970940044
86	19.158999999999807	1.4285326970940044
87	19.158999999999807	1.4285326970940044
88	19.158999999999807	1.4285326970940044
89	19.158999999999807	1.4285326970940044
90	19.158999999999807	1.4285326970940044
91	19.158999999999807	1.4285326970940044
92	19.158999999999807	1.4285326970940044
93	19.158999999999807	1.4285326970940044
94	19.158999999999807	1.4285326970940044
95	19.158999999999807	1.4285326970940044
96	19.158999999999807	1.4285326970940044
97	19.158999999999807	1.4285326970940044
98	19.158999999999807	1.4285326970940044
99	19.158999999999807	1.4285326970940044
100	19.158999999999807	1.4285326970940044
101	19.158999999999807	1.4285326970940044
102	19.158999999999807	1.4285326970940044
103	19.158999999999807	1.4285326970940044
104	19.158999999999807	1.4285326970940044
105	19.158999999999807	1.4285326970940044
106	19.158999999999807	1.4285326970940044
107	19.158999999999807	1.4285326970940044
108	19.158999999999807	1.4285326970940044
109	19.158999999999807	1.4285326970940044
110	19.158999999999807	1.4285326970940044
111	19.158999999999807	1.4285326970940044
112	19.158999999999807	1.4285326970940044
113	19.158999999999807	1.4285326970940044
114	19.158999999999807	1.4285326970940044
115	19.158999999999807	1.4285326970940044
116	19.158999999999807	1.4285326970940044
117	19.158999999999807	1.4285326970940044
118	19.158999999999807	1.4285326970940044
119	19.158999999999807	1.4285326970940044
120	19.158999999999807	1.4285326970940044


==> intercept_sim_files/intercept_mem1_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29999999999998495	1.509903313490213e-14
4	-0.39999999999999963	3.885780586188048e-16
5	3.292200000000035	7.863996386062328
6	4.015066666666538	8.476149263013948
7	8.53683333333311	10.055209925152681
8	9.903000000000239	10.113066350024667
9	13.83526666666646	9.038251099017458
10	14.585233333333255	8.677477664172885
11	17.244699999999938	6.1512301135626775
12	17.68369999999991	5.520177923763002
13	18.24999999999982	4.487937165335638
14	18.385933333333146	4.2280628498428525
15	18.803299999999815	3.0480254444475996
16	18.901899999999824	2.697603823766538
17	19.00049999999982	2.2813175469451963
18	19.006333333333135	2.3160929505431893
19	19.085833333333134	1.838603447970452
20	19.112233333333133	1.7530184479602364
21	19.131933333333137	1.7805037476949066
22	19.138499999999805	1.5783898177150888
23	19.14506666666647	1.5315664080353149
24	19.1449999999998	1.5325017672637964
25	19.151633333333134	1.481898781593716
26	19.151599999999803	1.4823868500946062
27	19.158266666666467	1.4285441291359673
28	19.158266666666467	1.4285441291359673
29	19.158266666666467	1.4285441291359673
30	19.158266666666467	1.4285441291359673
31	19.158266666666467	1.4285441291359673
32	19.158266666666467	1.4285441291359673
33	19.158266666666467	1.4285441291359673
34	19.158266666666467	1.4285441291359673
35	19.158266666666467	1.4285441291359673
36	19.158266666666467	1.4285441291359673
37	19.158266666666467	1.4285441291359673
38	19.158266666666467	1.4285441291359673
39	19.158266666666467	1.4285441291359673
40	19.158266666666467	1.4285441291359673
41	19.158266666666467	1.4285441291359673
42	19.158266666666467	1.4285441291359673
43	19.158266666666467	1.4285441291359673
44	19.158266666666467	1.4285441291359673
45	19.158266666666467	1.4285441291359673
46	19.158266666666467	1.4285441291359673
47	19.158266666666467	1.4285441291359673
48	19.158266666666467	1.4285441291359673
49	19.158266666666467	1.4285441291359673
50	19.158266666666467	1.4285441291359673
51	19.158266666666467	1.4285441291359673
52	19.158266666666467	1.4285441291359673
53	19.158266666666467	1.4285441291359673
54	19.158266666666467	1.4285441291359673
55	19.158266666666467	1.4285441291359673
56	19.158266666666467	1.4285441291359673
57	19.158266666666467	1.4285441291359673
58	19.158266666666467	1.4285441291359673
59	19.158266666666467	1.4285441291359673
60	19.158266666666467	1.4285441291359673
61	19.158266666666467	1.4285441291359673
62	19.158266666666467	1.4285441291359673
63	19.158266666666467	1.4285441291359673
64	19.158266666666467	1.4285441291359673
65	19.158266666666467	1.4285441291359673
66	19.158266666666467	1.4285441291359673
67	19.158266666666467	1.4285441291359673
68	19.158266666666467	1.4285441291359673
69	19.158266666666467	1.4285441291359673
70	19.158266666666467	1.4285441291359673
71	19.158266666666467	1.4285441291359673
72	19.158266666666467	1.4285441291359673
73	19.158266666666467	1.4285441291359673
74	19.158266666666467	1.4285441291359673
75	19.158266666666467	1.4285441291359673
76	19.158266666666467	1.4285441291359673
77	19.158266666666467	1.4285441291359673
78	19.158266666666467	1.4285441291359673
79	19.158266666666467	1.4285441291359673
80	19.158266666666467	1.4285441291359673
81	19.158266666666467	1.4285441291359673
82	19.158266666666467	1.4285441291359673
83	19.158266666666467	1.4285441291359673
84	19.158266666666467	1.4285441291359673
85	19.158266666666467	1.4285441291359673
86	19.158266666666467	1.4285441291359673
87	19.158266666666467	1.4285441291359673
88	19.158266666666467	1.4285441291359673
89	19.158266666666467	1.4285441291359673
90	19.158266666666467	1.4285441291359673
91	19.158266666666467	1.4285441291359673
92	19.158266666666467	1.4285441291359673
93	19.158266666666467	1.4285441291359673
94	19.158266666666467	1.4285441291359673
95	19.158266666666467	1.4285441291359673
96	19.158266666666467	1.4285441291359673
97	19.158266666666467	1.4285441291359673
98	19.158266666666467	1.4285441291359673
99	19.158266666666467	1.4285441291359673
100	19.158266666666467	1.4285441291359673
101	19.158266666666467	1.4285441291359673
102	19.158266666666467	1.4285441291359673
103	19.158266666666467	1.4285441291359673
104	19.158266666666467	1.4285441291359673
105	19.158266666666467	1.4285441291359673
106	19.158266666666467	1.4285441291359673
107	19.158266666666467	1.4285441291359673
108	19.158266666666467	1.4285441291359673
109	19.158266666666467	1.4285441291359673
110	19.158266666666467	1.4285441291359673
111	19.158266666666467	1.4285441291359673
112	19.158266666666467	1.4285441291359673
113	19.158266666666467	1.4285441291359673
114	19.158266666666467	1.4285441291359673
115	19.158266666666467	1.4285441291359673
116	19.158266666666467	1.4285441291359673
117	19.158266666666467	1.4285441291359673
118	19.158266666666467	1.4285441291359673
119	19.158266666666467	1.4285441291359673
120	19.158266666666467	1.4285441291359673


==> maze_sim_files/maze_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	3.7050000000001178	13.73684734573422
3	6.963850000000168	17.960578169354452
4	9.514650000000007	20.321686701095892
5	14.15094999999996	23.129677021037192
6	19.046700000000435	24.81634016348912
7	24.732400000000418	25.433245963502035
8	30.084599999999675	24.797603772138775
9	34.54759999999983	23.31226167148952
10	38.56960000000008	21.02066520926479
11	41.349700000000055	18.80408226715675
12	43.510400000000296	16.471981721699336
13	44.900449999999985	14.606079378036377
14	46.04330000000018	12.716949127444037
15	46.71345000000016	11.437391490086373
16	47.43495000000013	9.712914263880785
17	47.832900000000194	8.548954765934777
18	47.98165000000014	8.11181781584741
19	48.13070000000017	7.6429416790918605
20	48.230050000000155	7.242144157464716
21	48.354600000000154	6.681981655167899
22	48.354400000000155	6.68349314655147
23	48.37920000000015	6.588322044344845
24	48.404050000000154	6.490888120858332
25	48.40395000000015	6.491671541097856
26	48.403850000000155	6.492456405514057
27	48.42875000000016	6.391900221178349
28	48.453700000000154	6.288835051899515
29	48.453700000000154	6.288835051899515
30	48.453700000000154	6.288835051899515
31	48.453700000000154	6.288835051899515
32	48.453700000000154	6.288835051899515
33	48.453700000000154	6.288835051899515
34	48.453700000000154	6.288835051899515
35	48.453700000000154	6.288835051899515
36	48.453700000000154	6.288835051899515
37	48.453700000000154	6.288835051899515
38	48.453700000000154	6.288835051899515
39	48.453700000000154	6.288835051899515
40	48.453700000000154	6.288835051899515
41	48.453700000000154	6.288835051899515
42	48.453700000000154	6.288835051899515
43	48.453700000000154	6.288835051899515
44	48.453700000000154	6.288835051899515
45	48.453700000000154	6.288835051899515
46	48.453700000000154	6.288835051899515
47	48.453700000000154	6.288835051899515
48	48.453700000000154	6.288835051899515
49	48.453700000000154	6.288835051899515
50	48.453700000000154	6.288835051899515
51	48.453700000000154	6.288835051899515
52	48.453700000000154	6.288835051899515
53	48.453700000000154	6.288835051899515
54	48.453700000000154	6.288835051899515
55	48.453700000000154	6.288835051899515
56	48.453700000000154	6.288835051899515
57	48.453700000000154	6.288835051899515
58	48.453700000000154	6.288835051899515
59	48.453700000000154	6.288835051899515
60	48.453700000000154	6.288835051899515
61	48.453700000000154	6.288835051899515
62	48.453700000000154	6.288835051899515
63	48.453700000000154	6.288835051899515
64	48.453700000000154	6.288835051899515
65	48.453700000000154	6.288835051899515
66	48.453700000000154	6.288835051899515
67	48.453700000000154	6.288835051899515
68	48.453700000000154	6.288835051899515
69	48.453700000000154	6.288835051899515
70	48.453700000000154	6.288835051899515
71	48.453700000000154	6.288835051899515
72	48.453700000000154	6.288835051899515
73	48.453700000000154	6.288835051899515
74	48.453700000000154	6.288835051899515
75	48.453700000000154	6.288835051899515
76	48.453700000000154	6.288835051899515
77	48.453700000000154	6.288835051899515
78	48.453700000000154	6.288835051899515
79	48.453700000000154	6.288835051899515
80	48.453700000000154	6.288835051899515
81	48.453700000000154	6.288835051899515
82	48.453700000000154	6.288835051899515
83	48.453700000000154	6.288835051899515
84	48.453700000000154	6.288835051899515
85	48.453700000000154	6.288835051899515
86	48.453700000000154	6.288835051899515
87	48.453700000000154	6.288835051899515
88	48.453700000000154	6.288835051899515
89	48.453700000000154	6.288835051899515
90	48.453700000000154	6.288835051899515
91	48.453700000000154	6.288835051899515
92	48.453700000000154	6.288835051899515
93	48.453700000000154	6.288835051899515
94	48.453700000000154	6.288835051899515
95	48.453700000000154	6.288835051899515
96	48.453700000000154	6.288835051899515
97	48.453700000000154	6.288835051899515
98	48.453700000000154	6.288835051899515
99	48.453700000000154	6.288835051899515


==> maze_sim_files/maze_mdp_fwd_gail.tex <==
% $\mathrm{GAIL}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.3799999999999913	7.737157100641051
3	0.5897500000000152	9.63990767266455
4	0.8518999999999751	11.400389747285057
5	1.3661499999999984	13.209312214400375
6	1.947800000000064	14.788899727836318
7	2.6717000000000897	16.374688672155074
8	3.6029499999999	17.80024680439847
9	4.581400000000165	19.177915529066272
10	5.6824000000000074	20.442996361590595
11	6.810899999999818	21.65222993573633
12	8.032099999999772	22.7696624830061
13	8.97100000000024	23.471452213273892
14	10.386999999999901	24.4487308668567
15	11.431349999999977	25.01565174400846
16	12.503150000000137	25.598979571019775
17	13.612299999999696	26.129133332546534
18	14.393950000000252	26.40624449628323
19	15.497299999999663	26.77263234555006
20	16.44299999999996	27.11161505701914
21	17.465800000000364	27.367312077732375
22	18.460849999999912	27.550821081729953
23	19.468149999999966	27.71836053191977
24	20.29769999999963	27.850195056946955
25	21.204099999999976	27.921815363439443
26	22.14245000000032	27.919759185879293
27	22.972850000000197	27.878236814359365
28	23.9199999999998	27.812761459445056
29	24.499149999999684	27.783360024977018
30	25.10459999999999	27.764407950467678
31	25.68635000000028	27.723104780624972
32	26.344400000000274	27.595850931616372
33	27.02884999999974	27.4906755587691
34	27.639799999999738	27.411403939966448
35	28.10704999999999	27.300546245405208
36	28.640300000000245	27.194121164509102
37	29.134700000000258	27.024010544513885
38	29.92014999999975	26.771937527521313
39	30.34234999999978	26.565755616535746
40	30.840450000000004	26.401879266398925
41	31.314600000000215	26.17115390730786
42	31.609800000000234	26.063295147774305
43	32.08069999999982	25.770581047194078
44	32.43259999999984	25.549561390364484
45	32.71025000000001	25.447820927095073
46	33.09350000000019	25.22880749758103
47	33.39755000000021	25.097000996085203
48	33.65229999999985	24.987484561475963
49	34.00759999999992	24.704137553049623
50	34.338650000000015	24.489579236432345
51	34.690400000000125	24.286773104716836
52	34.84795000000019	24.21112999836033
53	34.95589999999988	24.166609509610506
54	35.144099999999945	24.050498023741667
55	35.37770000000003	23.711997442434065
56	35.6418000000001	23.535113400194223
57	35.706450000000174	23.482075151006146
58	35.82124999999991	23.403392348920242
59	36.011299999999984	23.257846252609042
60	36.19675000000003	23.064303033855158
61	36.35765000000006	22.92856693030545
62	36.47395000000013	22.839612001903614
63	36.59049999999991	22.759697707790334
64	36.63229999999997	22.737595886768602
65	36.77420000000003	22.634649861661273
66	36.86640000000008	22.570132720921237
67	36.93380000000015	22.51385878875499
68	37.12634999999993	22.362560915009283
69	37.29430000000001	22.138355122050058
70	37.312600000000025	22.131800451838544
71	37.380950000000055	22.05837827442215
72	37.49945000000013	21.904832222537134
73	37.61819999999994	21.736882912690138
74	37.712199999999996	21.658444569266674
75	37.781400000000026	21.567208536108662
76	37.87575000000004	21.485752184587312
77	37.94530000000011	21.39178762773226
78	38.08999999999995	21.222898482535324
79	38.21000000000002	21.051577613091105
80	38.280250000000024	20.987520218870518
81	38.40065000000002	20.847006609523092
82	38.42130000000008	20.832071819912695
83	38.51699999999996	20.532320156280477
84	38.61290000000002	20.435358660664576
85	38.634000000000015	20.41815084673441
86	38.680150000000026	20.37338143209181
87	38.75140000000007	20.251013506488956
88	38.74779999999997	20.260245436815406
89	38.89420000000003	20.050847272871046
90	38.99090000000004	19.932186462854457
91	39.03780000000005	19.781446386955565
92	39.10980000000009	19.65001002442492
93	39.176950000000005	19.558416697102597
94	39.22430000000004	19.479243299214726
95	39.22175000000004	19.485870571711683
96	39.294200000000046	19.400499384294225
97	39.316800000000086	19.37586353585305
98	39.364450000000005	19.319698527603936
99	39.387200000000036	19.294260186905305


==> maze_sim_files/maze_mem10_fwd.tex <==
% $\mathrm{Opt. \ FSC \ on  \ POMDP, |n|=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.19500000000000528	5.64747509954657
3	0.11714999999999529	6.031351496762619
4	0.04959999999999746	6.539323347258633
5	0.0373	6.939696586306888
6	0.12519999999999556	7.656756164329514
7	0.043550000000002614	7.755149153788213
8	0.14694999999999286	8.366453292614366
9	0.07075000000000527	8.4611860538283
10	9.524599999999992	20.96454995557971
11	17.947550000000565	24.79170453997658
12	25.607500000000698	25.405909228956983
13	30.5028999999998	24.56195984831012
14	33.1931999999999	23.689321302224183
15	35.25900000000015	22.69956098694392
16	37.194000000000166	21.494604299683978
17	38.14295000000044	20.8765054618223
18	38.993849999999824	20.27455615241673
19	39.55650000000013	19.880957415325707
20	40.11035000000008	19.37387333182248
21	40.405350000000034	19.15164056621524
22	40.8810000000003	18.72861951666496
23	41.38269999999986	18.239088264219728
24	41.81545000000008	17.79510933648617
25	42.14410000000004	17.4717550689679
26	42.52344999999999	17.05889518982684
27	42.8836000000002	16.593304705211736
28	43.09949999999989	16.335484680596267
29	43.26085000000008	16.158933203571962
30	43.527550000000026	15.784442530463144
31	43.619799999999955	15.654697632340204
32	43.78725000000015	15.415667758404158
33	44.0050499999999	15.095179677549487
34	44.093300000000085	14.985626283542587
35	44.23680000000002	14.7789876432724
36	44.450599999999945	14.430770237239628
37	44.619900000000115	14.148925895275664
38	44.689549999999926	14.043462030336286
39	44.88435000000009	13.703170074019342
40	44.999550000000035	13.484293262811317
41	45.16999999999997	13.108532335849013
42	45.265800000000105	12.91842600164582
43	45.36179999999996	12.683827527997952
44	45.43300000000009	12.552089507328988
45	45.524350000000034	12.389127575317803
46	45.69094999999998	12.02405726439708
47	45.76295000000008	11.87775956557047
48	45.860099999999974	11.673134454378534
49	46.08245000000007	11.108750919770314
50	46.180250000000015	10.789570655846308
51	46.22824999999998	10.676957756659842
52	46.32635000000005	10.315298865156551
53	46.32464999999998	10.323940496607907
54	46.372950000000046	10.202335188450752
55	46.39635000000002	10.14456907303123
56	46.419799999999995	10.085928215092505
57	46.468300000000056	9.958454955965797
58	46.5169	9.828064122196215
59	46.54060000000004	9.765172381479001
60	46.53935000000002	9.77204260006575
61	46.5631	9.707973959071047
62	46.58690000000004	9.64290145080823
63	46.63575	9.503630723965427
64	46.659700000000036	9.435618999832494
65	46.67870000000002	9.397519689258468
66	46.727799999999995	9.25104897619716
67	46.80200000000002	8.994478083802301
68	46.82635	8.918607552611494
69	46.85075000000001	8.841439896165125
70	46.850200000000015	8.844899092697434
71	46.84965000000002	8.84836311853779
72	46.87410000000003	8.769369942589956
73	46.89860000000001	8.68899695246814
74	46.923150000000014	8.60720390588597
75	46.922750000000015	8.609846539718353
76	46.922350000000016	8.612492988531283
77	46.92195000000002	8.615143248809026
78	46.92155000000001	8.617797317035247
79	46.94615000000002	8.533496655972899
80	46.97080000000002	8.447666977337565
81	46.970500000000015	8.449739034431788
82	46.97020000000002	8.451814122423674
83	46.96990000000001	8.453892239081314
84	46.99460000000002	8.365666789921768
85	46.99435000000002	8.36744304297918
86	46.99410000000001	8.36922189871907
87	47.01885000000002	8.218173743448135
88	47.018650000000015	8.219530836823997
89	47.01845000000002	8.220890134133965
90	47.018250000000016	8.222251634284834
91	47.01805000000002	8.223615336182766
92	47.01785000000002	8.224981238732376
93	47.01765000000002	8.226349340837608
94	47.042450000000024	8.131658686731807
95	47.06730000000002	8.03511547583477
96	47.067200000000014	8.035820067671915
97	47.06710000000002	8.036525840809588
98	47.067000000000014	8.037232794936358
99	47.066900000000025	8.037940929740673


==> maze_sim_files/maze_mem10_trajsize5mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.01499999999999896	4.505971038522005
3	0.001550000000001051	5.212314514445539
4	1.4134999999999538	10.609046976519517
5	4.61595000000001	16.84351983991178
6	9.405449999999957	21.705349923405898
7	14.482899999999711	24.77896542614318
8	20.97804999999998	26.61980866192494
9	25.267599999999714	26.925061749975885
10	28.681750000000008	26.631436159875168
11	30.94830000000025	26.182802506798243
12	32.89510000000027	25.649048247254612
13	34.63634999999995	24.983192623792196
14	35.38644999999998	24.701974443301214
15	36.15835000000002	24.333137904460546
16	36.822150000000015	23.96846604139495
17	37.25750000000004	23.748855419788107
18	37.474149999999966	23.617498740923008
19	37.71654999999999	23.414389616163383
20	37.81449999999998	23.355563999826757
21	38.01794999999998	23.200983013603107
22	38.13699999999999	23.04618083327476
23	38.21129999999997	22.943101845870736
24	38.31074999999998	22.810466664176293
25	38.33539999999998	22.783058987765543
26	38.335099999999976	22.783860691068156
27	38.33479999999998	22.78466367888717
28	38.35949999999997	22.745773228228543
29	38.35924999999997	22.74644597376688
30	38.40899999999996	22.633891821779148
31	38.40384999999998	22.64450397287396
32	38.428749999999965	22.61535006223643
33	38.42869999999997	22.61548642656191
34	38.42864999999996	22.615623011040377
35	38.45359999999996	22.574887309574784
36	38.45359999999996	22.574887309574784
37	38.45359999999996	22.574887309574784
38	38.45359999999996	22.574887309574784
39	38.45359999999996	22.574887309574784
40	38.45359999999996	22.574887309574784
41	38.45359999999996	22.574887309574784
42	38.45359999999996	22.574887309574784
43	38.45359999999996	22.574887309574784
44	38.45359999999996	22.574887309574784
45	38.45359999999996	22.574887309574784
46	38.45359999999996	22.574887309574784
47	38.45359999999996	22.574887309574784
48	38.45359999999996	22.574887309574784
49	38.45359999999996	22.574887309574784
50	38.45359999999996	22.574887309574784
51	38.45359999999996	22.574887309574784
52	38.45359999999996	22.574887309574784
53	38.45359999999996	22.574887309574784
54	38.45359999999996	22.574887309574784
55	38.45359999999996	22.574887309574784
56	38.45359999999996	22.574887309574784
57	38.45359999999996	22.574887309574784
58	38.45359999999996	22.574887309574784
59	38.45359999999996	22.574887309574784
60	38.45359999999996	22.574887309574784
61	38.45359999999996	22.574887309574784
62	38.45359999999996	22.574887309574784
63	38.45359999999996	22.574887309574784
64	38.45359999999996	22.574887309574784
65	38.45359999999996	22.574887309574784
66	38.45359999999996	22.574887309574784
67	38.45359999999996	22.574887309574784
68	38.45359999999996	22.574887309574784
69	38.45359999999996	22.574887309574784
70	38.45359999999996	22.574887309574784
71	38.45359999999996	22.574887309574784
72	38.45359999999996	22.574887309574784
73	38.45359999999996	22.574887309574784
74	38.45359999999996	22.574887309574784
75	38.45359999999996	22.574887309574784
76	38.45359999999996	22.574887309574784
77	38.45359999999996	22.574887309574784
78	38.45359999999996	22.574887309574784
79	38.45359999999996	22.574887309574784
80	38.45359999999996	22.574887309574784
81	38.45359999999996	22.574887309574784
82	38.45359999999996	22.574887309574784
83	38.45359999999996	22.574887309574784
84	38.45359999999996	22.574887309574784
85	38.45359999999996	22.574887309574784
86	38.45359999999996	22.574887309574784
87	38.45359999999996	22.574887309574784
88	38.45359999999996	22.574887309574784
89	38.45359999999996	22.574887309574784
90	38.45359999999996	22.574887309574784
91	38.45359999999996	22.574887309574784
92	38.45359999999996	22.574887309574784
93	38.45359999999996	22.574887309574784
94	38.45359999999996	22.574887309574784
95	38.45359999999996	22.574887309574784
96	38.45359999999996	22.574887309574784
97	38.45359999999996	22.574887309574784
98	38.45359999999996	22.574887309574784
99	38.45359999999996	22.574887309574784


==> maze_sim_files/maze_mem10_trajsize5pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	-0.014999999999996443	4.5404597784806855
3	-0.04320000000000296	5.3794268988433975
4	0.6643999999999926	8.449606655933888
5	2.1187500000000004	12.116734850507298
6	4.481499999999828	15.89537661554453
7	7.164349999999758	18.881001670395804
8	9.902800000000303	21.137715395945758
9	12.34689999999973	22.67938602321456
10	15.061099999999982	23.973261705283246
11	17.761000000000443	24.870556869519344
12	20.401550000000153	25.406105813317865
13	22.9724999999998	25.662323038844526
14	25.413699999999583	25.64627053413408
15	27.569999999999997	25.417398962128505
16	29.720700000000377	24.991516390767455
17	31.53090000000044	24.466713820821887
18	32.91484999999973	23.99629272361661
19	34.32669999999983	23.412544439039593
20	35.74655000000006	22.66163758640363
21	37.274350000000126	21.727712881881903
22	38.275250000000284	21.002191372271135
23	39.15819999999977	20.326753374801388
24	39.91795000000003	19.67784217838681
25	40.58925	19.104452869357473
26	41.192099999999954	18.506949980750385
27	41.826250000000186	17.818490843432812
28	42.51174999999989	17.06180432830892
29	43.04365000000008	16.435431837268556
30	43.58675000000003	15.710702066982847
31	44.105950000000014	14.961166050729457
32	44.396200000000114	14.537870048944521
33	44.54209999999998	14.314999741180586
34	44.90830000000006	13.728836116364683
35	45.025250000000035	13.544528690120568
36	45.192450000000015	13.265622412744142
37	45.36005000000007	12.937181261677534
38	45.55805	12.484905894619269
39	45.68145000000005	12.243620416261733
40	45.80510000000003	11.994148322828082
41	45.80400000000003	11.99892803545384
42	45.87790000000006	11.782746351763649
43	45.926950000000026	11.679475959883634
44	46.02610000000004	11.463961304453216
45	46.05045000000005	11.411096783285076
46	46.07485000000005	11.357496752255734
47	46.099300000000056	11.303149539398348
48	46.09880000000004	11.305487099634368
49	46.14830000000005	11.169810074929654
50	46.19290000000005	11.079314039686732
51	46.192600000000056	11.080791724421161
52	46.19230000000006	11.082271911029814
53	46.21700000000005	11.001108625952192
54	46.21675000000006	11.002325864902385
55	46.24150000000006	10.942648571072738
56	46.24130000000005	10.943640816017298
57	46.24110000000007	10.94463479472933
58	46.24090000000005	10.945630506736439
59	46.240700000000054	10.94662795156567
60	46.24050000000006	10.947627128743413
61	46.240300000000055	10.94862803779542
62	46.26510000000006	10.886770962503034
63	46.289950000000054	10.824031781064757
64	46.28985000000006	10.824564285803847
65	46.289750000000055	10.825097687203598
66	46.28965000000006	10.825631985131409
67	46.28955000000006	10.826167179454597
68	46.31445000000006	10.761617266819185
69	46.31440000000005	10.761910733694085
70	46.314350000000054	10.762204656923235
71	46.31430000000005	10.762499036469219
72	46.31425000000006	10.762793872294525
73	46.314200000000056	10.76308916436168
74	46.314150000000055	10.763384912633164
75	46.31410000000006	10.763681117071455
76	46.31405000000005	10.763977777638726
77	46.31400000000006	10.76427489429737
78	46.313950000000055	10.76457246700957
79	46.313900000000054	10.764870495737533
80	46.31385000000006	10.765168980443356
81	46.31380000000006	10.765467921089188
82	46.313750000000056	10.765767317636975
83	46.33870000000005	10.67365412171479
84	46.33870000000005	10.67365412171479
85	46.33870000000005	10.67365412171479
86	46.33870000000005	10.67365412171479
87	46.33870000000005	10.67365412171479
88	46.33870000000005	10.67365412171479
89	46.33870000000005	10.67365412171479
90	46.33870000000005	10.67365412171479
91	46.33870000000005	10.67365412171479
92	46.33870000000005	10.67365412171479
93	46.33870000000005	10.67365412171479
94	46.33870000000005	10.67365412171479
95	46.33870000000005	10.67365412171479
96	46.33870000000005	10.67365412171479
97	46.33870000000005	10.67365412171479
98	46.33870000000005	10.67365412171479
99	46.33870000000005	10.67365412171479


==> maze_sim_files/maze_mem15_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ |n|=15, N=5}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.05499999999999883	4.783824306974564
3	0.03175000000000124	5.608664452211346
4	-0.025850000000002038	6.254420578878607
5	-0.06800000000000002	6.590391187175452
6	-0.1299500000000015	6.831957113265457
7	-0.20179999999999257	6.9307796646553586
8	-0.17360000000000572	7.367801099378175
9	-0.11014999999999382	7.944912332902024
10	-0.041350000000000046	8.478256611916082
11	0.012850000000002294	8.905086180240058
12	11.492349999999607	22.31509055499186
13	20.094999999999995	25.222018654342484
14	26.239999999999565	25.362435805734403
15	30.717399999999984	24.497686160941605
16	34.50385000000028	22.999991960378814
17	36.97795000000054	21.593192881033225
18	39.577049999999915	19.691674085701667
19	41.36140000000027	18.016226298534384
20	42.749350000000184	16.410755301859222
21	43.515100000000096	15.388496092536172
22	44.032400000000344	14.680040880052072
23	44.8757500000001	13.29119396207509
24	45.165800000000296	12.814232335961497
25	45.656450000000206	11.88477717071294
26	45.80315000000014	11.600630805154523
27	46.10015000000026	10.917062561765468
28	46.21275000000017	10.705653760396872
29	46.305600000000275	10.513702898598561
30	46.34870000000022	10.437516865136033
31	46.47190000000016	10.148854141724536
32	46.49035000000024	10.132761315529983
33	46.55885000000017	9.982721656817771
34	46.577550000000244	9.964626987373826
35	46.62630000000021	9.84468020354137
36	46.62515000000017	9.850996522053029
37	46.64900000000023	9.792851423359874
38	46.647900000000185	9.798970129049277
39	46.696800000000245	9.673816711102182
40	46.695800000000204	9.679515605648815
41	46.71980000000018	9.618375536440631
42	46.718850000000224	9.623866150227776
43	46.74290000000018	9.561543786962453
44	46.762000000000235	9.527749262024031
45	46.76120000000021	9.53252036766769
46	46.76040000000018	9.537297407546887
47	46.784600000000225	9.47247026070812
48	46.78385000000019	9.477024542413094
49	46.858100000000235	9.213704704949041
50	46.8575000000002	9.217457553468824
51	46.906900000000185	8.990696435204587
52	46.906400000000204	8.993813375871122
53	46.95590000000019	8.844305805997411
54	46.955500000000214	8.84689718206332
55	46.95510000000019	8.849492301256587
56	46.95470000000018	8.852091160285251
57	46.95430000000021	8.854693755856268
58	46.95390000000019	8.857300084675925
59	46.95350000000021	8.85991014344958
60	46.9531000000002	8.862523928881647
61	46.95270000000018	8.865141437676023
62	46.95230000000021	8.867762666535489
63	46.951900000000194	8.870387612162178
64	46.95150000000021	8.873016271257487
65	46.951100000000196	8.87564864052205
66	46.95070000000018	8.878284716655514
67	46.950300000000205	8.880924496357284
68	46.97490000000019	8.802253120082408
69	46.974550000000214	8.80462022449011
70	46.974200000000195	8.806990652884776
71	46.97385000000018	8.8093644025832
72	46.973500000000215	8.811741470901232
73	47.02315000000019	8.617362071858164
74	47.02290000000021	8.619113387698324
75	47.0226500000002	8.620867240452128
76	47.04740000000018	8.536269281132157
77	47.0472000000002	8.537726404611442
78	47.07200000000019	8.45131445397696
79	47.071850000000204	8.452466656396806
80	47.07170000000019	8.4536204735013
81	47.07155000000019	8.454775904629296
82	47.071400000000196	8.455932949119191
83	47.07125000000019	8.457091606308818
84	47.0711000000002	8.458251875535495
85	47.070950000000195	8.459413756135794
86	47.07080000000018	8.460577247445912
87	47.0706500000002	8.461742348801469
88	47.07050000000019	8.462909059537358
89	47.070350000000204	8.46407737898825
90	47.07020000000019	8.465247306487862
91	47.07005000000019	8.466418841369698
92	47.069900000000196	8.467591982966555
93	47.06975000000019	8.468766730610737
94	47.0696000000002	8.469943083634032
95	47.069450000000195	8.471121041367539
96	47.06930000000018	8.472300603141933
97	47.0691500000002	8.47348176828747
98	47.094000000000186	8.290106392562206
99	47.0939000000002	8.290793254568573


==> maze_sim_files/maze_mem1_fwd.tex <==
% $\mathrm{Opt. \ FSC \ on  \ POMDP, |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.4599999999999885	7.871746947152065
3	0.5501500000000233	9.439319889563055
4	0.6274000000000007	10.696481629021768
5	0.9562499999999988	12.118909643095035
6	1.5465500000000452	13.722617756736366
7	2.34365000000009	15.35550812176222
8	3.2528999999999098	16.907412326846252
9	3.8994000000001043	17.973580045166518
10	4.972600000000005	19.37577273917078
11	5.788399999999843	20.373906484520532
12	6.661149999999849	21.315355865607998
13	7.505900000000172	22.144929559382028
14	8.64755000000012	23.111325448738558
15	9.606749999999998	23.82175810970948
16	10.4030500000001	24.351146291242596
17	11.666199999999721	25.030844124000748
18	12.34715000000028	25.424858738594786
19	13.214699999999715	25.797040991362014
20	14.034199999999982	26.165068323243492
21	14.93055000000032	26.50595615512652
22	16.09884999999969	26.91571796697056
23	16.714650000000226	27.091552564913925
24	17.356799999999605	27.259395330051014
25	17.960349999999984	27.402975620860996
26	18.720350000000373	27.515845269180552
27	19.257050000000042	27.628124444078825
28	19.889949999999942	27.72210623306769
29	20.854349999999613	27.800095163101584
30	21.555850000000003	27.751579878945428
31	21.938850000000375	27.768145701099627
32	22.62270000000021	27.72489395308829
33	23.277999999999818	27.72558504342169
34	23.71469999999968	27.67052518312561
35	24.397350000000017	27.58659072769776
36	24.956450000000352	27.506893106956024
37	25.441750000000276	27.46913234773701
38	25.978099999999777	27.41115777179079
39	26.545649999999704	27.217780605286322
40	26.979400000000002	27.113298686069207
41	27.524150000000297	27.007002458205164
42	27.82505000000029	26.976844468868062
43	28.241649999999744	26.83686178146571
44	28.709149999999738	26.705428311066143
45	29.10765	26.58858319801004
46	29.417000000000254	26.465063215492314
47	29.912100000000283	26.311866212604606
48	30.47824999999974	26.058240192643353
49	30.925649999999784	25.87684287306909
50	31.229049999999987	25.721627108281783
51	31.433100000000202	25.65370313210166
52	31.677600000000258	25.528749836997424
53	32.03269999999974	25.341734169349976
54	32.338549999999806	25.121354439948114
55	32.62005	24.966202214143426
56	32.772150000000174	24.9152521435665
57	32.87960000000024	24.876692381423986
58	33.087299999999786	24.73051654757743
59	33.39544999999986	24.481215948099887
60	33.52924999999999	24.420589457207974
61	33.76335000000012	24.286856152608514
62	34.04295000000023	24.105396912258062
63	34.32819999999983	23.93876907361777
64	34.48904999999995	23.84906948074707
65	34.72525000000003	23.65271057273353
66	34.981950000000076	23.45325370172552
67	35.08920000000023	23.379190605322606
68	35.276699999999856	23.247057816205494
69	35.43460000000001	23.155197102162557
70	35.59785000000004	22.958972763986985
71	35.701450000000044	22.866603658993522
72	35.78530000000019	22.829845463997366
73	35.994349999999876	22.68296900931397
74	36.18385000000002	22.51905113848047
75	36.21375000000003	22.53365185533628
76	36.34880000000004	22.439588645070963
77	36.514150000000164	22.310622913255905
78	36.674849999999886	22.18937972268499
79	36.86590000000001	22.031185333295156
80	36.932350000000014	21.857016687496625
81	37.02395000000001	21.78377885945184
82	37.26075000000013	21.521409443563346
83	37.30309999999988	21.491103051960827
84	37.42055000000002	21.36411249496452
85	37.488250000000015	21.30747162235589
86	37.6811	21.112797133255462
87	37.799350000000125	21.001700278251256
88	37.892849999999896	20.83033710426937
89	37.98655000000001	20.716480253592774
90	38.05545000000001	20.627371386037023
91	38.07449999999999	20.615161162358124
92	38.18860000000009	20.423692615195773
93	38.25799999999991	20.354764208902097
94	38.30255000000002	20.31264553172474
95	38.4222	20.18503324644276
96	38.517099999999985	20.083511585128782
97	38.53720000000008	20.067242365606692
98	38.63234999999991	19.963018521193124
99	38.7027	19.88653294845533


==> maze_sim_files/maze_mem1_trajsize5mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	1.4500000000000162	12.011556934885682
3	2.1309499999999475	15.054121598336202
4	2.703150000000012	17.732356444576173
5	3.647300000000013	20.42001353354079
6	4.929599999999878	23.071720001768213
7	5.950149999999949	25.187779179147515
8	6.927350000000064	26.907703859257378
9	7.835100000000105	28.509072906532833
10	8.42335	29.717528998513636
11	9.086099999999933	30.73169970551575
12	9.762949999999863	31.669680015710394
13	10.153400000000078	32.442782994681366
14	10.416349999999971	33.17214777004199
15	10.60189999999998	33.665699998514675
16	10.869249999999997	34.166551763932894
17	11.068449999999881	34.548428467840736
18	11.334350000000056	35.00325492118542
19	11.567099999999936	35.35008299268908
20	11.786999999999969	35.61843189979032
21	11.783349999999999	35.985756734817905
22	11.990599999999906	36.19594399432065
23	12.108800000000018	36.372447162103285
24	12.287999999999933	36.61013201287327
25	12.278099999999961	36.82617928037071
26	12.25869999999999	37.09468202195566
27	12.365049999999918	37.26300502505801
28	12.547	37.346085082642766
29	12.719749999999934	37.36929976514813
30	12.878249999999959	37.39072922446821
31	12.947449999999987	37.5235509180234
32	12.917149999999934	37.636843131132856
33	12.90199999999999	37.81154051344649
34	12.94214999999994	37.90958254026936
35	13.097549999999963	37.784515598291094
36	13.07354999999999	37.88901061518365
37	13.104849999999947	37.928310685785696
38	13.091399999999986	38.02718719600494
39	13.13799999999995	38.01099651416678
40	13.209849999999964	38.00453457125213
41	13.20199999999998	38.12685491881021
42	13.194349999999952	38.242097132316
43	13.186849999999977	38.30192034451394
44	13.129599999999957	38.558154699622165
45	13.162349999999966	38.47947839404134
46	13.155199999999976	38.578452443818875
47	13.168099999999955	38.548760711467715
48	13.161199999999974	38.638008159841675
49	13.159349999999957	38.787231308479726
50	13.162699999999962	38.88875761335143
51	13.131099999999973	39.05316264772933
52	13.134499999999957	39.07098270775902
53	13.167949999999971	39.005296406994425
54	13.15649999999996	39.0534387442386
55	13.145099999999964	39.147403183225315
56	13.213899999999969	39.05773926880568
57	13.227849999999965	39.038186425313135
58	13.21184999999997	39.12004006359783
59	13.200899999999963	39.1896015441597
60	13.219949999999965	39.11935399514535
61	13.239049999999967	39.06532196331549
62	13.293199999999965	38.941508878830184
63	13.317549999999967	38.832708725988894
64	13.336949999999964	38.74969405940526
65	13.361399999999964	38.639670159565235
66	13.35089999999997	38.70957425741066
67	13.345399999999962	38.715521678520474
68	13.339949999999968	38.745982101341724
69	13.364499999999964	38.60955451374697
70	13.359099999999964	38.65406275141076
71	13.383699999999966	38.523360890633526
72	13.403349999999966	38.44072025570669
73	13.403049999999968	38.44259832136096
74	13.422749999999963	38.309859141446964
75	13.422549999999966	38.31114271980794
76	13.422349999999966	38.312426776145244
77	13.44214999999996	38.19679552498479
78	13.431999999999961	38.24908215892247
79	13.426899999999959	38.29508893304722
80	13.426799999999961	38.295862854360465
81	13.421699999999962	38.34315648339343
82	13.42159999999996	38.34394298243197
83	13.411499999999961	38.424635687927974
84	13.41139999999996	38.425447037607796
85	13.40629999999996	38.45967290955554
86	13.40119999999996	38.50947764589892
87	13.39609999999996	38.56054025542177
88	13.390999999999961	38.612855747794576
89	13.39089999999996	38.61371617948735
90	13.38579999999996	38.667291453630455
91	13.38569999999996	38.66816410834642
92	13.385599999999961	38.66903700171485
93	13.385499999999961	38.66991013372019
94	13.385399999999962	38.67078350434588
95	13.385299999999962	38.67165711357624
96	13.380199999999961	38.72653454622547
97	13.38009999999996	38.72742031158282
98	13.379999999999962	38.728306314632505
99	13.379899999999962	38.72919255535791


==> maze_sim_files/maze_mem1_trajsize5pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	1.1650000000000007	11.202087975016145
3	2.0049499999999543	14.237387418255294
4	2.8702500000000746	16.906714049084087
5	4.0655000000000125	19.204942065780987
6	5.640599999999847	21.518134483267808
7	6.685549999999828	23.114388726451473
8	8.10420000000016	24.768306610666656
9	9.716949999999958	26.268303669965288
10	11.45409999999997	27.703978111275102
11	12.480800000000187	28.558963065209504
12	13.650849999999737	29.490624260559848
13	14.899350000000195	30.226813338119488
14	16.440999999999676	30.887010845985156
15	17.45174999999996	31.45408029075874
16	18.405500000000256	31.872789174309904
17	19.331950000000013	32.21553265425715
18	20.445849999999883	32.513980112830005
19	21.282599999999736	32.64207633163062
20	21.916349999999976	32.81740677868202
21	22.641900000000195	33.06199017588029
22	23.204700000000106	33.32961427784612
23	23.8640499999999	33.331716616422604
24	24.65519999999984	33.29285092869039
25	24.998150000000006	33.47607879632114
26	25.522150000000167	33.49233963725886
27	26.002500000000154	33.49959094899512
28	26.514199999999903	33.35558346604066
29	26.84729999999989	33.34174654558446
30	27.166250000000016	33.21378683525106
31	27.43605000000012	33.18355248308262
32	27.62670000000011	33.17394078354276
33	27.737799999999936	33.279155655755496
34	27.809199999999933	33.33515809712023
35	28.135950000000026	33.28353365551061
36	28.373500000000117	33.179386488450895
37	28.62160000000012	33.0709778119728
38	28.765349999999973	32.99800106639024
39	28.974449999999983	32.89711404055836
40	29.059050000000045	32.948734999958525
41	29.308950000000113	32.70651746819741
42	29.43945000000012	32.527741524696964
43	29.56025000000001	32.34596582168309
44	29.691450000000014	32.236295412120356
45	29.783000000000055	32.1844614837658
46	29.949750000000087	31.976846310064694
47	30.021850000000104	31.86246565439491
48	30.114250000000023	31.79705712699685
49	30.221850000000035	31.456763304216473
50	30.234750000000055	31.38064463068751
51	30.277750000000072	31.308433687067296
52	30.26085000000008	31.396189136223175
53	30.308950000000028	31.32178530827236
54	30.34715000000003	31.32049539642521
55	30.445450000000047	31.179497258575275
56	30.488950000000067	31.04358311950309
57	30.572550000000074	30.757261443397287
58	30.611450000000048	30.650460419013275
59	30.610500000000048	30.65416773866154
60	30.60955000000006	30.657877679276748
61	30.658600000000064	30.642450229053154
62	30.672750000000065	30.52416047064198
63	30.67200000000005	30.527360776850617
64	30.671250000000047	30.530563185724162
65	30.670500000000057	30.53376769660095
66	30.719750000000065	30.278330947023786
67	30.714100000000066	30.31437070417252
68	30.738500000000055	30.19063973734245
69	30.73795000000005	30.192665910738942
70	30.73740000000006	30.194693759665707
71	30.736850000000064	30.196723283785232
72	30.736300000000064	30.198754482759803
73	30.735750000000056	30.200787356251254
74	30.76020000000005	30.08409988615247
75	30.80970000000006	29.888640081308456
76	30.80930000000006	29.88993967056474
77	30.803900000000063	29.91690700573838
78	30.803550000000058	29.917959696434828
79	30.803200000000054	29.919013515822908
80	30.80285000000006	29.920068463783608
81	30.82750000000006	29.901136161523997
82	30.877200000000062	29.71920439984901
83	30.877000000000066	29.719736893182684
84	30.901800000000062	29.708247790133946
85	30.901650000000064	29.708715762844754
86	30.926500000000065	29.62954484547476
87	30.926400000000065	29.629813415544945
88	30.926300000000065	29.630082320337895
89	30.926200000000062	29.630351559844833
90	30.926100000000066	29.630621134056604
91	30.95100000000006	29.618200131000517
92	30.950950000000063	29.618402878911212
93	30.950900000000065	29.61860579416259
94	30.950850000000063	29.61880887675101
95	30.95080000000006	29.61901212667295
96	30.950750000000063	29.619215543925165
97	30.95070000000006	29.61941912850421
98	30.950650000000063	29.61962288040649
99	30.950600000000065	29.61982679962858


==> maze_sim_files/maze_mem5_fwd.tex <==
% $\mathrm{Opt. \ FSC \ on  \ POMDP, |n|=5}$
x	y	err
0	0.0	0.0
1	-0.09999999999999647	3.5388358909926865e-15
2	0.10000000000000907	4.88978527135888
3	0.011949999999994278	5.183809622034727
4	-0.10590000000000288	5.372178812176595
5	-0.1635	5.622510804791646
6	1.4490000000000545	10.677874741726527
7	4.015050000000119	15.182790207912795
8	7.311500000000215	18.92277827777915
9	11.48979999999982	22.0434107152227
10	15.276649999999977	23.89352233927634
11	18.63635000000047	24.952876260613767
12	21.383000000000166	25.4482630252047
13	24.02549999999971	25.63457391395442
14	26.748599999999513	25.47697113159266
15	29.20229999999991	25.0860340570207
16	31.046000000000294	24.650777756492804
17	32.57360000000037	24.170549498097934
18	34.14934999999959	23.53487092757253
19	35.468499999999864	22.928724512061265
20	36.550549999999944	22.34852790895849
21	37.734949999999955	21.637615707316407
22	38.73695000000021	20.930646662191428
23	39.395999999999695	20.41213423432252
24	40.41654999999998	19.549691585738692
25	41.009299999999946	19.04327423291488
26	41.668299999999896	18.359571212585536
27	42.20865000000011	17.851333008419722
28	42.59014999999985	17.450618842250194
29	42.84245000000003	17.22931638218712
30	43.320299999999975	16.646490858736684
31	43.52914999999995	16.37890916018217
32	43.648450000000075	16.288041244959395
33	43.908049999999896	15.961037566445984
34	44.19320000000002	15.548059163767014
35	44.33395	15.378337764449698
36	44.514999999999986	15.165790945413947
37	44.69645000000006	14.989019727704033
38	44.86829999999995	14.838316451336457
39	45.01055	14.665829117288181
40	45.11809999999999	14.59416192831915
41	45.13589999999998	14.625213201522953
42	45.15375000000004	14.761301972979876
43	45.201749999999954	14.687136274219728
44	45.25985000000001	14.63935391257073
45	45.3031	14.615758974134712
46	45.28644999999999	14.754617629660876
47	45.33480000000002	14.677620684565959
48	45.34824999999996	14.707263067528825
49	45.39675	14.560185590764245
50	45.41534999999999	14.563370467632115
51	45.463999999999984	14.482510624888278
52	45.482750000000024	14.488331078405784
53	45.531549999999974	14.388288278926678
54	45.55545000000001	14.349447038039392
55	45.6294	14.023870922109934
56	45.72849999999998	13.418769606413306
57	45.75280000000001	13.373417370290912
58	45.802149999999976	13.011246303775085
59	45.8016	13.014236337180916
60	45.80104999999999	13.017229885713022
61	45.85049999999998	12.760633203332807
62	45.87505	12.709855722922272
63	45.87464999999999	12.712007409433737
64	45.94925	12.532084800124059
65	45.949	12.533608778001692
66	45.973749999999995	12.480045510233532
67	45.998549999999994	12.263779307273134
68	45.9984	12.264587536480803
69	45.99824999999999	12.265396933548462
70	45.9981	12.266207498244924
71	45.997949999999996	12.2670192303387
72	45.9978	12.267832129598188
73	45.99764999999999	12.268646195791083
74	46.022499999999994	12.129269712146733
75	46.0224	12.12971055878911
76	46.04729999999999	12.070992200726522
77	46.04724999999999	12.071214621466233
78	46.04719999999999	12.071437452101586
79	46.047149999999995	12.071660692609791
80	46.04709999999999	12.07188434296816
81	46.04705	12.072108403153932
82	46.04699999999999	12.072332873144289
83	46.04694999999999	12.07255775291632
84	46.046899999999994	12.072783042447178
85	46.04684999999999	12.07300874171395
86	46.0468	12.073234850693527
87	46.046749999999996	12.073461369362938
88	46.04669999999999	12.07368829769924
89	46.04664999999999	12.07391563567923
90	46.04659999999999	12.074143383279866
91	46.046549999999996	12.074371540477806
92	46.046499999999995	12.074600107249925
93	46.04644999999999	12.074829083572986
94	46.04639999999999	12.07505846942372
95	46.04634999999999	12.075288264778557
96	46.046299999999995	12.075518469614455
97	46.04624999999999	12.075749083907827
98	46.04619999999999	12.075980107635155
99	46.04615	12.07621154077308


==> obstacle_sim_files/obstacle_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-10.0	0.0
3	-3.385	75.70116759337272
4	107.03833333333333	219.25845524682305
5	103.295	221.4273424286151
6	99.55166666666666	223.59622983678383
7	95.80833333333334	225.7651174647858
8	92.065	227.9340053063609
9	88.32166666666667	230.10289335546122
10	84.57833333333333	232.27178160628105
11	81.67666666666666	234.8576280548589
12	90.23	242.58661085613238
13	125.165	257.35331959843853
14	220.24	264.02567880164315
15	340.69666666666666	214.55134891727337
16	415.90833333333336	124.8857475076952
17	444.7416666666667	24.17384807091226
18	444.7416666666667	24.17384807091226
19	444.7416666666667	24.17384807091226
20	444.7416666666667	24.17384807091226
21	444.7416666666667	24.17384807091226
22	444.7416666666667	24.17384807091226
23	444.7416666666667	24.17384807091226
24	444.7416666666667	24.17384807091226
25	444.7416666666667	24.17384807091226
26	444.7416666666667	24.17384807091226
27	444.7416666666667	24.17384807091226
28	444.7416666666667	24.17384807091226
29	444.7416666666667	24.17384807091226
30	444.7416666666667	24.17384807091226
31	444.7416666666667	24.17384807091226
32	444.7416666666667	24.17384807091226
33	444.7416666666667	24.17384807091226
34	444.7416666666667	24.17384807091226
35	444.7416666666667	24.17384807091226
36	444.7416666666667	24.17384807091226
37	444.7416666666667	24.17384807091226
38	444.7416666666667	24.17384807091226
39	444.7416666666667	24.17384807091226
40	444.7416666666667	24.17384807091226
41	444.7416666666667	24.17384807091226
42	444.7416666666667	24.17384807091226
43	444.7416666666667	24.17384807091226
44	444.7416666666667	24.17384807091226
45	444.7416666666667	24.17384807091226
46	444.7416666666667	24.17384807091226
47	444.7416666666667	24.17384807091226
48	444.7416666666667	24.17384807091226
49	444.7416666666667	24.17384807091226
50	444.7416666666667	24.17384807091226
51	444.7416666666667	24.17384807091226
52	444.7416666666667	24.17384807091226
53	444.7416666666667	24.17384807091226
54	444.7416666666667	24.17384807091226
55	444.7416666666667	24.17384807091226
56	444.7416666666667	24.17384807091226
57	444.7416666666667	24.17384807091226
58	444.7416666666667	24.17384807091226
59	444.7416666666667	24.17384807091226
60	444.7416666666667	24.17384807091226
61	444.7416666666667	24.17384807091226
62	444.7416666666667	24.17384807091226
63	444.7416666666667	24.17384807091226
64	444.7416666666667	24.17384807091226
65	444.7416666666667	24.17384807091226
66	444.7416666666667	24.17384807091226
67	444.7416666666667	24.17384807091226
68	444.7416666666667	24.17384807091226
69	444.7416666666667	24.17384807091226
70	444.7416666666667	24.17384807091226
71	444.7416666666667	24.17384807091226
72	444.7416666666667	24.17384807091226
73	444.7416666666667	24.17384807091226
74	444.7416666666667	24.17384807091226
75	444.7416666666667	24.17384807091226
76	444.7416666666667	24.17384807091226
77	444.7416666666667	24.17384807091226
78	444.7416666666667	24.17384807091226
79	444.7416666666667	24.17384807091226
80	444.7416666666667	24.17384807091226
81	444.7416666666667	24.17384807091226
82	444.7416666666667	24.17384807091226
83	444.7416666666667	24.17384807091226
84	444.7416666666667	24.17384807091226
85	444.7416666666667	24.17384807091226
86	444.7416666666667	24.17384807091226
87	444.7416666666667	24.17384807091226
88	444.7416666666667	24.17384807091226
89	444.7416666666667	24.17384807091226
90	444.7416666666667	24.17384807091226
91	444.7416666666667	24.17384807091226
92	444.7416666666667	24.17384807091226
93	444.7416666666667	24.17384807091226
94	444.7416666666667	24.17384807091226
95	444.7416666666667	24.17384807091226
96	444.7416666666667	24.17384807091226
97	444.7416666666667	24.17384807091226
98	444.7416666666667	24.17384807091226
99	444.7416666666667	24.17384807091226
100	444.7416666666667	24.17384807091226
101	444.7416666666667	24.17384807091226
102	444.7416666666667	24.17384807091226
103	444.7416666666667	24.17384807091226
104	444.7416666666667	24.17384807091226
105	444.7416666666667	24.17384807091226
106	444.7416666666667	24.17384807091226
107	444.7416666666667	24.17384807091226
108	444.7416666666667	24.17384807091226
109	444.7416666666667	24.17384807091226
110	444.7416666666667	24.17384807091226
111	444.7416666666667	24.17384807091226
112	444.7416666666667	24.17384807091226
113	444.7416666666667	24.17384807091226
114	444.7416666666667	24.17384807091226
115	444.7416666666667	24.17384807091226
116	444.7416666666667	24.17384807091226
117	444.7416666666667	24.17384807091226
118	444.7416666666667	24.17384807091226
119	444.7416666666667	24.17384807091226
120	444.7416666666667	24.17384807091226
121	444.7416666666667	24.17384807091226
122	444.7416666666667	24.17384807091226
123	444.7416666666667	24.17384807091226
124	444.7416666666667	24.17384807091226
125	444.7416666666667	24.17384807091226
126	444.7416666666667	24.17384807091226
127	444.7416666666667	24.17384807091226
128	444.7416666666667	24.17384807091226
129	444.7416666666667	24.17384807091226
130	444.7416666666667	24.17384807091226
131	444.7416666666667	24.17384807091226
132	444.7416666666667	24.17384807091226
133	444.7416666666667	24.17384807091226
134	444.7416666666667	24.17384807091226
135	444.7416666666667	24.17384807091226
136	444.7416666666667	24.17384807091226
137	444.7416666666667	24.17384807091226
138	444.7416666666667	24.17384807091226
139	444.7416666666667	24.17384807091226
140	444.7416666666667	24.17384807091226
141	444.7416666666667	24.17384807091226
142	444.7416666666667	24.17384807091226
143	444.7416666666667	24.17384807091226
144	444.7416666666667	24.17384807091226
145	444.7416666666667	24.17384807091226
146	444.7416666666667	24.17384807091226
147	444.7416666666667	24.17384807091226
148	444.7416666666667	24.17384807091226
149	444.7416666666667	24.17384807091226
150	444.7416666666667	24.17384807091226
151	444.7416666666667	24.17384807091226
152	444.7416666666667	24.17384807091226
153	444.7416666666667	24.17384807091226
154	444.7416666666667	24.17384807091226
155	444.7416666666667	24.17384807091226
156	444.7416666666667	24.17384807091226
157	444.7416666666667	24.17384807091226
158	444.7416666666667	24.17384807091226
159	444.7416666666667	24.17384807091226
160	444.7416666666667	24.17384807091226
161	444.7416666666667	24.17384807091226
162	444.7416666666667	24.17384807091226
163	444.7416666666667	24.17384807091226
164	444.7416666666667	24.17384807091226
165	444.7416666666667	24.17384807091226
166	444.7416666666667	24.17384807091226
167	444.7416666666667	24.17384807091226
168	444.7416666666667	24.17384807091226
169	444.7416666666667	24.17384807091226
170	444.7416666666667	24.17384807091226
171	444.7416666666667	24.17384807091226
172	444.7416666666667	24.17384807091226
173	444.7416666666667	24.17384807091226
174	444.7416666666667	24.17384807091226
175	444.7416666666667	24.17384807091226
176	444.7416666666667	24.17384807091226
177	444.7416666666667	24.17384807091226
178	444.7416666666667	24.17384807091226
179	444.7416666666667	24.17384807091226
180	444.7416666666667	24.17384807091226
181	444.7416666666667	24.17384807091226
182	444.7416666666667	24.17384807091226
183	444.7416666666667	24.17384807091226
184	444.7416666666667	24.17384807091226
185	444.7416666666667	24.17384807091226
186	444.7416666666667	24.17384807091226
187	444.7416666666667	24.17384807091226
188	444.7416666666667	24.17384807091226
189	444.7416666666667	24.17384807091226
190	444.7416666666667	24.17384807091226
191	444.7416666666667	24.17384807091226
192	444.7416666666667	24.17384807091226
193	444.7416666666667	24.17384807091226
194	444.7416666666667	24.17384807091226
195	444.7416666666667	24.17384807091226
196	444.7416666666667	24.17384807091226
197	444.7416666666667	24.17384807091226
198	444.7416666666667	24.17384807091226
199	444.7416666666667	24.17384807091226
200	444.7416666666667	24.17384807091226
201	444.7416666666667	24.17384807091226
202	444.7416666666667	24.17384807091226
203	444.7416666666667	24.17384807091226
204	444.7416666666667	24.17384807091226
205	444.7416666666667	24.17384807091226
206	444.7416666666667	24.17384807091226
207	444.7416666666667	24.17384807091226
208	444.7416666666667	24.17384807091226
209	444.7416666666667	24.17384807091226
210	444.7416666666667	24.17384807091226
211	444.7416666666667	24.17384807091226
212	444.7416666666667	24.17384807091226
213	444.7416666666667	24.17384807091226
214	444.7416666666667	24.17384807091226
215	444.7416666666667	24.17384807091226
216	444.7416666666667	24.17384807091226
217	444.7416666666667	24.17384807091226
218	444.7416666666667	24.17384807091226
219	444.7416666666667	24.17384807091226
220	444.7416666666667	24.17384807091226
221	444.7416666666667	24.17384807091226
222	444.7416666666667	24.17384807091226
223	444.7416666666667	24.17384807091226
224	444.7416666666667	24.17384807091226
225	444.7416666666667	24.17384807091226
226	444.7416666666667	24.17384807091226
227	444.7416666666667	24.17384807091226
228	444.7416666666667	24.17384807091226
229	444.7416666666667	24.17384807091226
230	444.7416666666667	24.17384807091226
231	444.7416666666667	24.17384807091226
232	444.7416666666667	24.17384807091226
233	444.7416666666667	24.17384807091226
234	444.7416666666667	24.17384807091226
235	444.7416666666667	24.17384807091226
236	444.7416666666667	24.17384807091226
237	444.7416666666667	24.17384807091226
238	444.7416666666667	24.17384807091226
239	444.7416666666667	24.17384807091226
240	444.7416666666667	24.17384807091226
241	444.7416666666667	24.17384807091226
242	444.7416666666667	24.17384807091226
243	444.7416666666667	24.17384807091226
244	444.7416666666667	24.17384807091226
245	444.7416666666667	24.17384807091226
246	444.7416666666667	24.17384807091226
247	444.7416666666667	24.17384807091226
248	444.7416666666667	24.17384807091226
249	444.7416666666667	24.17384807091226
250	444.7416666666667	24.17384807091226
251	444.7416666666667	24.17384807091226
252	444.7416666666667	24.17384807091226
253	444.7416666666667	24.17384807091226
254	444.7416666666667	24.17384807091226
255	444.7416666666667	24.17384807091226
256	444.7416666666667	24.17384807091226
257	444.7416666666667	24.17384807091226
258	444.7416666666667	24.17384807091226
259	444.7416666666667	24.17384807091226
260	444.7416666666667	24.17384807091226
261	444.7416666666667	24.17384807091226
262	444.7416666666667	24.17384807091226
263	444.7416666666667	24.17384807091226
264	444.7416666666667	24.17384807091226
265	444.7416666666667	24.17384807091226
266	444.7416666666667	24.17384807091226
267	444.7416666666667	24.17384807091226
268	444.7416666666667	24.17384807091226
269	444.7416666666667	24.17384807091226
270	444.7416666666667	24.17384807091226
271	444.7416666666667	24.17384807091226
272	444.7416666666667	24.17384807091226
273	444.7416666666667	24.17384807091226
274	444.7416666666667	24.17384807091226
275	444.7416666666667	24.17384807091226
276	444.7416666666667	24.17384807091226
277	444.7416666666667	24.17384807091226
278	444.7416666666667	24.17384807091226
279	444.7416666666667	24.17384807091226
280	444.7416666666667	24.17384807091226
281	444.7416666666667	24.17384807091226
282	444.7416666666667	24.17384807091226
283	444.7416666666667	24.17384807091226
284	444.7416666666667	24.17384807091226
285	444.7416666666667	24.17384807091226
286	444.7416666666667	24.17384807091226
287	444.7416666666667	24.17384807091226
288	444.7416666666667	24.17384807091226
289	444.7416666666667	24.17384807091226
290	444.7416666666667	24.17384807091226
291	444.7416666666667	24.17384807091226
292	444.7416666666667	24.17384807091226
293	444.7416666666667	24.17384807091226
294	444.7416666666667	24.17384807091226
295	444.7416666666667	24.17384807091226
296	444.7416666666667	24.17384807091226
297	444.7416666666667	24.17384807091226
298	444.7416666666667	24.17384807091226
299	444.7416666666667	24.17384807091226


==> obstacle_sim_files/obstacle_mem1_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-50.5	102.51707174905066
3	-46.74666666666667	107.34329270563744
4	-5.873333333333333	125.7223287867198
5	19.63	142.0115480046175
6	31.158333333333335	153.87998547749604
7	35.038333333333334	161.57662845810214
8	36.815	166.67612538993427
9	32.515	172.91871821272915
10	21.96	185.27616792237913
11	1.2583333333333333	209.24648526850004
12	-17.613333333333333	228.4517173399196
13	-28.218333333333334	246.34853493351002
14	-19.483333333333334	264.5065526388573
15	11.943333333333333	270.36174554761226
16	59.96	265.40942912162404
17	103.115	252.06729612347408
18	137.97166666666666	237.2741611102117
19	162.21666666666667	225.67189248011223
20	187.02166666666668	206.65382776652285
21	203.29833333333335	195.95529931736152
22	216.36166666666668	180.52987988295925
23	225.19666666666666	171.11398147303967
24	230.39166666666668	165.4445171768732
25	233.15333333333334	161.12404069191226
26	235.54333333333332	158.08590952038958
27	236.815	156.1344957880863
28	237.965	154.30457038489368
29	238.185	154.28960034623208
30	239.01333333333332	152.60562404082125
31	238.90833333333333	152.9809898774661
32	239.24	152.01794543188967
33	239.23833333333334	152.02563883729746
34	239.23666666666668	152.03338664765707
35	239.235	152.0411888546427
36	239.40166666666667	151.5313509824146
37	239.40166666666667	151.5313509824146
38	239.40166666666667	151.5313509824146
39	239.40166666666667	151.5313509824146
40	239.40166666666667	151.5313509824146
41	239.40166666666667	151.5313509824146
42	239.40166666666667	151.5313509824146
43	239.40166666666667	151.5313509824146
44	239.40166666666667	151.5313509824146
45	239.40166666666667	151.5313509824146
46	239.40166666666667	151.5313509824146
47	239.40166666666667	151.5313509824146
48	239.40166666666667	151.5313509824146
49	239.40166666666667	151.5313509824146
50	239.40166666666667	151.5313509824146
51	239.40166666666667	151.5313509824146
52	239.40166666666667	151.5313509824146
53	239.40166666666667	151.5313509824146
54	239.40166666666667	151.5313509824146
55	239.40166666666667	151.5313509824146
56	239.40166666666667	151.5313509824146
57	239.40166666666667	151.5313509824146
58	239.40166666666667	151.5313509824146
59	239.40166666666667	151.5313509824146
60	239.40166666666667	151.5313509824146
61	239.40166666666667	151.5313509824146
62	239.40166666666667	151.5313509824146
63	239.40166666666667	151.5313509824146
64	239.40166666666667	151.5313509824146
65	239.40166666666667	151.5313509824146
66	239.40166666666667	151.5313509824146
67	239.40166666666667	151.5313509824146
68	239.40166666666667	151.5313509824146
69	239.40166666666667	151.5313509824146
70	239.40166666666667	151.5313509824146
71	239.40166666666667	151.5313509824146
72	239.40166666666667	151.5313509824146
73	239.40166666666667	151.5313509824146
74	239.40166666666667	151.5313509824146
75	239.40166666666667	151.5313509824146
76	239.40166666666667	151.5313509824146
77	239.40166666666667	151.5313509824146
78	239.40166666666667	151.5313509824146
79	239.40166666666667	151.5313509824146
80	239.40166666666667	151.5313509824146
81	239.40166666666667	151.5313509824146
82	239.40166666666667	151.5313509824146
83	239.40166666666667	151.5313509824146
84	239.40166666666667	151.5313509824146
85	239.40166666666667	151.5313509824146
86	239.40166666666667	151.5313509824146
87	239.40166666666667	151.5313509824146
88	239.40166666666667	151.5313509824146
89	239.40166666666667	151.5313509824146
90	239.40166666666667	151.5313509824146
91	239.40166666666667	151.5313509824146
92	239.40166666666667	151.5313509824146
93	239.40166666666667	151.5313509824146
94	239.40166666666667	151.5313509824146
95	239.40166666666667	151.5313509824146
96	239.40166666666667	151.5313509824146
97	239.40166666666667	151.5313509824146
98	239.40166666666667	151.5313509824146
99	239.40166666666667	151.5313509824146
100	239.40166666666667	151.5313509824146
101	239.40166666666667	151.5313509824146
102	239.40166666666667	151.5313509824146
103	239.40166666666667	151.5313509824146
104	239.40166666666667	151.5313509824146
105	239.40166666666667	151.5313509824146
106	239.40166666666667	151.5313509824146
107	239.40166666666667	151.5313509824146
108	239.40166666666667	151.5313509824146
109	239.40166666666667	151.5313509824146
110	239.40166666666667	151.5313509824146
111	239.40166666666667	151.5313509824146
112	239.40166666666667	151.5313509824146
113	239.40166666666667	151.5313509824146
114	239.40166666666667	151.5313509824146
115	239.40166666666667	151.5313509824146
116	239.40166666666667	151.5313509824146
117	239.40166666666667	151.5313509824146
118	239.40166666666667	151.5313509824146
119	239.40166666666667	151.5313509824146
120	239.40166666666667	151.5313509824146
121	239.40166666666667	151.5313509824146
122	239.40166666666667	151.5313509824146
123	239.40166666666667	151.5313509824146
124	239.40166666666667	151.5313509824146
125	239.40166666666667	151.5313509824146
126	239.40166666666667	151.5313509824146
127	239.40166666666667	151.5313509824146
128	239.40166666666667	151.5313509824146
129	239.40166666666667	151.5313509824146
130	239.40166666666667	151.5313509824146
131	239.40166666666667	151.5313509824146
132	239.40166666666667	151.5313509824146
133	239.40166666666667	151.5313509824146
134	239.40166666666667	151.5313509824146
135	239.40166666666667	151.5313509824146
136	239.40166666666667	151.5313509824146
137	239.40166666666667	151.5313509824146
138	239.40166666666667	151.5313509824146
139	239.40166666666667	151.5313509824146
140	239.40166666666667	151.5313509824146
141	239.40166666666667	151.5313509824146
142	239.40166666666667	151.5313509824146
143	239.40166666666667	151.5313509824146
144	239.40166666666667	151.5313509824146
145	239.40166666666667	151.5313509824146
146	239.40166666666667	151.5313509824146
147	239.40166666666667	151.5313509824146
148	239.40166666666667	151.5313509824146
149	239.40166666666667	151.5313509824146
150	239.40166666666667	151.5313509824146
151	239.40166666666667	151.5313509824146
152	239.40166666666667	151.5313509824146
153	239.40166666666667	151.5313509824146
154	239.40166666666667	151.5313509824146
155	239.40166666666667	151.5313509824146
156	239.40166666666667	151.5313509824146
157	239.40166666666667	151.5313509824146
158	239.40166666666667	151.5313509824146
159	239.40166666666667	151.5313509824146
160	239.40166666666667	151.5313509824146
161	239.40166666666667	151.5313509824146
162	239.40166666666667	151.5313509824146
163	239.40166666666667	151.5313509824146
164	239.40166666666667	151.5313509824146
165	239.40166666666667	151.5313509824146
166	239.40166666666667	151.5313509824146
167	239.40166666666667	151.5313509824146
168	239.40166666666667	151.5313509824146
169	239.40166666666667	151.5313509824146
170	239.40166666666667	151.5313509824146
171	239.40166666666667	151.5313509824146
172	239.40166666666667	151.5313509824146
173	239.40166666666667	151.5313509824146
174	239.40166666666667	151.5313509824146
175	239.40166666666667	151.5313509824146
176	239.40166666666667	151.5313509824146
177	239.40166666666667	151.5313509824146
178	239.40166666666667	151.5313509824146
179	239.40166666666667	151.5313509824146
180	239.40166666666667	151.5313509824146
181	239.40166666666667	151.5313509824146
182	239.40166666666667	151.5313509824146
183	239.40166666666667	151.5313509824146
184	239.40166666666667	151.5313509824146
185	239.40166666666667	151.5313509824146
186	239.40166666666667	151.5313509824146
187	239.40166666666667	151.5313509824146
188	239.40166666666667	151.5313509824146
189	239.40166666666667	151.5313509824146
190	239.40166666666667	151.5313509824146
191	239.40166666666667	151.5313509824146
192	239.40166666666667	151.5313509824146
193	239.40166666666667	151.5313509824146
194	239.40166666666667	151.5313509824146
195	239.40166666666667	151.5313509824146
196	239.40166666666667	151.5313509824146
197	239.40166666666667	151.5313509824146
198	239.40166666666667	151.5313509824146
199	239.40166666666667	151.5313509824146
200	239.40166666666667	151.5313509824146
201	239.40166666666667	151.5313509824146
202	239.40166666666667	151.5313509824146
203	239.40166666666667	151.5313509824146
204	239.40166666666667	151.5313509824146
205	239.40166666666667	151.5313509824146
206	239.40166666666667	151.5313509824146
207	239.40166666666667	151.5313509824146
208	239.40166666666667	151.5313509824146
209	239.40166666666667	151.5313509824146
210	239.40166666666667	151.5313509824146
211	239.40166666666667	151.5313509824146
212	239.40166666666667	151.5313509824146
213	239.40166666666667	151.5313509824146
214	239.40166666666667	151.5313509824146
215	239.40166666666667	151.5313509824146
216	239.40166666666667	151.5313509824146
217	239.40166666666667	151.5313509824146
218	239.40166666666667	151.5313509824146
219	239.40166666666667	151.5313509824146
220	239.40166666666667	151.5313509824146
221	239.40166666666667	151.5313509824146
222	239.40166666666667	151.5313509824146
223	239.40166666666667	151.5313509824146
224	239.40166666666667	151.5313509824146
225	239.40166666666667	151.5313509824146
226	239.40166666666667	151.5313509824146
227	239.40166666666667	151.5313509824146
228	239.40166666666667	151.5313509824146
229	239.40166666666667	151.5313509824146
230	239.40166666666667	151.5313509824146
231	239.40166666666667	151.5313509824146
232	239.40166666666667	151.5313509824146
233	239.40166666666667	151.5313509824146
234	239.40166666666667	151.5313509824146
235	239.40166666666667	151.5313509824146
236	239.40166666666667	151.5313509824146
237	239.40166666666667	151.5313509824146
238	239.40166666666667	151.5313509824146
239	239.40166666666667	151.5313509824146
240	239.40166666666667	151.5313509824146
241	239.40166666666667	151.5313509824146
242	239.40166666666667	151.5313509824146
243	239.40166666666667	151.5313509824146
244	239.40166666666667	151.5313509824146
245	239.40166666666667	151.5313509824146
246	239.40166666666667	151.5313509824146
247	239.40166666666667	151.5313509824146
248	239.40166666666667	151.5313509824146
249	239.40166666666667	151.5313509824146
250	239.40166666666667	151.5313509824146
251	239.40166666666667	151.5313509824146
252	239.40166666666667	151.5313509824146
253	239.40166666666667	151.5313509824146
254	239.40166666666667	151.5313509824146
255	239.40166666666667	151.5313509824146
256	239.40166666666667	151.5313509824146
257	239.40166666666667	151.5313509824146
258	239.40166666666667	151.5313509824146
259	239.40166666666667	151.5313509824146
260	239.40166666666667	151.5313509824146
261	239.40166666666667	151.5313509824146
262	239.40166666666667	151.5313509824146
263	239.40166666666667	151.5313509824146
264	239.40166666666667	151.5313509824146
265	239.40166666666667	151.5313509824146
266	239.40166666666667	151.5313509824146
267	239.40166666666667	151.5313509824146
268	239.40166666666667	151.5313509824146
269	239.40166666666667	151.5313509824146
270	239.40166666666667	151.5313509824146
271	239.40166666666667	151.5313509824146
272	239.40166666666667	151.5313509824146
273	239.40166666666667	151.5313509824146
274	239.40166666666667	151.5313509824146
275	239.40166666666667	151.5313509824146
276	239.40166666666667	151.5313509824146
277	239.40166666666667	151.5313509824146
278	239.40166666666667	151.5313509824146
279	239.40166666666667	151.5313509824146
280	239.40166666666667	151.5313509824146
281	239.40166666666667	151.5313509824146
282	239.40166666666667	151.5313509824146
283	239.40166666666667	151.5313509824146
284	239.40166666666667	151.5313509824146
285	239.40166666666667	151.5313509824146
286	239.40166666666667	151.5313509824146
287	239.40166666666667	151.5313509824146
288	239.40166666666667	151.5313509824146
289	239.40166666666667	151.5313509824146
290	239.40166666666667	151.5313509824146
291	239.40166666666667	151.5313509824146
292	239.40166666666667	151.5313509824146
293	239.40166666666667	151.5313509824146
294	239.40166666666667	151.5313509824146
295	239.40166666666667	151.5313509824146
296	239.40166666666667	151.5313509824146
297	239.40166666666667	151.5313509824146
298	239.40166666666667	151.5313509824146
299	239.40166666666667	151.5313509824146


==> obstacle_sim_files/obstacle_mem1_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-40.0	90.0
3	-41.733333333333334	93.28716715366228
4	-26.836666666666666	112.49552578757095
5	-11.07	131.43720338372015
6	4.226666666666667	147.60341670240507
7	15.748333333333333	159.4209783264284
8	21.0	169.32616454641615
9	22.76	176.6571040179272
10	17.348333333333333	190.0843505672071
11	5.373333333333333	206.67291538940992
12	-6.86	223.0762359971691
13	-16.585	238.90401721542466
14	-22.43166666666667	253.13825997641788
15	-15.581666666666667	260.8989970541974
16	-1.4483333333333333	265.5904943025793
17	18.465	270.0375012999717
18	46.69166666666667	270.907911654905
19	70.16333333333333	266.8199580033073
20	96.565	264.11422864927414
21	118.41333333333333	258.7550305254395
22	139.19333333333333	251.8741073543597
23	159.02166666666668	243.51198026084253
24	173.61	237.60531258089952
25	188.05333333333334	231.3018456956663
26	202.65166666666667	224.42109303098414
27	214.375	217.09145778143062
28	224.37166666666667	210.03399771756492
29	232.455	205.24257511945763
30	241.635	198.41858559200918
31	249.06	191.9263740778389
32	256.2266666666667	185.3604918949972
33	262.9633333333333	177.5203800193717
34	267.58166666666665	172.2235272271344
35	270.565	168.9034905155417
36	272.975	166.56252392119748
37	275.84833333333336	163.20648066346985
38	277.405	161.35997327404286
39	279.65166666666664	158.11985010498307
40	281.585	154.8036264917595
41	281.68666666666667	154.76074595610174
42	282.63166666666666	153.39958495344396
43	283.41833333333335	152.228906575664
44	284.55	150.09257421116422
45	285.3566666666667	148.76129465989797
46	286.00333333333333	147.65797186591524
47	286.32	147.11466366975955
48	286.64	146.54593273100357
49	286.795	146.2730995147998
50	286.95166666666665	145.98818216059664
51	287.11	145.69098999823757
52	287.1016666666667	145.72213740731186
53	287.43	145.0595111210102
54	287.5933333333333	144.72430556828468
55	287.59	144.73720519157007
56	287.755	144.38323416634464
57	287.75333333333333	144.38981666154888
58	287.75166666666667	144.39645654893667
59	287.91833333333335	144.01756257677567
60	287.91833333333335	144.01756257677567
61	287.91833333333335	144.01756257677567
62	287.91833333333335	144.01756257677567
63	287.91833333333335	144.01756257677567
64	287.91833333333335	144.01756257677567
65	287.91833333333335	144.01756257677567
66	287.91833333333335	144.01756257677567
67	287.91833333333335	144.01756257677567
68	287.91833333333335	144.01756257677567
69	287.91833333333335	144.01756257677567
70	287.91833333333335	144.01756257677567
71	287.91833333333335	144.01756257677567
72	287.91833333333335	144.01756257677567
73	287.91833333333335	144.01756257677567
74	287.91833333333335	144.01756257677567
75	287.91833333333335	144.01756257677567
76	287.91833333333335	144.01756257677567
77	287.91833333333335	144.01756257677567
78	287.91833333333335	144.01756257677567
79	287.91833333333335	144.01756257677567
80	287.91833333333335	144.01756257677567
81	287.91833333333335	144.01756257677567
82	287.91833333333335	144.01756257677567
83	287.91833333333335	144.01756257677567
84	287.91833333333335	144.01756257677567
85	287.91833333333335	144.01756257677567
86	287.91833333333335	144.01756257677567
87	287.91833333333335	144.01756257677567
88	287.91833333333335	144.01756257677567
89	287.91833333333335	144.01756257677567
90	287.91833333333335	144.01756257677567
91	287.91833333333335	144.01756257677567
92	287.91833333333335	144.01756257677567
93	287.91833333333335	144.01756257677567
94	287.91833333333335	144.01756257677567
95	287.91833333333335	144.01756257677567
96	287.91833333333335	144.01756257677567
97	287.91833333333335	144.01756257677567
98	287.91833333333335	144.01756257677567
99	287.91833333333335	144.01756257677567
100	287.91833333333335	144.01756257677567
101	287.91833333333335	144.01756257677567
102	287.91833333333335	144.01756257677567
103	287.91833333333335	144.01756257677567
104	287.91833333333335	144.01756257677567
105	287.91833333333335	144.01756257677567
106	287.91833333333335	144.01756257677567
107	287.91833333333335	144.01756257677567
108	287.91833333333335	144.01756257677567
109	287.91833333333335	144.01756257677567
110	287.91833333333335	144.01756257677567
111	287.91833333333335	144.01756257677567
112	287.91833333333335	144.01756257677567
113	287.91833333333335	144.01756257677567
114	287.91833333333335	144.01756257677567
115	287.91833333333335	144.01756257677567
116	287.91833333333335	144.01756257677567
117	287.91833333333335	144.01756257677567
118	287.91833333333335	144.01756257677567
119	287.91833333333335	144.01756257677567
120	287.91833333333335	144.01756257677567
121	287.91833333333335	144.01756257677567
122	287.91833333333335	144.01756257677567
123	287.91833333333335	144.01756257677567
124	287.91833333333335	144.01756257677567
125	287.91833333333335	144.01756257677567
126	287.91833333333335	144.01756257677567
127	287.91833333333335	144.01756257677567
128	287.91833333333335	144.01756257677567
129	287.91833333333335	144.01756257677567
130	287.91833333333335	144.01756257677567
131	287.91833333333335	144.01756257677567
132	287.91833333333335	144.01756257677567
133	287.91833333333335	144.01756257677567
134	287.91833333333335	144.01756257677567
135	287.91833333333335	144.01756257677567
136	287.91833333333335	144.01756257677567
137	287.91833333333335	144.01756257677567
138	287.91833333333335	144.01756257677567
139	287.91833333333335	144.01756257677567
140	287.91833333333335	144.01756257677567
141	287.91833333333335	144.01756257677567
142	287.91833333333335	144.01756257677567
143	287.91833333333335	144.01756257677567
144	287.91833333333335	144.01756257677567
145	287.91833333333335	144.01756257677567
146	287.91833333333335	144.01756257677567
147	287.91833333333335	144.01756257677567
148	287.91833333333335	144.01756257677567
149	287.91833333333335	144.01756257677567
150	287.91833333333335	144.01756257677567
151	287.91833333333335	144.01756257677567
152	287.91833333333335	144.01756257677567
153	287.91833333333335	144.01756257677567
154	287.91833333333335	144.01756257677567
155	287.91833333333335	144.01756257677567
156	287.91833333333335	144.01756257677567
157	287.91833333333335	144.01756257677567
158	287.91833333333335	144.01756257677567
159	287.91833333333335	144.01756257677567
160	287.91833333333335	144.01756257677567
161	287.91833333333335	144.01756257677567
162	287.91833333333335	144.01756257677567
163	287.91833333333335	144.01756257677567
164	287.91833333333335	144.01756257677567
165	287.91833333333335	144.01756257677567
166	287.91833333333335	144.01756257677567
167	287.91833333333335	144.01756257677567
168	287.91833333333335	144.01756257677567
169	287.91833333333335	144.01756257677567
170	287.91833333333335	144.01756257677567
171	287.91833333333335	144.01756257677567
172	287.91833333333335	144.01756257677567
173	287.91833333333335	144.01756257677567
174	287.91833333333335	144.01756257677567
175	287.91833333333335	144.01756257677567
176	287.91833333333335	144.01756257677567
177	287.91833333333335	144.01756257677567
178	287.91833333333335	144.01756257677567
179	287.91833333333335	144.01756257677567
180	287.91833333333335	144.01756257677567
181	287.91833333333335	144.01756257677567
182	287.91833333333335	144.01756257677567
183	287.91833333333335	144.01756257677567
184	287.91833333333335	144.01756257677567
185	287.91833333333335	144.01756257677567
186	287.91833333333335	144.01756257677567
187	287.91833333333335	144.01756257677567
188	287.91833333333335	144.01756257677567
189	287.91833333333335	144.01756257677567
190	287.91833333333335	144.01756257677567
191	287.91833333333335	144.01756257677567
192	287.91833333333335	144.01756257677567
193	287.91833333333335	144.01756257677567
194	287.91833333333335	144.01756257677567
195	287.91833333333335	144.01756257677567
196	287.91833333333335	144.01756257677567
197	287.91833333333335	144.01756257677567
198	287.91833333333335	144.01756257677567
199	287.91833333333335	144.01756257677567
200	287.91833333333335	144.01756257677567
201	287.91833333333335	144.01756257677567
202	287.91833333333335	144.01756257677567
203	287.91833333333335	144.01756257677567
204	287.91833333333335	144.01756257677567
205	287.91833333333335	144.01756257677567
206	287.91833333333335	144.01756257677567
207	287.91833333333335	144.01756257677567
208	287.91833333333335	144.01756257677567
209	287.91833333333335	144.01756257677567
210	287.91833333333335	144.01756257677567
211	287.91833333333335	144.01756257677567
212	287.91833333333335	144.01756257677567
213	287.91833333333335	144.01756257677567
214	287.91833333333335	144.01756257677567
215	287.91833333333335	144.01756257677567
216	287.91833333333335	144.01756257677567
217	287.91833333333335	144.01756257677567
218	287.91833333333335	144.01756257677567
219	287.91833333333335	144.01756257677567
220	287.91833333333335	144.01756257677567
221	287.91833333333335	144.01756257677567
222	287.91833333333335	144.01756257677567
223	287.91833333333335	144.01756257677567
224	287.91833333333335	144.01756257677567
225	287.91833333333335	144.01756257677567
226	287.91833333333335	144.01756257677567
227	287.91833333333335	144.01756257677567
228	287.91833333333335	144.01756257677567
229	287.91833333333335	144.01756257677567
230	287.91833333333335	144.01756257677567
231	287.91833333333335	144.01756257677567
232	287.91833333333335	144.01756257677567
233	287.91833333333335	144.01756257677567
234	287.91833333333335	144.01756257677567
235	287.91833333333335	144.01756257677567
236	287.91833333333335	144.01756257677567
237	287.91833333333335	144.01756257677567
238	287.91833333333335	144.01756257677567
239	287.91833333333335	144.01756257677567
240	287.91833333333335	144.01756257677567
241	287.91833333333335	144.01756257677567
242	287.91833333333335	144.01756257677567
243	287.91833333333335	144.01756257677567
244	287.91833333333335	144.01756257677567
245	287.91833333333335	144.01756257677567
246	287.91833333333335	144.01756257677567
247	287.91833333333335	144.01756257677567
248	287.91833333333335	144.01756257677567
249	287.91833333333335	144.01756257677567
250	287.91833333333335	144.01756257677567
251	287.91833333333335	144.01756257677567
252	287.91833333333335	144.01756257677567
253	287.91833333333335	144.01756257677567
254	287.91833333333335	144.01756257677567
255	287.91833333333335	144.01756257677567
256	287.91833333333335	144.01756257677567
257	287.91833333333335	144.01756257677567
258	287.91833333333335	144.01756257677567
259	287.91833333333335	144.01756257677567
260	287.91833333333335	144.01756257677567
261	287.91833333333335	144.01756257677567
262	287.91833333333335	144.01756257677567
263	287.91833333333335	144.01756257677567
264	287.91833333333335	144.01756257677567
265	287.91833333333335	144.01756257677567
266	287.91833333333335	144.01756257677567
267	287.91833333333335	144.01756257677567
268	287.91833333333335	144.01756257677567
269	287.91833333333335	144.01756257677567
270	287.91833333333335	144.01756257677567
271	287.91833333333335	144.01756257677567
272	287.91833333333335	144.01756257677567
273	287.91833333333335	144.01756257677567
274	287.91833333333335	144.01756257677567
275	287.91833333333335	144.01756257677567
276	287.91833333333335	144.01756257677567
277	287.91833333333335	144.01756257677567
278	287.91833333333335	144.01756257677567
279	287.91833333333335	144.01756257677567
280	287.91833333333335	144.01756257677567
281	287.91833333333335	144.01756257677567
282	287.91833333333335	144.01756257677567
283	287.91833333333335	144.01756257677567
284	287.91833333333335	144.01756257677567
285	287.91833333333335	144.01756257677567
286	287.91833333333335	144.01756257677567
287	287.91833333333335	144.01756257677567
288	287.91833333333335	144.01756257677567
289	287.91833333333335	144.01756257677567
290	287.91833333333335	144.01756257677567
291	287.91833333333335	144.01756257677567
292	287.91833333333335	144.01756257677567
293	287.91833333333335	144.01756257677567
294	287.91833333333335	144.01756257677567
295	287.91833333333335	144.01756257677567
296	287.91833333333335	144.01756257677567
297	287.91833333333335	144.01756257677567
298	287.91833333333335	144.01756257677567
299	287.91833333333335	144.01756257677567


==> obstacle_sim_files/obstacle_mem5_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=10, N=10}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-10.2	7.743384273042546
3	-14.863333333333333	15.165684583588185
4	-18.008333333333333	32.61172995343319
5	-20.63	47.53458144691483
6	-23.565	57.465199106358206
7	-23.113333333333333	76.72878961351867
8	-19.341666666666665	100.85496978610392
9	-13.831666666666667	123.61698911242718
10	-6.891666666666667	147.62174613029143
11	-2.3633333333333333	168.81285887699212
12	4.716666666666667	190.87976945943709
13	13.18	208.12905675725716
14	24.14	220.90588584281355
15	39.535	232.73380811920515
16	68.625	243.18724139025056
17	103.37166666666667	253.61491188523797
18	141.59666666666666	257.80205712048905
19	176.36666666666667	260.0647974811032
20	212.88833333333332	253.9167826878595
21	246.22833333333332	244.3025778221684
22	274.565	231.18387870913492
23	299.7633333333333	215.44932270850882
24	323.10333333333335	196.5463541310858
25	340.79333333333335	178.1598176419763
26	355.3	159.52813753902035
27	366.185	142.30426595268884
28	374.48833333333334	126.92332277359023
29	380.015	115.00525252497563
30	384.75666666666666	103.15986358829431
31	388.36833333333334	92.73508503917027
32	389.66	88.66397840536335
33	391.1333333333333	83.60382101847279
34	391.4433333333333	82.53171181767401
35	391.75666666666666	81.40217516886258
36	391.905	80.88003034330146
37	392.56	78.26459224962413
38	392.885	76.91901655854271
39	392.87666666666667	76.98241003992766
40	393.205	75.54360534375691
41	393.2	75.5830227851035
42	393.195	75.62274993897861
43	393.52666666666664	74.06244632440638
44	393.525	74.07619528791591
45	393.5233333333333	74.09005413834039
46	393.69	73.25617539384149
47	393.69	73.25617539384149
48	393.69	73.25617539384149
49	393.69	73.25617539384149
50	393.69	73.25617539384149
51	393.69	73.25617539384149
52	393.69	73.25617539384149
53	393.69	73.25617539384149
54	393.69	73.25617539384149
55	393.69	73.25617539384149
56	393.69	73.25617539384149
57	393.69	73.25617539384149
58	393.69	73.25617539384149
59	393.69	73.25617539384149
60	393.69	73.25617539384149
61	393.69	73.25617539384149
62	393.69	73.25617539384149
63	393.69	73.25617539384149
64	393.69	73.25617539384149
65	393.69	73.25617539384149
66	393.69	73.25617539384149
67	393.69	73.25617539384149
68	393.69	73.25617539384149
69	393.69	73.25617539384149
70	393.69	73.25617539384149
71	393.69	73.25617539384149
72	393.69	73.25617539384149
73	393.69	73.25617539384149
74	393.69	73.25617539384149
75	393.69	73.25617539384149
76	393.69	73.25617539384149
77	393.69	73.25617539384149
78	393.69	73.25617539384149
79	393.69	73.25617539384149
80	393.69	73.25617539384149
81	393.69	73.25617539384149
82	393.69	73.25617539384149
83	393.69	73.25617539384149
84	393.69	73.25617539384149
85	393.69	73.25617539384149
86	393.69	73.25617539384149
87	393.69	73.25617539384149
88	393.69	73.25617539384149
89	393.69	73.25617539384149
90	393.69	73.25617539384149
91	393.69	73.25617539384149
92	393.69	73.25617539384149
93	393.69	73.25617539384149
94	393.69	73.25617539384149
95	393.69	73.25617539384149
96	393.69	73.25617539384149
97	393.69	73.25617539384149
98	393.69	73.25617539384149
99	393.69	73.25617539384149
100	393.69	73.25617539384149
101	393.69	73.25617539384149
102	393.69	73.25617539384149
103	393.69	73.25617539384149
104	393.69	73.25617539384149
105	393.69	73.25617539384149
106	393.69	73.25617539384149
107	393.69	73.25617539384149
108	393.69	73.25617539384149
109	393.69	73.25617539384149
110	393.69	73.25617539384149
111	393.69	73.25617539384149
112	393.69	73.25617539384149
113	393.69	73.25617539384149
114	393.69	73.25617539384149
115	393.69	73.25617539384149
116	393.69	73.25617539384149
117	393.69	73.25617539384149
118	393.69	73.25617539384149
119	393.69	73.25617539384149
120	393.69	73.25617539384149
121	393.69	73.25617539384149
122	393.69	73.25617539384149
123	393.69	73.25617539384149
124	393.69	73.25617539384149
125	393.69	73.25617539384149
126	393.69	73.25617539384149
127	393.69	73.25617539384149
128	393.69	73.25617539384149
129	393.69	73.25617539384149
130	393.69	73.25617539384149
131	393.69	73.25617539384149
132	393.69	73.25617539384149
133	393.69	73.25617539384149
134	393.69	73.25617539384149
135	393.69	73.25617539384149
136	393.69	73.25617539384149
137	393.69	73.25617539384149
138	393.69	73.25617539384149
139	393.69	73.25617539384149
140	393.69	73.25617539384149
141	393.69	73.25617539384149
142	393.69	73.25617539384149
143	393.69	73.25617539384149
144	393.69	73.25617539384149
145	393.69	73.25617539384149
146	393.69	73.25617539384149
147	393.69	73.25617539384149
148	393.69	73.25617539384149
149	393.69	73.25617539384149
150	393.69	73.25617539384149
151	393.69	73.25617539384149
152	393.69	73.25617539384149
153	393.69	73.25617539384149
154	393.69	73.25617539384149
155	393.69	73.25617539384149
156	393.69	73.25617539384149
157	393.69	73.25617539384149
158	393.69	73.25617539384149
159	393.69	73.25617539384149
160	393.69	73.25617539384149
161	393.69	73.25617539384149
162	393.69	73.25617539384149
163	393.69	73.25617539384149
164	393.69	73.25617539384149
165	393.69	73.25617539384149
166	393.69	73.25617539384149
167	393.69	73.25617539384149
168	393.69	73.25617539384149
169	393.69	73.25617539384149
170	393.69	73.25617539384149
171	393.69	73.25617539384149
172	393.69	73.25617539384149
173	393.69	73.25617539384149
174	393.69	73.25617539384149
175	393.69	73.25617539384149
176	393.69	73.25617539384149
177	393.69	73.25617539384149
178	393.69	73.25617539384149
179	393.69	73.25617539384149
180	393.69	73.25617539384149
181	393.69	73.25617539384149
182	393.69	73.25617539384149
183	393.69	73.25617539384149
184	393.69	73.25617539384149
185	393.69	73.25617539384149
186	393.69	73.25617539384149
187	393.69	73.25617539384149
188	393.69	73.25617539384149
189	393.69	73.25617539384149
190	393.69	73.25617539384149
191	393.69	73.25617539384149
192	393.69	73.25617539384149
193	393.69	73.25617539384149
194	393.69	73.25617539384149
195	393.69	73.25617539384149
196	393.69	73.25617539384149
197	393.69	73.25617539384149
198	393.69	73.25617539384149
199	393.69	73.25617539384149
200	393.69	73.25617539384149
201	393.69	73.25617539384149
202	393.69	73.25617539384149
203	393.69	73.25617539384149
204	393.69	73.25617539384149
205	393.69	73.25617539384149
206	393.69	73.25617539384149
207	393.69	73.25617539384149
208	393.69	73.25617539384149
209	393.69	73.25617539384149
210	393.69	73.25617539384149
211	393.69	73.25617539384149
212	393.69	73.25617539384149
213	393.69	73.25617539384149
214	393.69	73.25617539384149
215	393.69	73.25617539384149
216	393.69	73.25617539384149
217	393.69	73.25617539384149
218	393.69	73.25617539384149
219	393.69	73.25617539384149
220	393.69	73.25617539384149
221	393.69	73.25617539384149
222	393.69	73.25617539384149
223	393.69	73.25617539384149
224	393.69	73.25617539384149
225	393.69	73.25617539384149
226	393.69	73.25617539384149
227	393.69	73.25617539384149
228	393.69	73.25617539384149
229	393.69	73.25617539384149
230	393.69	73.25617539384149
231	393.69	73.25617539384149
232	393.69	73.25617539384149
233	393.69	73.25617539384149
234	393.69	73.25617539384149
235	393.69	73.25617539384149
236	393.69	73.25617539384149
237	393.69	73.25617539384149
238	393.69	73.25617539384149
239	393.69	73.25617539384149
240	393.69	73.25617539384149
241	393.69	73.25617539384149
242	393.69	73.25617539384149
243	393.69	73.25617539384149
244	393.69	73.25617539384149
245	393.69	73.25617539384149
246	393.69	73.25617539384149
247	393.69	73.25617539384149
248	393.69	73.25617539384149
249	393.69	73.25617539384149
250	393.69	73.25617539384149
251	393.69	73.25617539384149
252	393.69	73.25617539384149
253	393.69	73.25617539384149
254	393.69	73.25617539384149
255	393.69	73.25617539384149
256	393.69	73.25617539384149
257	393.69	73.25617539384149
258	393.69	73.25617539384149
259	393.69	73.25617539384149
260	393.69	73.25617539384149
261	393.69	73.25617539384149
262	393.69	73.25617539384149
263	393.69	73.25617539384149
264	393.69	73.25617539384149
265	393.69	73.25617539384149
266	393.69	73.25617539384149
267	393.69	73.25617539384149
268	393.69	73.25617539384149
269	393.69	73.25617539384149
270	393.69	73.25617539384149
271	393.69	73.25617539384149
272	393.69	73.25617539384149
273	393.69	73.25617539384149
274	393.69	73.25617539384149
275	393.69	73.25617539384149
276	393.69	73.25617539384149
277	393.69	73.25617539384149
278	393.69	73.25617539384149
279	393.69	73.25617539384149
280	393.69	73.25617539384149
281	393.69	73.25617539384149
282	393.69	73.25617539384149
283	393.69	73.25617539384149
284	393.69	73.25617539384149
285	393.69	73.25617539384149
286	393.69	73.25617539384149
287	393.69	73.25617539384149
288	393.69	73.25617539384149
289	393.69	73.25617539384149
290	393.69	73.25617539384149
291	393.69	73.25617539384149
292	393.69	73.25617539384149
293	393.69	73.25617539384149
294	393.69	73.25617539384149
295	393.69	73.25617539384149
296	393.69	73.25617539384149
297	393.69	73.25617539384149
298	393.69	73.25617539384149
299	393.69	73.25617539384149


==> obstacle_sim_files/obstacle_mem5_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-44.4	95.58577299995859
3	-40.47833333333333	103.64504907241192
4	-3.2383333333333333	129.36861364806774
5	22.231666666666666	147.16315661159302
6	35.105	157.97578076507222
7	40.92	167.1933619096926
8	40.115	174.47319309376132
9	37.04666666666667	182.76932954470809
10	25.231666666666666	197.93905963844946
11	5.963333333333333	218.537079970936
12	-12.33	238.2590769869401
13	-23.006666666666668	253.5071201279251
14	-17.648333333333333	269.3225971405924
15	13.193333333333333	276.5381576242657
16	61.031666666666666	275.3109345156628
17	110.03333333333333	260.66459717848574
18	145.10333333333332	242.54822061235998
19	172.98166666666665	227.28535954585536
20	193.31166666666667	212.58341389649658
21	213.3	193.15436831715854
22	223.445	185.0175405423308
23	230.27333333333334	177.4255016118642
24	237.71666666666667	169.48860253388372
25	240.19166666666666	166.6953956489361
26	242.63	163.15268850578803
27	244.38833333333332	160.5288163037682
28	245.63	159.32127844913452
29	246.315	158.26421718653594
30	246.97333333333333	156.73312547838066
31	246.965	156.75436338956138
32	247.125	156.60984230990508
33	247.355	156.64289208791703
34	247.52	156.154516211774
35	247.51833333333335	156.15899909138162
36	247.685	155.9746745735776
37	247.685	155.9746745735776
38	247.685	155.9746745735776
39	247.685	155.9746745735776
40	247.685	155.9746745735776
41	247.685	155.9746745735776
42	247.685	155.9746745735776
43	247.685	155.9746745735776
44	247.685	155.9746745735776
45	247.685	155.9746745735776
46	247.685	155.9746745735776
47	247.685	155.9746745735776
48	247.685	155.9746745735776
49	247.685	155.9746745735776
50	247.685	155.9746745735776
51	247.685	155.9746745735776
52	247.685	155.9746745735776
53	247.685	155.9746745735776
54	247.685	155.9746745735776
55	247.685	155.9746745735776
56	247.685	155.9746745735776
57	247.685	155.9746745735776
58	247.685	155.9746745735776
59	247.685	155.9746745735776
60	247.685	155.9746745735776
61	247.685	155.9746745735776
62	247.685	155.9746745735776
63	247.685	155.9746745735776
64	247.685	155.9746745735776
65	247.685	155.9746745735776
66	247.685	155.9746745735776
67	247.685	155.9746745735776
68	247.685	155.9746745735776
69	247.685	155.9746745735776
70	247.685	155.9746745735776
71	247.685	155.9746745735776
72	247.685	155.9746745735776
73	247.685	155.9746745735776
74	247.685	155.9746745735776
75	247.685	155.9746745735776
76	247.685	155.9746745735776
77	247.685	155.9746745735776
78	247.685	155.9746745735776
79	247.685	155.9746745735776
80	247.685	155.9746745735776
81	247.685	155.9746745735776
82	247.685	155.9746745735776
83	247.685	155.9746745735776
84	247.685	155.9746745735776
85	247.685	155.9746745735776
86	247.685	155.9746745735776
87	247.685	155.9746745735776
88	247.685	155.9746745735776
89	247.685	155.9746745735776
90	247.685	155.9746745735776
91	247.685	155.9746745735776
92	247.685	155.9746745735776
93	247.685	155.9746745735776
94	247.685	155.9746745735776
95	247.685	155.9746745735776
96	247.685	155.9746745735776
97	247.685	155.9746745735776
98	247.685	155.9746745735776
99	247.685	155.9746745735776
100	247.685	155.9746745735776
101	247.685	155.9746745735776
102	247.685	155.9746745735776
103	247.685	155.9746745735776
104	247.685	155.9746745735776
105	247.685	155.9746745735776
106	247.685	155.9746745735776
107	247.685	155.9746745735776
108	247.685	155.9746745735776
109	247.685	155.9746745735776
110	247.685	155.9746745735776
111	247.685	155.9746745735776
112	247.685	155.9746745735776
113	247.685	155.9746745735776
114	247.685	155.9746745735776
115	247.685	155.9746745735776
116	247.685	155.9746745735776
117	247.685	155.9746745735776
118	247.685	155.9746745735776
119	247.685	155.9746745735776
120	247.685	155.9746745735776
121	247.685	155.9746745735776
122	247.685	155.9746745735776
123	247.685	155.9746745735776
124	247.685	155.9746745735776
125	247.685	155.9746745735776
126	247.685	155.9746745735776
127	247.685	155.9746745735776
128	247.685	155.9746745735776
129	247.685	155.9746745735776
130	247.685	155.9746745735776
131	247.685	155.9746745735776
132	247.685	155.9746745735776
133	247.685	155.9746745735776
134	247.685	155.9746745735776
135	247.685	155.9746745735776
136	247.685	155.9746745735776
137	247.685	155.9746745735776
138	247.685	155.9746745735776
139	247.685	155.9746745735776
140	247.685	155.9746745735776
141	247.685	155.9746745735776
142	247.685	155.9746745735776
143	247.685	155.9746745735776
144	247.685	155.9746745735776
145	247.685	155.9746745735776
146	247.685	155.9746745735776
147	247.685	155.9746745735776
148	247.685	155.9746745735776
149	247.685	155.9746745735776
150	247.685	155.9746745735776
151	247.685	155.9746745735776
152	247.685	155.9746745735776
153	247.685	155.9746745735776
154	247.685	155.9746745735776
155	247.685	155.9746745735776
156	247.685	155.9746745735776
157	247.685	155.9746745735776
158	247.685	155.9746745735776
159	247.685	155.9746745735776
160	247.685	155.9746745735776
161	247.685	155.9746745735776
162	247.685	155.9746745735776
163	247.685	155.9746745735776
164	247.685	155.9746745735776
165	247.685	155.9746745735776
166	247.685	155.9746745735776
167	247.685	155.9746745735776
168	247.685	155.9746745735776
169	247.685	155.9746745735776
170	247.685	155.9746745735776
171	247.685	155.9746745735776
172	247.685	155.9746745735776
173	247.685	155.9746745735776
174	247.685	155.9746745735776
175	247.685	155.9746745735776
176	247.685	155.9746745735776
177	247.685	155.9746745735776
178	247.685	155.9746745735776
179	247.685	155.9746745735776
180	247.685	155.9746745735776
181	247.685	155.9746745735776
182	247.685	155.9746745735776
183	247.685	155.9746745735776
184	247.685	155.9746745735776
185	247.685	155.9746745735776
186	247.685	155.9746745735776
187	247.685	155.9746745735776
188	247.685	155.9746745735776
189	247.685	155.9746745735776
190	247.685	155.9746745735776
191	247.685	155.9746745735776
192	247.685	155.9746745735776
193	247.685	155.9746745735776
194	247.685	155.9746745735776
195	247.685	155.9746745735776
196	247.685	155.9746745735776
197	247.685	155.9746745735776
198	247.685	155.9746745735776
199	247.685	155.9746745735776
200	247.685	155.9746745735776
201	247.685	155.9746745735776
202	247.685	155.9746745735776
203	247.685	155.9746745735776
204	247.685	155.9746745735776
205	247.685	155.9746745735776
206	247.685	155.9746745735776
207	247.685	155.9746745735776
208	247.685	155.9746745735776
209	247.685	155.9746745735776
210	247.685	155.9746745735776
211	247.685	155.9746745735776
212	247.685	155.9746745735776
213	247.685	155.9746745735776
214	247.685	155.9746745735776
215	247.685	155.9746745735776
216	247.685	155.9746745735776
217	247.685	155.9746745735776
218	247.685	155.9746745735776
219	247.685	155.9746745735776
220	247.685	155.9746745735776
221	247.685	155.9746745735776
222	247.685	155.9746745735776
223	247.685	155.9746745735776
224	247.685	155.9746745735776
225	247.685	155.9746745735776
226	247.685	155.9746745735776
227	247.685	155.9746745735776
228	247.685	155.9746745735776
229	247.685	155.9746745735776
230	247.685	155.9746745735776
231	247.685	155.9746745735776
232	247.685	155.9746745735776
233	247.685	155.9746745735776
234	247.685	155.9746745735776
235	247.685	155.9746745735776
236	247.685	155.9746745735776
237	247.685	155.9746745735776
238	247.685	155.9746745735776
239	247.685	155.9746745735776
240	247.685	155.9746745735776
241	247.685	155.9746745735776
242	247.685	155.9746745735776
243	247.685	155.9746745735776
244	247.685	155.9746745735776
245	247.685	155.9746745735776
246	247.685	155.9746745735776
247	247.685	155.9746745735776
248	247.685	155.9746745735776
249	247.685	155.9746745735776
250	247.685	155.9746745735776
251	247.685	155.9746745735776
252	247.685	155.9746745735776
253	247.685	155.9746745735776
254	247.685	155.9746745735776
255	247.685	155.9746745735776
256	247.685	155.9746745735776
257	247.685	155.9746745735776
258	247.685	155.9746745735776
259	247.685	155.9746745735776
260	247.685	155.9746745735776
261	247.685	155.9746745735776
262	247.685	155.9746745735776
263	247.685	155.9746745735776
264	247.685	155.9746745735776
265	247.685	155.9746745735776
266	247.685	155.9746745735776
267	247.685	155.9746745735776
268	247.685	155.9746745735776
269	247.685	155.9746745735776
270	247.685	155.9746745735776
271	247.685	155.9746745735776
272	247.685	155.9746745735776
273	247.685	155.9746745735776
274	247.685	155.9746745735776
275	247.685	155.9746745735776
276	247.685	155.9746745735776
277	247.685	155.9746745735776
278	247.685	155.9746745735776
279	247.685	155.9746745735776
280	247.685	155.9746745735776
281	247.685	155.9746745735776
282	247.685	155.9746745735776
283	247.685	155.9746745735776
284	247.685	155.9746745735776
285	247.685	155.9746745735776
286	247.685	155.9746745735776
287	247.685	155.9746745735776
288	247.685	155.9746745735776
289	247.685	155.9746745735776
290	247.685	155.9746745735776
291	247.685	155.9746745735776
292	247.685	155.9746745735776
293	247.685	155.9746745735776
294	247.685	155.9746745735776
295	247.685	155.9746745735776
296	247.685	155.9746745735776
297	247.685	155.9746745735776
298	247.685	155.9746745735776
299	247.685	155.9746745735776


==> obstacle_sim_files/obstacle_mem5_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-5.0	0.0
2	-35.3	83.36612021678751
3	-35.955	90.5158161593881
4	-23.503333333333334	110.77677248513098
5	-9.6	127.61892492886375
6	2.3	140.93719641504353
7	12.411666666666667	153.2196969405546
8	19.47	162.85792100273213
9	23.016666666666666	172.1405909585382
10	17.375	185.13027226343436
11	7.383333333333334	201.85816734089147
12	-5.578333333333333	217.34467372636843
13	-18.553333333333335	234.1021297544205
14	-22.541666666666668	246.92171147394922
15	-14.593333333333334	257.9308394813528
16	1.955	263.73876527415587
17	27.425	264.51643498089504
18	50.49166666666667	266.82797191677605
19	76.90666666666667	265.04558970528586
20	102.385	261.25084390613506
21	124.34666666666666	258.2759309128342
22	146.24833333333333	251.9734443624757
23	162.935	246.69896116860056
24	179.94333333333333	240.45470146278177
25	197.30833333333334	232.9464815443422
26	212.40166666666667	224.30679956379873
27	226.07333333333332	215.61972224780695
28	239.14833333333334	206.02459318543183
29	250.07166666666666	197.6109052251137
30	258.51666666666665	190.64259681986525
31	266.545	182.49088006893118
32	270.9533333333333	177.2300515024342
33	275.57666666666665	171.83698900088052
34	278.565	168.4490005164765
35	281.9216666666667	164.3385191118898
36	283.79833333333335	161.84024323559217
37	286.36833333333334	158.55141962117196
38	288.2916666666667	155.9648676162544
39	289.225	154.7084064996696
40	290.505	152.8508095333477
41	291.29333333333335	151.35480596561487
42	292.09	150.11905908311496
43	292.895	148.81373360121435
44	293.37166666666667	147.68961889908044
45	293.685	146.82363266291162
46	293.665	146.89460884706813
47	293.9816666666667	146.33188760675304
48	294.47	145.41733883321282
49	294.62666666666667	145.12785382398377
50	294.9533333333333	144.48574724018863
51	294.94666666666666	144.51100473281906
52	295.10833333333335	144.18372514685157
53	295.10333333333335	144.20306049302653
54	295.26666666666665	143.85714750713146
55	295.2633333333333	143.87030266489555
56	295.42833333333334	143.50537108608737
57	295.4266666666667	143.51208296013166
58	295.425	143.51885256531943
59	295.42333333333335	143.5256798934907
60	295.4216666666667	143.53256493640117
61	295.42	143.5395076857465
62	295.41833333333335	143.54650813315538
63	295.4166666666667	143.55356627018773
64	295.415	143.56068208833042
65	295.41333333333336	143.56785557901142
66	295.4116666666667	143.57508673358114
67	295.41	143.58237554333206
68	295.40833333333336	143.5897219994831
69	295.4066666666667	143.59712609318547
70	295.405	143.604587815524
71	295.57166666666666	143.1448504041347
72	295.57166666666666	143.1448504041347
73	295.57166666666666	143.1448504041347
74	295.57166666666666	143.1448504041347
75	295.57166666666666	143.1448504041347
76	295.57166666666666	143.1448504041347
77	295.57166666666666	143.1448504041347
78	295.57166666666666	143.1448504041347
79	295.57166666666666	143.1448504041347
80	295.57166666666666	143.1448504041347
81	295.57166666666666	143.1448504041347
82	295.57166666666666	143.1448504041347
83	295.57166666666666	143.1448504041347
84	295.57166666666666	143.1448504041347
85	295.57166666666666	143.1448504041347
86	295.57166666666666	143.1448504041347
87	295.57166666666666	143.1448504041347
88	295.57166666666666	143.1448504041347
89	295.57166666666666	143.1448504041347
90	295.57166666666666	143.1448504041347
91	295.57166666666666	143.1448504041347
92	295.57166666666666	143.1448504041347
93	295.57166666666666	143.1448504041347
94	295.57166666666666	143.1448504041347
95	295.57166666666666	143.1448504041347
96	295.57166666666666	143.1448504041347
97	295.57166666666666	143.1448504041347
98	295.57166666666666	143.1448504041347
99	295.57166666666666	143.1448504041347
100	295.57166666666666	143.1448504041347
101	295.57166666666666	143.1448504041347
102	295.57166666666666	143.1448504041347
103	295.57166666666666	143.1448504041347
104	295.57166666666666	143.1448504041347
105	295.57166666666666	143.1448504041347
106	295.57166666666666	143.1448504041347
107	295.57166666666666	143.1448504041347
108	295.57166666666666	143.1448504041347
109	295.57166666666666	143.1448504041347
110	295.57166666666666	143.1448504041347
111	295.57166666666666	143.1448504041347
112	295.57166666666666	143.1448504041347
113	295.57166666666666	143.1448504041347
114	295.57166666666666	143.1448504041347
115	295.57166666666666	143.1448504041347
116	295.57166666666666	143.1448504041347
117	295.57166666666666	143.1448504041347
118	295.57166666666666	143.1448504041347
119	295.57166666666666	143.1448504041347
120	295.57166666666666	143.1448504041347
121	295.57166666666666	143.1448504041347
122	295.57166666666666	143.1448504041347
123	295.57166666666666	143.1448504041347
124	295.57166666666666	143.1448504041347
125	295.57166666666666	143.1448504041347
126	295.57166666666666	143.1448504041347
127	295.57166666666666	143.1448504041347
128	295.57166666666666	143.1448504041347
129	295.57166666666666	143.1448504041347
130	295.57166666666666	143.1448504041347
131	295.57166666666666	143.1448504041347
132	295.57166666666666	143.1448504041347
133	295.57166666666666	143.1448504041347
134	295.57166666666666	143.1448504041347
135	295.57166666666666	143.1448504041347
136	295.57166666666666	143.1448504041347
137	295.57166666666666	143.1448504041347
138	295.57166666666666	143.1448504041347
139	295.57166666666666	143.1448504041347
140	295.57166666666666	143.1448504041347
141	295.57166666666666	143.1448504041347
142	295.57166666666666	143.1448504041347
143	295.57166666666666	143.1448504041347
144	295.57166666666666	143.1448504041347
145	295.57166666666666	143.1448504041347
146	295.57166666666666	143.1448504041347
147	295.57166666666666	143.1448504041347
148	295.57166666666666	143.1448504041347
149	295.57166666666666	143.1448504041347
150	295.57166666666666	143.1448504041347
151	295.57166666666666	143.1448504041347
152	295.57166666666666	143.1448504041347
153	295.57166666666666	143.1448504041347
154	295.57166666666666	143.1448504041347
155	295.57166666666666	143.1448504041347
156	295.57166666666666	143.1448504041347
157	295.57166666666666	143.1448504041347
158	295.57166666666666	143.1448504041347
159	295.57166666666666	143.1448504041347
160	295.57166666666666	143.1448504041347
161	295.57166666666666	143.1448504041347
162	295.57166666666666	143.1448504041347
163	295.57166666666666	143.1448504041347
164	295.57166666666666	143.1448504041347
165	295.57166666666666	143.1448504041347
166	295.57166666666666	143.1448504041347
167	295.57166666666666	143.1448504041347
168	295.57166666666666	143.1448504041347
169	295.57166666666666	143.1448504041347
170	295.57166666666666	143.1448504041347
171	295.57166666666666	143.1448504041347
172	295.57166666666666	143.1448504041347
173	295.57166666666666	143.1448504041347
174	295.57166666666666	143.1448504041347
175	295.57166666666666	143.1448504041347
176	295.57166666666666	143.1448504041347
177	295.57166666666666	143.1448504041347
178	295.57166666666666	143.1448504041347
179	295.57166666666666	143.1448504041347
180	295.57166666666666	143.1448504041347
181	295.57166666666666	143.1448504041347
182	295.57166666666666	143.1448504041347
183	295.57166666666666	143.1448504041347
184	295.57166666666666	143.1448504041347
185	295.57166666666666	143.1448504041347
186	295.57166666666666	143.1448504041347
187	295.57166666666666	143.1448504041347
188	295.57166666666666	143.1448504041347
189	295.57166666666666	143.1448504041347
190	295.57166666666666	143.1448504041347
191	295.57166666666666	143.1448504041347
192	295.57166666666666	143.1448504041347
193	295.57166666666666	143.1448504041347
194	295.57166666666666	143.1448504041347
195	295.57166666666666	143.1448504041347
196	295.57166666666666	143.1448504041347
197	295.57166666666666	143.1448504041347
198	295.57166666666666	143.1448504041347
199	295.57166666666666	143.1448504041347
200	295.57166666666666	143.1448504041347
201	295.57166666666666	143.1448504041347
202	295.57166666666666	143.1448504041347
203	295.57166666666666	143.1448504041347
204	295.57166666666666	143.1448504041347
205	295.57166666666666	143.1448504041347
206	295.57166666666666	143.1448504041347
207	295.57166666666666	143.1448504041347
208	295.57166666666666	143.1448504041347
209	295.57166666666666	143.1448504041347
210	295.57166666666666	143.1448504041347
211	295.57166666666666	143.1448504041347
212	295.57166666666666	143.1448504041347
213	295.57166666666666	143.1448504041347
214	295.57166666666666	143.1448504041347
215	295.57166666666666	143.1448504041347
216	295.57166666666666	143.1448504041347
217	295.57166666666666	143.1448504041347
218	295.57166666666666	143.1448504041347
219	295.57166666666666	143.1448504041347
220	295.57166666666666	143.1448504041347
221	295.57166666666666	143.1448504041347
222	295.57166666666666	143.1448504041347
223	295.57166666666666	143.1448504041347
224	295.57166666666666	143.1448504041347
225	295.57166666666666	143.1448504041347
226	295.57166666666666	143.1448504041347
227	295.57166666666666	143.1448504041347
228	295.57166666666666	143.1448504041347
229	295.57166666666666	143.1448504041347
230	295.57166666666666	143.1448504041347
231	295.57166666666666	143.1448504041347
232	295.57166666666666	143.1448504041347
233	295.57166666666666	143.1448504041347
234	295.57166666666666	143.1448504041347
235	295.57166666666666	143.1448504041347
236	295.57166666666666	143.1448504041347
237	295.57166666666666	143.1448504041347
238	295.57166666666666	143.1448504041347
239	295.57166666666666	143.1448504041347
240	295.57166666666666	143.1448504041347
241	295.57166666666666	143.1448504041347
242	295.57166666666666	143.1448504041347
243	295.57166666666666	143.1448504041347
244	295.57166666666666	143.1448504041347
245	295.57166666666666	143.1448504041347
246	295.57166666666666	143.1448504041347
247	295.57166666666666	143.1448504041347
248	295.57166666666666	143.1448504041347
249	295.57166666666666	143.1448504041347
250	295.57166666666666	143.1448504041347
251	295.57166666666666	143.1448504041347
252	295.57166666666666	143.1448504041347
253	295.57166666666666	143.1448504041347
254	295.57166666666666	143.1448504041347
255	295.57166666666666	143.1448504041347
256	295.57166666666666	143.1448504041347
257	295.57166666666666	143.1448504041347
258	295.57166666666666	143.1448504041347
259	295.57166666666666	143.1448504041347
260	295.57166666666666	143.1448504041347
261	295.57166666666666	143.1448504041347
262	295.57166666666666	143.1448504041347
263	295.57166666666666	143.1448504041347
264	295.57166666666666	143.1448504041347
265	295.57166666666666	143.1448504041347
266	295.57166666666666	143.1448504041347
267	295.57166666666666	143.1448504041347
268	295.57166666666666	143.1448504041347
269	295.57166666666666	143.1448504041347
270	295.57166666666666	143.1448504041347
271	295.57166666666666	143.1448504041347
272	295.57166666666666	143.1448504041347
273	295.57166666666666	143.1448504041347
274	295.57166666666666	143.1448504041347
275	295.57166666666666	143.1448504041347
276	295.57166666666666	143.1448504041347
277	295.57166666666666	143.1448504041347
278	295.57166666666666	143.1448504041347
279	295.57166666666666	143.1448504041347
280	295.57166666666666	143.1448504041347
281	295.57166666666666	143.1448504041347
282	295.57166666666666	143.1448504041347
283	295.57166666666666	143.1448504041347
284	295.57166666666666	143.1448504041347
285	295.57166666666666	143.1448504041347
286	295.57166666666666	143.1448504041347
287	295.57166666666666	143.1448504041347
288	295.57166666666666	143.1448504041347
289	295.57166666666666	143.1448504041347
290	295.57166666666666	143.1448504041347
291	295.57166666666666	143.1448504041347
292	295.57166666666666	143.1448504041347
293	295.57166666666666	143.1448504041347
294	295.57166666666666	143.1448504041347
295	295.57166666666666	143.1448504041347
296	295.57166666666666	143.1448504041347
297	295.57166666666666	143.1448504041347
298	295.57166666666666	143.1448504041347
299	295.57166666666666	143.1448504041347


==> rock_sim_files/rock_mdp_fwd.tex <==
% $\mathrm{Opt. \ policy \  on \ MDP}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.1283333333333319	4.083017334711572
4	6.253333333333535	24.841333610649247
5	24.13489999999953	43.04331049834101
6	24.83129999999987	43.52864853913255
7	37.06959999999909	48.52782029420623
8	74.61149999999853	43.287960424926666
9	95.0404333333324	20.56143838545585
10	98.8731999999992	7.5331269576452575
11	99.40649999999923	1.8381606068748937
12	99.43983333333254	0.13149133896277101
13	99.43983333333254	0.13149133896277101
14	99.43983333333254	0.13149133896277101
15	99.43983333333254	0.13149133896277101
16	99.43983333333254	0.13149133896277101
17	99.43983333333254	0.13149133896277101
18	99.43983333333254	0.13149133896277101
19	99.43983333333254	0.13149133896277101
20	99.43983333333254	0.13149133896277101
21	99.43983333333254	0.13149133896277101
22	99.43983333333254	0.13149133896277101
23	99.43983333333254	0.13149133896277101
24	99.43983333333254	0.13149133896277101
25	99.43983333333254	0.13149133896277101
26	99.43983333333254	0.13149133896277101
27	99.43983333333254	0.13149133896277101
28	99.43983333333254	0.13149133896277101
29	99.43983333333254	0.13149133896277101
30	99.43983333333254	0.13149133896277101
31	99.43983333333254	0.13149133896277101
32	99.43983333333254	0.13149133896277101
33	99.43983333333254	0.13149133896277101
34	99.43983333333254	0.13149133896277101
35	99.43983333333254	0.13149133896277101
36	99.43983333333254	0.13149133896277101
37	99.43983333333254	0.13149133896277101
38	99.43983333333254	0.13149133896277101
39	99.43983333333254	0.13149133896277101
40	99.43983333333254	0.13149133896277101
41	99.43983333333254	0.13149133896277101
42	99.43983333333254	0.13149133896277101
43	99.43983333333254	0.13149133896277101
44	99.43983333333254	0.13149133896277101
45	99.43983333333254	0.13149133896277101
46	99.43983333333254	0.13149133896277101
47	99.43983333333254	0.13149133896277101
48	99.43983333333254	0.13149133896277101
49	99.43983333333254	0.13149133896277101
50	99.43983333333254	0.13149133896277101
51	99.43983333333254	0.13149133896277101
52	99.43983333333254	0.13149133896277101
53	99.43983333333254	0.13149133896277101
54	99.43983333333254	0.13149133896277101
55	99.43983333333254	0.13149133896277101
56	99.43983333333254	0.13149133896277101
57	99.43983333333254	0.13149133896277101
58	99.43983333333254	0.13149133896277101
59	99.43983333333254	0.13149133896277101
60	99.43983333333254	0.13149133896277101
61	99.43983333333254	0.13149133896277101
62	99.43983333333254	0.13149133896277101
63	99.43983333333254	0.13149133896277101
64	99.43983333333254	0.13149133896277101
65	99.43983333333254	0.13149133896277101
66	99.43983333333254	0.13149133896277101
67	99.43983333333254	0.13149133896277101
68	99.43983333333254	0.13149133896277101
69	99.43983333333254	0.13149133896277101
70	99.43983333333254	0.13149133896277101
71	99.43983333333254	0.13149133896277101
72	99.43983333333254	0.13149133896277101
73	99.43983333333254	0.13149133896277101
74	99.43983333333254	0.13149133896277101
75	99.43983333333254	0.13149133896277101
76	99.43983333333254	0.13149133896277101
77	99.43983333333254	0.13149133896277101
78	99.43983333333254	0.13149133896277101
79	99.43983333333254	0.13149133896277101
80	99.43983333333254	0.13149133896277101
81	99.43983333333254	0.13149133896277101
82	99.43983333333254	0.13149133896277101
83	99.43983333333254	0.13149133896277101
84	99.43983333333254	0.13149133896277101
85	99.43983333333254	0.13149133896277101
86	99.43983333333254	0.13149133896277101
87	99.43983333333254	0.13149133896277101
88	99.43983333333254	0.13149133896277101
89	99.43983333333254	0.13149133896277101
90	99.43983333333254	0.13149133896277101
91	99.43983333333254	0.13149133896277101
92	99.43983333333254	0.13149133896277101
93	99.43983333333254	0.13149133896277101
94	99.43983333333254	0.13149133896277101
95	99.43983333333254	0.13149133896277101
96	99.43983333333254	0.13149133896277101
97	99.43983333333254	0.13149133896277101
98	99.43983333333254	0.13149133896277101
99	99.43983333333254	0.13149133896277101
100	99.43983333333254	0.13149133896277101
101	99.43983333333254	0.13149133896277101
102	99.43983333333254	0.13149133896277101
103	99.43983333333254	0.13149133896277101
104	99.43983333333254	0.13149133896277101
105	99.43983333333254	0.13149133896277101
106	99.43983333333254	0.13149133896277101
107	99.43983333333254	0.13149133896277101
108	99.43983333333254	0.13149133896277101
109	99.43983333333254	0.13149133896277101
110	99.43983333333254	0.13149133896277101
111	99.43983333333254	0.13149133896277101
112	99.43983333333254	0.13149133896277101
113	99.43983333333254	0.13149133896277101
114	99.43983333333254	0.13149133896277101
115	99.43983333333254	0.13149133896277101
116	99.43983333333254	0.13149133896277101
117	99.43983333333254	0.13149133896277101
118	99.43983333333254	0.13149133896277101
119	99.43983333333254	0.13149133896277101
120	99.43983333333254	0.13149133896277101
121	99.43983333333254	0.13149133896277101
122	99.43983333333254	0.13149133896277101
123	99.43983333333254	0.13149133896277101
124	99.43983333333254	0.13149133896277101
125	99.43983333333254	0.13149133896277101
126	99.43983333333254	0.13149133896277101
127	99.43983333333254	0.13149133896277101
128	99.43983333333254	0.13149133896277101
129	99.43983333333254	0.13149133896277101
130	99.43983333333254	0.13149133896277101
131	99.43983333333254	0.13149133896277101
132	99.43983333333254	0.13149133896277101
133	99.43983333333254	0.13149133896277101
134	99.43983333333254	0.13149133896277101
135	99.43983333333254	0.13149133896277101
136	99.43983333333254	0.13149133896277101
137	99.43983333333254	0.13149133896277101
138	99.43983333333254	0.13149133896277101
139	99.43983333333254	0.13149133896277101
140	99.43983333333254	0.13149133896277101
141	99.43983333333254	0.13149133896277101
142	99.43983333333254	0.13149133896277101
143	99.43983333333254	0.13149133896277101
144	99.43983333333254	0.13149133896277101
145	99.43983333333254	0.13149133896277101
146	99.43983333333254	0.13149133896277101
147	99.43983333333254	0.13149133896277101
148	99.43983333333254	0.13149133896277101
149	99.43983333333254	0.13149133896277101
150	99.43983333333254	0.13149133896277101
151	99.43983333333254	0.13149133896277101
152	99.43983333333254	0.13149133896277101
153	99.43983333333254	0.13149133896277101
154	99.43983333333254	0.13149133896277101
155	99.43983333333254	0.13149133896277101
156	99.43983333333254	0.13149133896277101
157	99.43983333333254	0.13149133896277101
158	99.43983333333254	0.13149133896277101
159	99.43983333333254	0.13149133896277101
160	99.43983333333254	0.13149133896277101
161	99.43983333333254	0.13149133896277101
162	99.43983333333254	0.13149133896277101
163	99.43983333333254	0.13149133896277101
164	99.43983333333254	0.13149133896277101
165	99.43983333333254	0.13149133896277101
166	99.43983333333254	0.13149133896277101
167	99.43983333333254	0.13149133896277101
168	99.43983333333254	0.13149133896277101
169	99.43983333333254	0.13149133896277101
170	99.43983333333254	0.13149133896277101
171	99.43983333333254	0.13149133896277101
172	99.43983333333254	0.13149133896277101
173	99.43983333333254	0.13149133896277101
174	99.43983333333254	0.13149133896277101
175	99.43983333333254	0.13149133896277101
176	99.43983333333254	0.13149133896277101
177	99.43983333333254	0.13149133896277101
178	99.43983333333254	0.13149133896277101
179	99.43983333333254	0.13149133896277101
180	99.43983333333254	0.13149133896277101
181	99.43983333333254	0.13149133896277101
182	99.43983333333254	0.13149133896277101
183	99.43983333333254	0.13149133896277101
184	99.43983333333254	0.13149133896277101
185	99.43983333333254	0.13149133896277101
186	99.43983333333254	0.13149133896277101
187	99.43983333333254	0.13149133896277101
188	99.43983333333254	0.13149133896277101
189	99.43983333333254	0.13149133896277101
190	99.43983333333254	0.13149133896277101
191	99.43983333333254	0.13149133896277101
192	99.43983333333254	0.13149133896277101
193	99.43983333333254	0.13149133896277101
194	99.43983333333254	0.13149133896277101
195	99.43983333333254	0.13149133896277101
196	99.43983333333254	0.13149133896277101
197	99.43983333333254	0.13149133896277101
198	99.43983333333254	0.13149133896277101
199	99.43983333333254	0.13149133896277101
200	99.43983333333254	0.13149133896277101
201	99.43983333333254	0.13149133896277101
202	99.43983333333254	0.13149133896277101
203	99.43983333333254	0.13149133896277101
204	99.43983333333254	0.13149133896277101
205	99.43983333333254	0.13149133896277101
206	99.43983333333254	0.13149133896277101
207	99.43983333333254	0.13149133896277101
208	99.43983333333254	0.13149133896277101
209	99.43983333333254	0.13149133896277101
210	99.43983333333254	0.13149133896277101
211	99.43983333333254	0.13149133896277101
212	99.43983333333254	0.13149133896277101
213	99.43983333333254	0.13149133896277101
214	99.43983333333254	0.13149133896277101
215	99.43983333333254	0.13149133896277101
216	99.43983333333254	0.13149133896277101
217	99.43983333333254	0.13149133896277101
218	99.43983333333254	0.13149133896277101
219	99.43983333333254	0.13149133896277101
220	99.43983333333254	0.13149133896277101
221	99.43983333333254	0.13149133896277101
222	99.43983333333254	0.13149133896277101
223	99.43983333333254	0.13149133896277101
224	99.43983333333254	0.13149133896277101
225	99.43983333333254	0.13149133896277101
226	99.43983333333254	0.13149133896277101
227	99.43983333333254	0.13149133896277101
228	99.43983333333254	0.13149133896277101
229	99.43983333333254	0.13149133896277101
230	99.43983333333254	0.13149133896277101
231	99.43983333333254	0.13149133896277101
232	99.43983333333254	0.13149133896277101
233	99.43983333333254	0.13149133896277101
234	99.43983333333254	0.13149133896277101
235	99.43983333333254	0.13149133896277101
236	99.43983333333254	0.13149133896277101
237	99.43983333333254	0.13149133896277101
238	99.43983333333254	0.13149133896277101
239	99.43983333333254	0.13149133896277101
240	99.43983333333254	0.13149133896277101
241	99.43983333333254	0.13149133896277101
242	99.43983333333254	0.13149133896277101
243	99.43983333333254	0.13149133896277101
244	99.43983333333254	0.13149133896277101
245	99.43983333333254	0.13149133896277101
246	99.43983333333254	0.13149133896277101
247	99.43983333333254	0.13149133896277101
248	99.43983333333254	0.13149133896277101
249	99.43983333333254	0.13149133896277101
250	99.43983333333254	0.13149133896277101
251	99.43983333333254	0.13149133896277101
252	99.43983333333254	0.13149133896277101
253	99.43983333333254	0.13149133896277101
254	99.43983333333254	0.13149133896277101
255	99.43983333333254	0.13149133896277101
256	99.43983333333254	0.13149133896277101
257	99.43983333333254	0.13149133896277101
258	99.43983333333254	0.13149133896277101
259	99.43983333333254	0.13149133896277101
260	99.43983333333254	0.13149133896277101
261	99.43983333333254	0.13149133896277101
262	99.43983333333254	0.13149133896277101
263	99.43983333333254	0.13149133896277101
264	99.43983333333254	0.13149133896277101
265	99.43983333333254	0.13149133896277101
266	99.43983333333254	0.13149133896277101
267	99.43983333333254	0.13149133896277101
268	99.43983333333254	0.13149133896277101
269	99.43983333333254	0.13149133896277101
270	99.43983333333254	0.13149133896277101
271	99.43983333333254	0.13149133896277101
272	99.43983333333254	0.13149133896277101
273	99.43983333333254	0.13149133896277101
274	99.43983333333254	0.13149133896277101
275	99.43983333333254	0.13149133896277101
276	99.43983333333254	0.13149133896277101
277	99.43983333333254	0.13149133896277101
278	99.43983333333254	0.13149133896277101
279	99.43983333333254	0.13149133896277101
280	99.43983333333254	0.13149133896277101
281	99.43983333333254	0.13149133896277101
282	99.43983333333254	0.13149133896277101
283	99.43983333333254	0.13149133896277101
284	99.43983333333254	0.13149133896277101
285	99.43983333333254	0.13149133896277101
286	99.43983333333254	0.13149133896277101
287	99.43983333333254	0.13149133896277101
288	99.43983333333254	0.13149133896277101
289	99.43983333333254	0.13149133896277101
290	99.43983333333254	0.13149133896277101
291	99.43983333333254	0.13149133896277101
292	99.43983333333254	0.13149133896277101
293	99.43983333333254	0.13149133896277101
294	99.43983333333254	0.13149133896277101
295	99.43983333333254	0.13149133896277101
296	99.43983333333254	0.13149133896277101
297	99.43983333333254	0.13149133896277101
298	99.43983333333254	0.13149133896277101
299	99.43983333333254	0.13149133896277101
300	99.43983333333254	0.13149133896277101
301	99.43983333333254	0.13149133896277101
302	99.43983333333254	0.13149133896277101
303	99.43983333333254	0.13149133896277101
304	99.43983333333254	0.13149133896277101
305	99.43983333333254	0.13149133896277101
306	99.43983333333254	0.13149133896277101
307	99.43983333333254	0.13149133896277101
308	99.43983333333254	0.13149133896277101
309	99.43983333333254	0.13149133896277101
310	99.43983333333254	0.13149133896277101
311	99.43983333333254	0.13149133896277101
312	99.43983333333254	0.13149133896277101
313	99.43983333333254	0.13149133896277101
314	99.43983333333254	0.13149133896277101
315	99.43983333333254	0.13149133896277101
316	99.43983333333254	0.13149133896277101
317	99.43983333333254	0.13149133896277101
318	99.43983333333254	0.13149133896277101
319	99.43983333333254	0.13149133896277101
320	99.43983333333254	0.13149133896277101
321	99.43983333333254	0.13149133896277101
322	99.43983333333254	0.13149133896277101
323	99.43983333333254	0.13149133896277101
324	99.43983333333254	0.13149133896277101
325	99.43983333333254	0.13149133896277101
326	99.43983333333254	0.13149133896277101
327	99.43983333333254	0.13149133896277101
328	99.43983333333254	0.13149133896277101
329	99.43983333333254	0.13149133896277101
330	99.43983333333254	0.13149133896277101
331	99.43983333333254	0.13149133896277101
332	99.43983333333254	0.13149133896277101
333	99.43983333333254	0.13149133896277101
334	99.43983333333254	0.13149133896277101
335	99.43983333333254	0.13149133896277101
336	99.43983333333254	0.13149133896277101
337	99.43983333333254	0.13149133896277101
338	99.43983333333254	0.13149133896277101
339	99.43983333333254	0.13149133896277101
340	99.43983333333254	0.13149133896277101
341	99.43983333333254	0.13149133896277101
342	99.43983333333254	0.13149133896277101
343	99.43983333333254	0.13149133896277101
344	99.43983333333254	0.13149133896277101
345	99.43983333333254	0.13149133896277101
346	99.43983333333254	0.13149133896277101
347	99.43983333333254	0.13149133896277101
348	99.43983333333254	0.13149133896277101
349	99.43983333333254	0.13149133896277101
350	99.43983333333254	0.13149133896277101
351	99.43983333333254	0.13149133896277101
352	99.43983333333254	0.13149133896277101
353	99.43983333333254	0.13149133896277101
354	99.43983333333254	0.13149133896277101
355	99.43983333333254	0.13149133896277101
356	99.43983333333254	0.13149133896277101
357	99.43983333333254	0.13149133896277101
358	99.43983333333254	0.13149133896277101
359	99.43983333333254	0.13149133896277101
360	99.43983333333254	0.13149133896277101
361	99.43983333333254	0.13149133896277101
362	99.43983333333254	0.13149133896277101
363	99.43983333333254	0.13149133896277101
364	99.43983333333254	0.13149133896277101
365	99.43983333333254	0.13149133896277101
366	99.43983333333254	0.13149133896277101
367	99.43983333333254	0.13149133896277101
368	99.43983333333254	0.13149133896277101
369	99.43983333333254	0.13149133896277101
370	99.43983333333254	0.13149133896277101
371	99.43983333333254	0.13149133896277101
372	99.43983333333254	0.13149133896277101
373	99.43983333333254	0.13149133896277101
374	99.43983333333254	0.13149133896277101
375	99.43983333333254	0.13149133896277101
376	99.43983333333254	0.13149133896277101
377	99.43983333333254	0.13149133896277101
378	99.43983333333254	0.13149133896277101
379	99.43983333333254	0.13149133896277101
380	99.43983333333254	0.13149133896277101
381	99.43983333333254	0.13149133896277101
382	99.43983333333254	0.13149133896277101
383	99.43983333333254	0.13149133896277101
384	99.43983333333254	0.13149133896277101
385	99.43983333333254	0.13149133896277101
386	99.43983333333254	0.13149133896277101
387	99.43983333333254	0.13149133896277101
388	99.43983333333254	0.13149133896277101
389	99.43983333333254	0.13149133896277101
390	99.43983333333254	0.13149133896277101
391	99.43983333333254	0.13149133896277101
392	99.43983333333254	0.13149133896277101
393	99.43983333333254	0.13149133896277101
394	99.43983333333254	0.13149133896277101
395	99.43983333333254	0.13149133896277101
396	99.43983333333254	0.13149133896277101
397	99.43983333333254	0.13149133896277101
398	99.43983333333254	0.13149133896277101
399	99.43983333333254	0.13149133896277101
400	99.43983333333254	0.13149133896277101
401	99.43983333333254	0.13149133896277101
402	99.43983333333254	0.13149133896277101
403	99.43983333333254	0.13149133896277101
404	99.43983333333254	0.13149133896277101
405	99.43983333333254	0.13149133896277101
406	99.43983333333254	0.13149133896277101
407	99.43983333333254	0.13149133896277101
408	99.43983333333254	0.13149133896277101
409	99.43983333333254	0.13149133896277101
410	99.43983333333254	0.13149133896277101
411	99.43983333333254	0.13149133896277101
412	99.43983333333254	0.13149133896277101
413	99.43983333333254	0.13149133896277101
414	99.43983333333254	0.13149133896277101
415	99.43983333333254	0.13149133896277101
416	99.43983333333254	0.13149133896277101
417	99.43983333333254	0.13149133896277101
418	99.43983333333254	0.13149133896277101
419	99.43983333333254	0.13149133896277101
420	99.43983333333254	0.13149133896277101
421	99.43983333333254	0.13149133896277101
422	99.43983333333254	0.13149133896277101
423	99.43983333333254	0.13149133896277101
424	99.43983333333254	0.13149133896277101
425	99.43983333333254	0.13149133896277101
426	99.43983333333254	0.13149133896277101
427	99.43983333333254	0.13149133896277101
428	99.43983333333254	0.13149133896277101
429	99.43983333333254	0.13149133896277101
430	99.43983333333254	0.13149133896277101
431	99.43983333333254	0.13149133896277101
432	99.43983333333254	0.13149133896277101
433	99.43983333333254	0.13149133896277101
434	99.43983333333254	0.13149133896277101
435	99.43983333333254	0.13149133896277101
436	99.43983333333254	0.13149133896277101
437	99.43983333333254	0.13149133896277101
438	99.43983333333254	0.13149133896277101
439	99.43983333333254	0.13149133896277101
440	99.43983333333254	0.13149133896277101
441	99.43983333333254	0.13149133896277101
442	99.43983333333254	0.13149133896277101
443	99.43983333333254	0.13149133896277101
444	99.43983333333254	0.13149133896277101
445	99.43983333333254	0.13149133896277101
446	99.43983333333254	0.13149133896277101
447	99.43983333333254	0.13149133896277101
448	99.43983333333254	0.13149133896277101
449	99.43983333333254	0.13149133896277101
450	99.43983333333254	0.13149133896277101
451	99.43983333333254	0.13149133896277101
452	99.43983333333254	0.13149133896277101
453	99.43983333333254	0.13149133896277101
454	99.43983333333254	0.13149133896277101
455	99.43983333333254	0.13149133896277101
456	99.43983333333254	0.13149133896277101
457	99.43983333333254	0.13149133896277101
458	99.43983333333254	0.13149133896277101
459	99.43983333333254	0.13149133896277101
460	99.43983333333254	0.13149133896277101
461	99.43983333333254	0.13149133896277101
462	99.43983333333254	0.13149133896277101
463	99.43983333333254	0.13149133896277101
464	99.43983333333254	0.13149133896277101
465	99.43983333333254	0.13149133896277101
466	99.43983333333254	0.13149133896277101
467	99.43983333333254	0.13149133896277101
468	99.43983333333254	0.13149133896277101
469	99.43983333333254	0.13149133896277101
470	99.43983333333254	0.13149133896277101
471	99.43983333333254	0.13149133896277101
472	99.43983333333254	0.13149133896277101
473	99.43983333333254	0.13149133896277101
474	99.43983333333254	0.13149133896277101
475	99.43983333333254	0.13149133896277101
476	99.43983333333254	0.13149133896277101
477	99.43983333333254	0.13149133896277101
478	99.43983333333254	0.13149133896277101
479	99.43983333333254	0.13149133896277101
480	99.43983333333254	0.13149133896277101
481	99.43983333333254	0.13149133896277101
482	99.43983333333254	0.13149133896277101
483	99.43983333333254	0.13149133896277101
484	99.43983333333254	0.13149133896277101
485	99.43983333333254	0.13149133896277101
486	99.43983333333254	0.13149133896277101
487	99.43983333333254	0.13149133896277101
488	99.43983333333254	0.13149133896277101
489	99.43983333333254	0.13149133896277101
490	99.43983333333254	0.13149133896277101
491	99.43983333333254	0.13149133896277101
492	99.43983333333254	0.13149133896277101
493	99.43983333333254	0.13149133896277101
494	99.43983333333254	0.13149133896277101
495	99.43983333333254	0.13149133896277101
496	99.43983333333254	0.13149133896277101
497	99.43983333333254	0.13149133896277101
498	99.43983333333254	0.13149133896277101
499	99.43983333333254	0.13149133896277101


==> rock_sim_files/rock_mem10_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=10, N=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29996666666665167	0.0018254375426791172
4	-0.3999333333333329	0.002581128091014121
5	-2.1500999999999624	2.0109433913796053
6	-3.1691333333334013	3.179429809817464
7	-3.5519666666668286	3.789990694652906
8	7.1298666666665085	31.50817779533135
9	61.58489999999993	48.19223321231308
10	83.13459999999986	34.16661513095302
11	91.39653333333285	22.082675139474475
12	94.5936333333328	13.27053840149513
13	95.19266666666623	10.644507482995921
14	95.35719999999957	9.817095369473135
15	95.42313333333287	9.44565004903772
16	95.58926666666618	8.425779773739487
17	95.62206666666619	8.194830874534256
18	95.68826666666622	7.7375191326993775
19	95.68779999999956	7.74364026110024
20	95.72069999999954	7.524523119551463
21	95.71893333333287	7.548741718252686
22	95.71853333333286	7.554137708273111
23	95.71676666666623	7.578324938856009
24	95.71639999999955	7.583278822954161
25	95.74799999999955	7.357349341531568
26	95.74763333333287	7.362462975496474
27	95.74589999999954	7.386935529929321
28	95.80959999999955	6.923581046443255
29	95.84269999999955	6.6495117647840205
30	95.84239999999954	6.6542063568842575
31	95.87546666666621	6.367883330868628
32	95.87519999999952	6.372237045182709
33	95.94033333333289	5.795957202127156
34	95.94016666666622	5.798949615136348
35	95.93863333333287	5.826737577657755
36	95.93846666666622	5.829742159726168
37	95.93693333333286	5.857458145722322
38	95.97009999999955	5.523429730701756
39	95.9699333333329	5.526633332830647
40	96.0031333333329	5.169089879487787
41	96.00299999999956	5.171824726341694
42	96.00286666666621	5.174560701053678
43	96.00273333333288	5.177297801835406
44	96.00259999999957	5.180036026901728
45	96.00246666666622	5.182775374470935
46	96.00233333333288	5.185515842763977
47	96.00219999999955	5.1882574300047
48	96.00206666666622	5.191000134420667
49	96.0019333333329	5.193743954241665
50	96.00179999999956	5.1964888877009985
51	96.00033333333289	5.2266286031777565
52	96.00023333333287	5.228691035579984
53	96.00009999999955	5.231450084823516
54	95.99996666666623	5.234210223668414
55	96.03319999999957	4.843980225668434
56	96.03309999999956	4.846214439126711
57	96.03299999999956	4.848449683489935
58	96.03289999999957	4.8506859573329
59	96.03279999999958	4.852923259232556
60	96.03269999999956	4.855161587767519
61	96.03126666666624	4.8880837140494355
62	96.03119999999957	4.889558933073572
63	96.03109999999957	4.891813173388064
64	96.03099999999958	4.894068416631104
65	96.03089999999958	4.896324661416981
66	96.06416666666622	4.4375638180074155
67	96.06409999999956	4.4391967580482525
68	96.0640333333329	4.440830597859863
69	96.06396666666623	4.442465336449563
70	96.06256666666623	4.4767028877908785
71	96.0625333333329	4.4775301505283
72	96.06246666666623	4.479184961078883
73	96.06239999999956	4.4808406473190825
74	96.06233333333289	4.482497208278225
75	96.09563333333291	4.001035399188046
76	96.09559999999956	4.001965430468791
77	96.09556666666624	4.002896078119268
78	96.09553333333292	4.003827341709681
79	96.09549999999957	4.004759220810449
80	96.09546666666624	4.005691714991996
81	96.0954333333329	4.006624823824789
82	96.09539999999957	4.0075585468794745
83	96.09536666666625	4.008492883726916
84	96.0953333333329	4.0094278339378375
85	96.09529999999958	4.01036339708351
86	96.09526666666623	4.01129957273483
87	96.09523333333291	4.012236360463066
88	96.09519999999958	4.0131737598398285
89	96.09516666666624	4.014111770436373
90	96.09513333333291	4.015050391824339
91	96.09509999999958	4.015989623575625
92	96.09506666666624	4.0169294652617955
93	96.09503333333292	4.017869916455127
94	96.09499999999957	4.018810976727739
95	96.09496666666625	4.019752645651445
96	96.0949333333329	4.020694922799091
97	96.09489999999958	4.021637807742892
98	96.09486666666625	4.0225813000553705
99	96.0948333333329	4.023525399309567
100	96.09479999999958	4.024470105077978
101	96.09476666666623	4.025415416933896
102	96.09473333333291	4.0263613344501055
103	96.09469999999959	4.02730785720026
104	96.09466666666624	4.02825498475733
105	96.09463333333291	4.029202716694973
106	96.09459999999957	4.0301510525868345
107	96.09456666666624	4.031099992006545
108	96.09453333333292	4.032049534528279
109	96.09449999999957	4.0329996797255125
110	96.09446666666625	4.033950427172957
111	96.0944333333329	4.034901776444606
112	96.09439999999958	4.035853727114859
113	96.09436666666625	4.036806278758286
114	96.09433333333291	4.03775943094963
115	96.09429999999958	4.038713183263582
116	96.09426666666623	4.039667535275097
117	96.09423333333291	4.04062248655943
118	96.09419999999959	4.041578036691427
119	96.09416666666624	4.042534185246804
120	96.09413333333292	4.043490931800845
121	96.09409999999957	4.044448275929199
122	96.09406666666624	4.045406217207681
123	96.09403333333292	4.046364755211983
124	96.09399999999957	4.0473238895183705
125	96.09396666666625	4.048283619703041
126	96.0939333333329	4.049243945341997
127	96.09389999999958	4.050204866012001
128	96.09386666666626	4.05116638128933
129	96.09383333333291	4.0521284907509445
130	96.09379999999958	4.053091193973712
131	96.09376666666624	4.054054490534438
132	96.0937333333329	4.055018380010369
133	96.09369999999959	4.055982861978979
134	96.09366666666624	4.056947936017371
135	96.09363333333292	4.057913601703293
136	96.09359999999957	4.058879858614529
137	96.09356666666625	4.059846706328827
138	96.09353333333291	4.060814144424169
139	96.09349999999958	4.06178217247883
140	96.09213333333291	4.101974091689025
141	96.09213333333291	4.101974091689025
142	96.09209999999958	4.102966519076909
143	96.09206666666624	4.103959518427233
144	96.09203333333292	4.104953089324545
145	96.12536666666625	3.4674764885848917
146	96.12536666666625	3.4674764885848917
147	96.12536666666625	3.4674764885848917
148	96.12536666666625	3.4674764885848917
149	96.12536666666625	3.4674764885848917
150	96.12536666666625	3.4674764885848917
151	96.12536666666625	3.4674764885848917
152	96.12536666666625	3.4674764885848917
153	96.12536666666625	3.4674764885848917
154	96.12536666666625	3.4674764885848917
155	96.12536666666625	3.4674764885848917
156	96.12536666666625	3.4674764885848917
157	96.12536666666625	3.4674764885848917
158	96.12536666666625	3.4674764885848917
159	96.12536666666625	3.4674764885848917
160	96.12536666666625	3.4674764885848917
161	96.12536666666625	3.4674764885848917
162	96.12536666666625	3.4674764885848917
163	96.12536666666625	3.4674764885848917
164	96.12536666666625	3.4674764885848917
165	96.12536666666625	3.4674764885848917
166	96.12536666666625	3.4674764885848917
167	96.12536666666625	3.4674764885848917
168	96.12536666666625	3.4674764885848917
169	96.12536666666625	3.4674764885848917
170	96.12536666666625	3.4674764885848917
171	96.12536666666625	3.4674764885848917
172	96.12536666666625	3.4674764885848917
173	96.12536666666625	3.4674764885848917
174	96.12536666666625	3.4674764885848917
175	96.12536666666625	3.4674764885848917
176	96.12536666666625	3.4674764885848917
177	96.12536666666625	3.4674764885848917
178	96.12536666666625	3.4674764885848917
179	96.12536666666625	3.4674764885848917
180	96.12536666666625	3.4674764885848917
181	96.12536666666625	3.4674764885848917
182	96.12536666666625	3.4674764885848917
183	96.12536666666625	3.4674764885848917
184	96.12536666666625	3.4674764885848917
185	96.12536666666625	3.4674764885848917
186	96.12536666666625	3.4674764885848917
187	96.12536666666625	3.4674764885848917
188	96.12536666666625	3.4674764885848917
189	96.12536666666625	3.4674764885848917
190	96.12536666666625	3.4674764885848917
191	96.12536666666625	3.4674764885848917
192	96.12536666666625	3.4674764885848917
193	96.12536666666625	3.4674764885848917
194	96.12536666666625	3.4674764885848917
195	96.12536666666625	3.4674764885848917
196	96.12536666666625	3.4674764885848917
197	96.12536666666625	3.4674764885848917
198	96.12536666666625	3.4674764885848917
199	96.12536666666625	3.4674764885848917
200	96.12536666666625	3.4674764885848917
201	96.12536666666625	3.4674764885848917
202	96.12536666666625	3.4674764885848917
203	96.12536666666625	3.4674764885848917
204	96.12536666666625	3.4674764885848917
205	96.12536666666625	3.4674764885848917
206	96.12536666666625	3.4674764885848917
207	96.12536666666625	3.4674764885848917
208	96.12536666666625	3.4674764885848917
209	96.12536666666625	3.4674764885848917
210	96.12536666666625	3.4674764885848917
211	96.12536666666625	3.4674764885848917
212	96.12536666666625	3.4674764885848917
213	96.12536666666625	3.4674764885848917
214	96.12536666666625	3.4674764885848917
215	96.12536666666625	3.4674764885848917
216	96.12536666666625	3.4674764885848917
217	96.12536666666625	3.4674764885848917
218	96.12536666666625	3.4674764885848917
219	96.12536666666625	3.4674764885848917
220	96.12536666666625	3.4674764885848917
221	96.12536666666625	3.4674764885848917
222	96.12536666666625	3.4674764885848917
223	96.12536666666625	3.4674764885848917
224	96.12536666666625	3.4674764885848917
225	96.12536666666625	3.4674764885848917
226	96.12536666666625	3.4674764885848917
227	96.12536666666625	3.4674764885848917
228	96.12536666666625	3.4674764885848917
229	96.12536666666625	3.4674764885848917
230	96.12536666666625	3.4674764885848917
231	96.12536666666625	3.4674764885848917
232	96.12536666666625	3.4674764885848917
233	96.12536666666625	3.4674764885848917
234	96.12536666666625	3.4674764885848917
235	96.12536666666625	3.4674764885848917
236	96.12536666666625	3.4674764885848917
237	96.12536666666625	3.4674764885848917
238	96.12536666666625	3.4674764885848917
239	96.12536666666625	3.4674764885848917
240	96.12536666666625	3.4674764885848917
241	96.12536666666625	3.4674764885848917
242	96.12536666666625	3.4674764885848917
243	96.12536666666625	3.4674764885848917
244	96.12536666666625	3.4674764885848917
245	96.12536666666625	3.4674764885848917
246	96.12536666666625	3.4674764885848917
247	96.12536666666625	3.4674764885848917
248	96.12536666666625	3.4674764885848917
249	96.12536666666625	3.4674764885848917
250	96.12536666666625	3.4674764885848917
251	96.12536666666625	3.4674764885848917
252	96.12536666666625	3.4674764885848917
253	96.12536666666625	3.4674764885848917
254	96.12536666666625	3.4674764885848917
255	96.12536666666625	3.4674764885848917
256	96.12536666666625	3.4674764885848917
257	96.12536666666625	3.4674764885848917
258	96.12536666666625	3.4674764885848917
259	96.12536666666625	3.4674764885848917
260	96.12536666666625	3.4674764885848917
261	96.12536666666625	3.4674764885848917
262	96.12536666666625	3.4674764885848917
263	96.12536666666625	3.4674764885848917
264	96.12536666666625	3.4674764885848917
265	96.12536666666625	3.4674764885848917
266	96.12536666666625	3.4674764885848917
267	96.12536666666625	3.4674764885848917
268	96.12536666666625	3.4674764885848917
269	96.12536666666625	3.4674764885848917
270	96.12536666666625	3.4674764885848917
271	96.12536666666625	3.4674764885848917
272	96.12536666666625	3.4674764885848917
273	96.12536666666625	3.4674764885848917
274	96.12536666666625	3.4674764885848917
275	96.12536666666625	3.4674764885848917
276	96.12536666666625	3.4674764885848917
277	96.12536666666625	3.4674764885848917
278	96.12536666666625	3.4674764885848917
279	96.12536666666625	3.4674764885848917
280	96.12536666666625	3.4674764885848917
281	96.12536666666625	3.4674764885848917
282	96.12536666666625	3.4674764885848917
283	96.12536666666625	3.4674764885848917
284	96.12536666666625	3.4674764885848917
285	96.12536666666625	3.4674764885848917
286	96.12536666666625	3.4674764885848917
287	96.12536666666625	3.4674764885848917
288	96.12536666666625	3.4674764885848917
289	96.12536666666625	3.4674764885848917
290	96.12536666666625	3.4674764885848917
291	96.12536666666625	3.4674764885848917
292	96.12536666666625	3.4674764885848917
293	96.12536666666625	3.4674764885848917
294	96.12536666666625	3.4674764885848917
295	96.12536666666625	3.4674764885848917
296	96.12536666666625	3.4674764885848917
297	96.12536666666625	3.4674764885848917
298	96.12536666666625	3.4674764885848917
299	96.12536666666625	3.4674764885848917
300	96.12536666666625	3.4674764885848917
301	96.12536666666625	3.4674764885848917
302	96.12536666666625	3.4674764885848917
303	96.12536666666625	3.4674764885848917
304	96.12536666666625	3.4674764885848917
305	96.12536666666625	3.4674764885848917
306	96.12536666666625	3.4674764885848917
307	96.12536666666625	3.4674764885848917
308	96.12536666666625	3.4674764885848917
309	96.12536666666625	3.4674764885848917
310	96.12536666666625	3.4674764885848917
311	96.12536666666625	3.4674764885848917
312	96.12536666666625	3.4674764885848917
313	96.12536666666625	3.4674764885848917
314	96.12536666666625	3.4674764885848917
315	96.12536666666625	3.4674764885848917
316	96.12536666666625	3.4674764885848917
317	96.12536666666625	3.4674764885848917
318	96.12536666666625	3.4674764885848917
319	96.12536666666625	3.4674764885848917
320	96.12536666666625	3.4674764885848917
321	96.12536666666625	3.4674764885848917
322	96.12536666666625	3.4674764885848917
323	96.12536666666625	3.4674764885848917
324	96.12536666666625	3.4674764885848917
325	96.12536666666625	3.4674764885848917
326	96.12536666666625	3.4674764885848917
327	96.12536666666625	3.4674764885848917
328	96.12536666666625	3.4674764885848917
329	96.12536666666625	3.4674764885848917
330	96.12536666666625	3.4674764885848917
331	96.12536666666625	3.4674764885848917
332	96.12536666666625	3.4674764885848917
333	96.12536666666625	3.4674764885848917
334	96.12536666666625	3.4674764885848917
335	96.12536666666625	3.4674764885848917
336	96.12536666666625	3.4674764885848917
337	96.12536666666625	3.4674764885848917
338	96.12536666666625	3.4674764885848917
339	96.12536666666625	3.4674764885848917
340	96.12536666666625	3.4674764885848917
341	96.12536666666625	3.4674764885848917
342	96.12536666666625	3.4674764885848917
343	96.12536666666625	3.4674764885848917
344	96.12536666666625	3.4674764885848917
345	96.12536666666625	3.4674764885848917
346	96.12536666666625	3.4674764885848917
347	96.12536666666625	3.4674764885848917
348	96.12536666666625	3.4674764885848917
349	96.12536666666625	3.4674764885848917
350	96.12536666666625	3.4674764885848917
351	96.12536666666625	3.4674764885848917
352	96.12536666666625	3.4674764885848917
353	96.12536666666625	3.4674764885848917
354	96.12536666666625	3.4674764885848917
355	96.12536666666625	3.4674764885848917
356	96.12536666666625	3.4674764885848917
357	96.12536666666625	3.4674764885848917
358	96.12536666666625	3.4674764885848917
359	96.12536666666625	3.4674764885848917
360	96.12536666666625	3.4674764885848917
361	96.12536666666625	3.4674764885848917
362	96.12536666666625	3.4674764885848917
363	96.12536666666625	3.4674764885848917
364	96.12536666666625	3.4674764885848917
365	96.12536666666625	3.4674764885848917
366	96.12536666666625	3.4674764885848917
367	96.12536666666625	3.4674764885848917
368	96.12536666666625	3.4674764885848917
369	96.12536666666625	3.4674764885848917
370	96.12536666666625	3.4674764885848917
371	96.12536666666625	3.4674764885848917
372	96.12536666666625	3.4674764885848917
373	96.12536666666625	3.4674764885848917
374	96.12536666666625	3.4674764885848917
375	96.12536666666625	3.4674764885848917
376	96.12536666666625	3.4674764885848917
377	96.12536666666625	3.4674764885848917
378	96.12536666666625	3.4674764885848917
379	96.12536666666625	3.4674764885848917
380	96.12536666666625	3.4674764885848917
381	96.12536666666625	3.4674764885848917
382	96.12536666666625	3.4674764885848917
383	96.12536666666625	3.4674764885848917
384	96.12536666666625	3.4674764885848917
385	96.12536666666625	3.4674764885848917
386	96.12536666666625	3.4674764885848917
387	96.12536666666625	3.4674764885848917
388	96.12536666666625	3.4674764885848917
389	96.12536666666625	3.4674764885848917
390	96.12536666666625	3.4674764885848917
391	96.12536666666625	3.4674764885848917
392	96.12536666666625	3.4674764885848917
393	96.12536666666625	3.4674764885848917
394	96.12536666666625	3.4674764885848917
395	96.12536666666625	3.4674764885848917
396	96.12536666666625	3.4674764885848917
397	96.12536666666625	3.4674764885848917
398	96.12536666666625	3.4674764885848917
399	96.12536666666625	3.4674764885848917
400	96.12536666666625	3.4674764885848917
401	96.12536666666625	3.4674764885848917
402	96.12536666666625	3.4674764885848917
403	96.12536666666625	3.4674764885848917
404	96.12536666666625	3.4674764885848917
405	96.12536666666625	3.4674764885848917
406	96.12536666666625	3.4674764885848917
407	96.12536666666625	3.4674764885848917
408	96.12536666666625	3.4674764885848917
409	96.12536666666625	3.4674764885848917
410	96.12536666666625	3.4674764885848917
411	96.12536666666625	3.4674764885848917
412	96.12536666666625	3.4674764885848917
413	96.12536666666625	3.4674764885848917
414	96.12536666666625	3.4674764885848917
415	96.12536666666625	3.4674764885848917
416	96.12536666666625	3.4674764885848917
417	96.12536666666625	3.4674764885848917
418	96.12536666666625	3.4674764885848917
419	96.12536666666625	3.4674764885848917
420	96.12536666666625	3.4674764885848917
421	96.12536666666625	3.4674764885848917
422	96.12536666666625	3.4674764885848917
423	96.12536666666625	3.4674764885848917
424	96.12536666666625	3.4674764885848917
425	96.12536666666625	3.4674764885848917
426	96.12536666666625	3.4674764885848917
427	96.12536666666625	3.4674764885848917
428	96.12536666666625	3.4674764885848917
429	96.12536666666625	3.4674764885848917
430	96.12536666666625	3.4674764885848917
431	96.12536666666625	3.4674764885848917
432	96.12536666666625	3.4674764885848917
433	96.12536666666625	3.4674764885848917
434	96.12536666666625	3.4674764885848917
435	96.12536666666625	3.4674764885848917
436	96.12536666666625	3.4674764885848917
437	96.12536666666625	3.4674764885848917
438	96.12536666666625	3.4674764885848917
439	96.12536666666625	3.4674764885848917
440	96.12536666666625	3.4674764885848917
441	96.12536666666625	3.4674764885848917
442	96.12536666666625	3.4674764885848917
443	96.12536666666625	3.4674764885848917
444	96.12536666666625	3.4674764885848917
445	96.12536666666625	3.4674764885848917
446	96.12536666666625	3.4674764885848917
447	96.12536666666625	3.4674764885848917
448	96.12536666666625	3.4674764885848917
449	96.12536666666625	3.4674764885848917
450	96.12536666666625	3.4674764885848917
451	96.12536666666625	3.4674764885848917
452	96.12536666666625	3.4674764885848917
453	96.12536666666625	3.4674764885848917
454	96.12536666666625	3.4674764885848917
455	96.12536666666625	3.4674764885848917
456	96.12536666666625	3.4674764885848917
457	96.12536666666625	3.4674764885848917
458	96.12536666666625	3.4674764885848917
459	96.12536666666625	3.4674764885848917
460	96.12536666666625	3.4674764885848917
461	96.12536666666625	3.4674764885848917
462	96.12536666666625	3.4674764885848917
463	96.12536666666625	3.4674764885848917
464	96.12536666666625	3.4674764885848917
465	96.12536666666625	3.4674764885848917
466	96.12536666666625	3.4674764885848917
467	96.12536666666625	3.4674764885848917
468	96.12536666666625	3.4674764885848917
469	96.12536666666625	3.4674764885848917
470	96.12536666666625	3.4674764885848917
471	96.12536666666625	3.4674764885848917
472	96.12536666666625	3.4674764885848917
473	96.12536666666625	3.4674764885848917
474	96.12536666666625	3.4674764885848917
475	96.12536666666625	3.4674764885848917
476	96.12536666666625	3.4674764885848917
477	96.12536666666625	3.4674764885848917
478	96.12536666666625	3.4674764885848917
479	96.12536666666625	3.4674764885848917
480	96.12536666666625	3.4674764885848917
481	96.12536666666625	3.4674764885848917
482	96.12536666666625	3.4674764885848917
483	96.12536666666625	3.4674764885848917
484	96.12536666666625	3.4674764885848917
485	96.12536666666625	3.4674764885848917
486	96.12536666666625	3.4674764885848917
487	96.12536666666625	3.4674764885848917
488	96.12536666666625	3.4674764885848917
489	96.12536666666625	3.4674764885848917
490	96.12536666666625	3.4674764885848917
491	96.12536666666625	3.4674764885848917
492	96.12536666666625	3.4674764885848917
493	96.12536666666625	3.4674764885848917
494	96.12536666666625	3.4674764885848917
495	96.12536666666625	3.4674764885848917
496	96.12536666666625	3.4674764885848917
497	96.12536666666625	3.4674764885848917
498	96.12536666666625	3.4674764885848917
499	96.12536666666625	3.4674764885848917


==> rock_sim_files/rock_mem10_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.3165333333333185	3.2403816620199675
4	-0.030433333333328455	12.870844461244857
5	4.786600000000139	26.032255257148613
6	6.940466666666768	29.377600352120318
7	12.22296666666655	35.036998004950014
8	23.184366666666243	42.21885943823674
9	25.713633333333103	43.409570113807206
10	27.31039999999986	44.18510509028969
11	28.273866666666557	44.620847486149735
12	29.6379	45.20807560886246
13	30.568066666666727	45.57708401081485
14	31.531833333333392	45.94624797854102
15	32.42830000000012	46.25669143424956
16	33.45860000000012	46.60509527980872
17	34.68860000000013	46.979156619789485
18	35.88580000000012	47.32607588169523
19	36.749566666666816	47.542087036773836
20	37.914033333333464	47.82796266898208
21	38.64496666666682	47.98055475570887
22	39.67633333333345	48.18771018861756
23	40.17400000000014	48.273894781064634
24	41.07186666666678	48.424933404004335
25	41.80280000000014	48.52782499583774
26	42.43390000000012	48.62216861463586
27	43.16450000000015	48.7045174128304
28	44.09570000000013	48.8083320569002
29	44.66020000000017	48.85204802216632
30	45.89216666666683	48.937887251483104
31	46.157066666666836	48.94940479783411
32	46.788866666666856	48.983337262605765
33	47.3873666666669	48.98809376163703
34	47.85240000000023	49.003974405892166
35	48.283966666666885	48.99515404199573
36	48.78226666666686	49.00045263936033
37	49.48046666666688	48.98622192462776
38	50.04553333333358	48.969970867006936
39	50.4769666666669	48.94781662953804
40	51.17536666666688	48.915113988748644
41	51.707266666666854	48.874908496373614
42	52.23940000000017	48.83381773225051
43	52.73803333333351	48.7812080976425
44	53.036766666666786	48.75843870427842
45	53.46886666666679	48.714412966960495
46	54.03470000000011	48.65909629839675
47	54.200366666666746	48.635365423378694
48	54.56620000000007	48.59558969248148
49	54.99876666666673	48.54001279163607
50	55.19800000000007	48.51468309697621
51	55.43026666666672	48.47874768661244
52	55.79613333333336	48.427308945631104
53	56.028466666666695	48.38876518692655
54	56.42753333333332	48.33052350136029
55	56.692966666666656	48.284203219398755
56	56.99193333333332	48.230903249496606
57	57.42419999999997	48.14212127676422
58	57.85659999999996	48.06613495771571
59	58.05553333333326	48.02628873213306
60	58.42126666666657	47.95688411892
61	58.720433333333226	47.88626301782386
62	59.01983333333322	47.8215315170785
63	59.285933333333226	47.7565287906156
64	59.552199999999864	47.694911627552486
65	59.618366666666525	47.67851479089482
66	59.81793333333319	47.6326984860427
67	60.01753333333317	47.58623882926191
68	60.15033333333316	47.551396262944266
69	60.24979999999983	47.52075511423102
70	60.44929999999983	47.47250712616049
71	60.64863333333317	47.409091654085834
72	60.7812666666665	47.375371123213455
73	60.98053333333315	47.322211638745614
74	61.24663333333316	47.251268081737784
75	61.446099999999824	47.18965590879011
76	61.57886666666648	47.156182628038025
77	61.8783999999998	47.075129174260304
78	62.01129999999979	47.03720338529882
79	62.110733333333116	47.002321837638206
80	62.24356666666647	46.96376339206202
81	62.509699999999796	46.88178469203156
82	62.67599999999979	46.835359476930655
83	62.74226666666643	46.814105924698374
84	63.0087333333331	46.73755924017466
85	63.00839999999975	46.738020526904464
86	63.14146666666641	46.696511866686386
87	63.17433333333309	46.68726887017038
88	63.27389999999974	46.652397103007424
89	63.40676666666642	46.607324791412786
90	63.639733333333055	46.53120989825659
91	63.73933333333304	46.49811759152769
92	63.83899999999971	46.46476527793183
93	63.93863333333303	46.43085910755417
94	64.13846666666636	46.35908073918469
95	64.17156666666635	46.348870553073546
96	64.27143333333302	46.317070725729316
97	64.30453333333301	46.30359143143112
98	64.37099999999968	46.2823651693237
99	64.40413333333301	46.27178373028364
100	64.50386666666635	46.2338538127876
101	64.57026666666633	46.21240550540002
102	64.63666666666633	46.18796541187812
103	64.769733333333	46.13836773513137
104	64.86949999999966	46.10527149632703
105	64.96926666666631	46.06911071562899
106	65.03573333333298	46.04681411124488
107	65.10219999999964	46.02136860734761
108	65.23543333333298	45.97595089985197
109	65.23526666666632	45.976191841671884
110	65.26843333333296	45.9620380337101
111	65.3015666666663	45.95073282925462
112	65.36803333333297	45.9279039524509
113	65.43443333333298	45.902013002469545
114	65.50089999999965	45.878967394548
115	65.56739999999965	45.84965333100563
116	65.70066666666632	45.79960450581324
117	65.7005666666663	45.79974894049313
118	65.7337666666663	45.78807024191909
119	65.73359999999964	45.788317262230315
120	65.76683333333297	45.77656369044674
121	65.83343333333298	45.74679805420527
122	65.86673333333297	45.73486139327606
123	65.86659999999964	45.73505749903449
124	65.8997666666663	45.720367998798444
125	65.9329666666663	45.70859164167665
126	65.99953333333296	45.684571718639994
127	66.06606666666629	45.66034422992837
128	66.06593333333294	45.66054152981053
129	66.1324999999996	45.63337748202091
130	66.1990999999996	45.60897772577266
131	66.19896666666627	45.60917549059815
132	66.26556666666626	45.581737691889735
133	66.26543333333292	45.58193299044656
134	66.29866666666626	45.569732479159356
135	66.33189999999959	45.557431216615406
136	66.39846666666625	45.532604555953775
137	66.39829999999958	45.532855175613214
138	66.43149999999959	45.52059934157991
139	66.49796666666624	45.48988626642433
140	66.56446666666625	45.46502154457769
141	66.59763333333291	45.45274554669061
142	66.66416666666625	45.42766858027041
143	66.76409999999957	45.38662946863678
144	66.79736666666625	45.37102581015328
145	66.79729999999958	45.37112770668948
146	66.79716666666624	45.371331498780165
147	66.86369999999958	45.34282602915291
148	66.86353333333292	45.34307962834311
149	66.93009999999958	45.314409599191634
150	66.99673333333291	45.28861559666209
151	67.03003333333291	45.27268088666237
152	67.02996666666624	45.272783199904275
153	67.02989999999957	45.27288566007245
154	67.06309999999957	45.2600989289312
155	67.09633333333291	45.24421104652252
156	67.09619999999957	45.24441938582041
157	67.16276666666623	45.21549775256526
158	67.19603333333289	45.1992497090999
159	67.22929999999955	45.18318955293734
160	67.26259999999955	45.167120060652344
161	67.26256666666623	45.16717010630919
162	67.29586666666623	45.15402347796767
163	67.2958333333329	45.154073710340704
164	67.29576666666621	45.15417698004814
165	67.29566666666622	45.15433033374461
166	67.36229999999954	45.12465182185137
167	67.3622666666662	45.124701988255715
168	67.39559999999955	45.11141910839559
169	67.39559999999955	45.11141910839559
170	67.39559999999955	45.11141910839559
171	67.39556666666621	45.11146916633909
172	67.39549999999954	45.11157238540158
173	67.39543333333289	45.11167575191088
174	67.42873333333287	45.098417796291926
175	67.46206666666622	45.0820466231173
176	67.46203333333288	45.08209668888055
177	67.46199999999955	45.08214682850234
178	67.46196666666621	45.08219704198347
179	67.49523333333289	45.06900221451815
180	67.49516666666622	45.069102719848175
181	67.52839999999955	45.05593005853903
182	67.56166666666621	45.042604763588656
183	67.56159999999954	45.042705722162616
184	67.6282666666662	45.01561967060866
185	67.62823333333287	45.01567000736698
186	67.62819999999954	45.01572041809426
187	67.6281666666662	45.015770902787004
188	67.62813333333287	45.01582146144701
189	67.6614666666662	45.002235446500336
190	67.6614666666662	45.002235446500336
191	67.6614666666662	45.002235446500336
192	67.6614666666662	45.002235446500336
193	67.6614666666662	45.002235446500336
194	67.6614666666662	45.002235446500336
195	67.6614666666662	45.002235446500336
196	67.6614666666662	45.002235446500336
197	67.66143333333287	45.002285822821605
198	67.66139999999953	45.002336273131256
199	67.69473333333286	44.98886972273155
200	67.69473333333286	44.98886972273155
201	67.69473333333286	44.98886972273155
202	67.69469999999953	44.98892317645185
203	67.6946666666662	44.988976704175705
204	67.69463333333286	44.98903030590433
205	67.72793333333287	44.97247268862288
206	67.72789999999952	44.97252322166614
207	67.72783333333285	44.972627400515016
208	67.76113333333285	44.95908224206655
209	67.7944666666662	44.942413776397025
210	67.7944666666662	44.942413776397025
211	67.7944666666662	44.942413776397025
212	67.7944666666662	44.942413776397025
213	67.7944666666662	44.942413776397025
214	67.7944666666662	44.942413776397025
215	67.7944666666662	44.942413776397025
216	67.7944666666662	44.942413776397025
217	67.7944666666662	44.942413776397025
218	67.79443333333286	44.94246424424877
219	67.79439999999953	44.942514786186756
220	67.79436666666619	44.94256540221339
221	67.82769999999952	44.92898228734622
222	67.82769999999952	44.92898228734622
223	67.82769999999952	44.92898228734622
224	67.82769999999952	44.92898228734622
225	67.82769999999952	44.92898228734622
226	67.82769999999952	44.92898228734622
227	67.82769999999952	44.92898228734622
228	67.82769999999952	44.92898228734622
229	67.82769999999952	44.92898228734622
230	67.82769999999952	44.92898228734622
231	67.82769999999952	44.92898228734622
232	67.82769999999952	44.92898228734622
233	67.82769999999952	44.92898228734622
234	67.82769999999952	44.92898228734622
235	67.82769999999952	44.92898228734622
236	67.82769999999952	44.92898228734622
237	67.82769999999952	44.92898228734622
238	67.82769999999952	44.92898228734622
239	67.82769999999952	44.92898228734622
240	67.82769999999952	44.92898228734622
241	67.82769999999952	44.92898228734622
242	67.82769999999952	44.92898228734622
243	67.82769999999952	44.92898228734622
244	67.82769999999952	44.92898228734622
245	67.82769999999952	44.92898228734622
246	67.82769999999952	44.92898228734622
247	67.82769999999952	44.92898228734622
248	67.82769999999952	44.92898228734622
249	67.82766666666619	44.92903286913235
250	67.82763333333286	44.92908352502714
251	67.82759999999952	44.92913425503235
252	67.86093333333285	44.915448201358736
253	67.86093333333285	44.915448201358736
254	67.86093333333285	44.915448201358736
255	67.86093333333285	44.915448201358736
256	67.86093333333285	44.915448201358736
257	67.86093333333285	44.915448201358736
258	67.86093333333285	44.915448201358736
259	67.86093333333285	44.915448201358736
260	67.86093333333285	44.915448201358736
261	67.86093333333285	44.915448201358736
262	67.86093333333285	44.915448201358736
263	67.86093333333285	44.915448201358736
264	67.86093333333285	44.915448201358736
265	67.86093333333285	44.915448201358736
266	67.86093333333285	44.915448201358736
267	67.86093333333285	44.915448201358736
268	67.86093333333285	44.915448201358736
269	67.86093333333285	44.915448201358736
270	67.86093333333285	44.915448201358736
271	67.86093333333285	44.915448201358736
272	67.86093333333285	44.915448201358736
273	67.86093333333285	44.915448201358736
274	67.86093333333285	44.915448201358736
275	67.86093333333285	44.915448201358736
276	67.86093333333285	44.915448201358736
277	67.86093333333285	44.915448201358736
278	67.86093333333285	44.915448201358736
279	67.86093333333285	44.915448201358736
280	67.86093333333285	44.915448201358736
281	67.86093333333285	44.915448201358736
282	67.86093333333285	44.915448201358736
283	67.86093333333285	44.915448201358736
284	67.86093333333285	44.915448201358736
285	67.86093333333285	44.915448201358736
286	67.86093333333285	44.915448201358736
287	67.86093333333285	44.915448201358736
288	67.86093333333285	44.915448201358736
289	67.86093333333285	44.915448201358736
290	67.86093333333285	44.915448201358736
291	67.86093333333285	44.915448201358736
292	67.86093333333285	44.915448201358736
293	67.86093333333285	44.915448201358736
294	67.86093333333285	44.915448201358736
295	67.86093333333285	44.915448201358736
296	67.86093333333285	44.915448201358736
297	67.86093333333285	44.915448201358736
298	67.86093333333285	44.915448201358736
299	67.86093333333285	44.915448201358736
300	67.86093333333285	44.915448201358736
301	67.86093333333285	44.915448201358736
302	67.86093333333285	44.915448201358736
303	67.86093333333285	44.915448201358736
304	67.86093333333285	44.915448201358736
305	67.86093333333285	44.915448201358736
306	67.86093333333285	44.915448201358736
307	67.86093333333285	44.915448201358736
308	67.86093333333285	44.915448201358736
309	67.86093333333285	44.915448201358736
310	67.86093333333285	44.915448201358736
311	67.86093333333285	44.915448201358736


==> rock_sim_files/rock_mem10_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.48773333333330954	0.8562609778696182
4	-1.8031000000000201	5.624688470484497
5	-1.5245000000000413	11.775497289569602
6	0.21510000000000384	17.713532171478274
7	2.6735666666666598	22.992601953937704
8	11.653366666666713	34.11918065642201
9	18.34099999999962	39.16831252002905
10	22.93249999999958	41.829072749504355
11	25.458599999999638	43.0699616055864
12	27.150999999999716	43.87847147520062
13	28.677533333333017	44.54067992950068
14	30.171233333333046	45.16518521839867
15	31.63199999999971	45.69768757096259
16	33.22569999999976	46.26584812627232
17	34.353299999999756	46.60412230454128
18	35.2143999999998	46.85104679698557
19	36.20843333333313	47.10402416155381
20	37.73663333333318	47.47299029973636
21	38.7975666666665	47.70125530226901
22	40.28759999999988	47.97079347102747
23	41.31599999999987	48.13553154721881
24	42.2780999999999	48.27357762851934
25	43.106166666666525	48.375081174493886
26	44.40153333333325	48.50797602094799
27	45.663733333333354	48.602036905828626
28	46.258966666666694	48.63986588110859
29	47.25436666666664	48.65836688174923
30	48.28233333333331	48.66781045573703
31	49.07816666666664	48.65065460305242
32	50.07453333333333	48.6226425798605
33	50.837200000000024	48.58496807477264
34	51.63349999999999	48.54081019530547
35	52.32949999999995	48.476981957935905
36	53.19236666666662	48.3985746869906
37	54.02179999999994	48.29846455212936
38	54.68459999999994	48.21921943416303
39	55.44733333333328	48.10840023206854
40	56.31043333333329	47.9768034347039
41	57.006633333333255	47.850541613085205
42	57.63639999999991	47.73366402976688
43	58.532833333333265	47.54909152976048
44	59.396633333333284	47.354464470968715
45	60.16056666666652	47.17167732526492
46	60.59139999999986	47.063993944840426
47	61.05533333333318	46.937899096099066
48	61.71953333333318	46.746433216331
49	62.350333333333175	46.564028175071904
50	62.98159999999988	46.36183374400413
51	63.51236666666655	46.189278305672836
52	64.1433333333332	45.977306310347814
53	64.53909999999986	45.83740686226338
54	65.1031666666665	45.63059244233956
55	65.70073333333319	45.40611551464081
56	66.2986333333332	45.166065965488535
57	66.99679999999987	44.87600966099061
58	67.2934666666665	44.76104791723352
59	67.8580666666665	44.51357412740019
60	68.3228666666665	44.311572270859145
61	68.65413333333316	44.15789196639214
62	69.3858999999998	43.82107215168672
63	69.71759999999979	43.653233521775455
64	69.94806666666645	43.538530249219995
65	70.17846666666644	43.428132621403535
66	70.54363333333309	43.24268407641009
67	71.00896666666645	42.98914199654209
68	71.27416666666646	42.845378155707415
69	71.57106666666645	42.685708102309505
70	71.76919999999977	42.57679201192435
71	72.13389999999976	42.36076251426539
72	72.59913333333309	42.10651373895576
73	72.89753333333306	41.9215881607024
74	73.1279999999997	41.78793074561125
75	73.32639999999974	41.67547963779181
76	73.69153333333306	41.453070111258214
77	74.02343333333303	41.24951176533972
78	74.35566666666635	41.04261973309649
79	74.65486666666632	40.8475492897948
80	74.78729999999965	40.762595869784164
81	75.01959999999967	40.61281278742784
82	75.38546666666633	40.35909193868924
83	75.51786666666632	40.27109286798913
84	75.71696666666631	40.12796990627476
85	75.91573333333302	39.986466032841
86	76.1144666666663	39.85459861440793
87	76.24629999999965	39.76045757168777
88	76.57823333333295	39.53410008518694
89	76.87706666666631	39.316557929141695
90	77.20949999999962	39.06795651703155
91	77.47543333333294	38.87294474497107
92	77.6746999999996	38.72131191703972
93	77.84056666666628	38.592855612736756
94	77.93973333333295	38.52000053559461
95	78.10553333333294	38.38881394428431
96	78.30469999999963	38.22798618695466
97	78.46916666666628	38.10529603575101
98	78.66833333333294	37.94418300463045
99	78.86753333333293	37.780896397282966
100	78.93329999999956	37.729845053706285
101	79.19906666666624	37.50925751236483
102	79.33176666666623	37.40379037226302
103	79.43099999999956	37.312800203146935
104	79.59699999999954	37.17862052757371
105	79.66279999999956	37.121793457392485
106	79.76193333333286	37.037470543521614
107	79.96116666666619	36.865282249096666
108	80.12713333333285	36.723337771988696
109	80.35986666666619	36.514777684049676
110	80.52596666666618	36.36071592252947
111	80.62543333333284	36.267167196775794
112	80.69156666666616	36.210331107004485
113	80.79103333333285	36.12074375755437
114	80.85713333333283	36.06308023148068
115	80.98996666666615	35.93766291787567
116	81.0560333333328	35.879977753601025
117	81.15543333333278	35.78815591522183
118	81.28826666666612	35.66572232544234
119	81.42103333333277	35.538576424296274
120	81.5204666666661	35.44090745333115
121	81.65333333333277	35.31240493399192
122	81.81969999999944	35.15581073701306
123	81.91936666666611	35.059659176878725
124	81.95233333333277	35.0294108032408
125	82.08529999999944	34.892349981669724
126	82.25173333333274	34.73124122451682
127	82.28476666666609	34.70050630676092
128	82.31769999999942	34.669677001331614
129	82.35066666666607	34.638806362549836
130	82.45043333333275	34.535100112960706
131	82.61679999999942	34.36557479649258
132	82.61643333333275	34.36648299257385
133	82.68279999999943	34.2931366917636
134	82.74923333333275	34.22849669615762
135	82.81576666666608	34.15847686024965
136	82.84896666666609	34.12617166143208
137	82.88209999999941	34.09328119913571
138	82.9152999999994	34.05673427155557
139	82.91506666666608	34.05731159377613
140	82.98149999999941	33.99196494884251
141	82.98119999999942	33.99270872643116
142	83.01426666666607	33.96021402262097
143	83.14739999999941	33.82170989034489
144	83.18056666666605	33.788834630375725
145	83.21363333333275	33.75604445822316
146	83.24666666666606	33.723174656145346
147	83.24626666666607	33.72417509832088
148	83.37926666666606	33.589683487576615
149	83.5123999999994	33.449198190290616
150	83.57893333333273	33.38101999932838
151	83.64546666666607	33.303753734109556
152	83.64533333333273	33.304099420675094
153	83.64509999999939	33.304700008507105
154	83.7114999999994	33.232486782514364
155	83.74459999999941	33.193915368733556
156	83.81103333333273	33.124803017259026
157	83.8773999999994	33.0513444392207
158	83.91036666666606	33.01284693164535
159	84.01009999999937	32.907578174689746
160	84.04329999999939	32.87222416838682
161	84.07653333333272	32.833154726823786
162	84.10969999999938	32.79794631644908
163	84.10956666666605	32.7982988148097
164	84.17616666666605	32.727784454581524
165	84.20936666666604	32.68849831768884
166	84.24256666666604	32.648824655907724
167	84.24236666666603	32.64934897358438
168	84.2754333333327	32.61444822690645
169	84.3753333333327	32.502636378539435
170	84.4419333333327	32.4222944118534
171	84.47523333333271	32.38601369849186
172	84.47516666666604	32.38619376584533
173	84.47509999999937	32.386373317440906
174	84.47503333333269	32.38655307375076
175	84.50829999999937	32.34595360231832
176	84.50819999999936	32.34622079048293
177	84.54146666666603	32.30987393737218
178	84.54139999999937	32.31005384355319
179	84.57466666666603	32.26970289433837
180	84.57459999999936	32.26987896124403
181	84.57443333333269	32.27032118958369
182	84.64109999999937	32.19708983935258
183	84.64106666666603	32.19717803673007
184	84.64096666666603	32.19744355895696
185	84.64089999999936	32.1976206759132
186	84.64086666666603	32.197708768102856
187	84.64076666666604	32.197973560648606
188	84.67399999999937	32.16171788529551
189	84.67376666666603	32.162343848236965
190	84.7403333333327	32.08871971927509
191	84.77356666666603	32.05130155358569
192	84.80676666666602	32.01421076457902
193	84.80659999999935	32.014661169116486
194	84.80643333333268	32.015112087037416
195	84.80626666666602	32.01556351831948
196	84.90619999999934	31.902718508407023
197	84.93949999999934	31.865361702272867
198	84.97276666666602	31.82329830505024
199	84.97266666666602	31.823568827033025
200	85.00593333333268	31.786453689093612
201	85.00579999999934	31.786818961533807
202	85.03899999999933	31.748753660576853
203	85.03889999999934	31.74902597125379
204	85.03879999999934	31.749298594247005
205	85.038666666666	31.749659917688906
206	85.10533333333268	31.673195369095314
207	85.10529999999935	31.673285724355495
208	85.10523333333268	31.673470643619215
209	85.10516666666601	31.673655772143128
210	85.10503333333267	31.67402223693025
211	85.13829999999933	31.6360659655506
212	85.17159999999933	31.593819439461903
213	85.17159999999933	31.593819439461903
214	85.17159999999933	31.593819439461903
215	85.17153333333266	31.594001798583438
216	85.17149999999934	31.59409308320133
217	85.17149999999934	31.59409308320133
218	85.17149999999934	31.59409308320133
219	85.17149999999934	31.59409308320133
220	85.17139999999934	31.594373793023962
221	85.17129999999935	31.594654816545347
222	85.17116666666601	31.595028068335324
223	85.17106666666602	31.595309296300623
224	85.20436666666602	31.556780849746005
225	85.20429999999936	31.556968245434486
226	85.23759999999936	31.514123493655106
227	85.23759999999936	31.514123493655106
228	85.23759999999936	31.514123493655106
229	85.23759999999936	31.514123493655106
230	85.23759999999936	31.514123493655106
231	85.23756666666603	31.514215185302405
232	85.23756666666603	31.514215185302405
233	85.23753333333269	31.51430793436889
234	85.23753333333269	31.51430793436889
235	85.23753333333269	31.51430793436889
236	85.23753333333269	31.51430793436889
237	85.23753333333269	31.51430793436889
238	85.23749999999934	31.514403327420666
239	85.23746666666602	31.514498825919432
240	85.23746666666602	31.514498825919432
241	85.23746666666602	31.514498825919432
242	85.23746666666602	31.514498825919432
243	85.23746666666602	31.514498825919432
244	85.23746666666602	31.514498825919432
245	85.23743333333269	31.51458956439417
246	85.23736666666602	31.514772203929276
247	85.2373333333327	31.51486315305147
248	85.27066666666603	31.47670566554825
249	85.27066666666603	31.47670566554825
250	85.27066666666603	31.47670566554825
251	85.27066666666603	31.47670566554825
252	85.2706333333327	31.476798666089877
253	85.27059999999936	31.476889866058997
254	85.27056666666603	31.47698561932015
255	85.2705333333327	31.477081478152098
256	85.2705333333327	31.477081478152098
257	85.27049999999936	31.477173736164126
258	85.27046666666602	31.477266099767498
259	85.27046666666602	31.477266099767498
260	85.27039999999936	31.47744913171984
261	85.27036666666602	31.47754096493087
262	85.27033333333269	31.477632903733692
263	85.27029999999935	31.477724736338107
264	85.27029999999935	31.477724736338107
265	85.27026666666602	31.47781678042849
266	85.27023333333268	31.477908930108708
267	85.27019999999936	31.47800097359011
268	85.2701333333327	31.478189083589374
269	85.27009999999936	31.478282185076935
270	85.26999999999936	31.478558628586185
271	85.26996666666601	31.47865003456908
272	85.26996666666601	31.47865003456908
273	85.26996666666601	31.47865003456908
274	85.26996666666601	31.47865003456908
275	85.26993333333269	31.478743346299787
276	85.26989999999935	31.478836763609937
277	85.26989999999935	31.478836763609937
278	85.26989999999935	31.478836763609937
279	85.26989999999935	31.478836763609937
280	85.26986666666602	31.478928486352387
281	85.26986666666602	31.478928486352387
282	85.26983333333268	31.479020420573388
283	85.26983333333268	31.479020420573388
284	85.26983333333268	31.479020420573388
285	85.26983333333268	31.479020420573388
286	85.26979999999935	31.479111930929875
287	85.26976666666602	31.47920354687453
288	85.26973333333268	31.479295268407164
289	85.26973333333268	31.479295268407164
290	85.26973333333268	31.479295268407164
291	85.26973333333268	31.479295268407164
292	85.26973333333268	31.479295268407164
293	85.26969999999935	31.479387519084185
294	85.26966666666601	31.479479875344527
295	85.26963333333269	31.479572337187857
296	85.26963333333269	31.479572337187857
297	85.26963333333269	31.479572337187857
298	85.26963333333269	31.479572337187857
299	85.26959999999936	31.479664375169595
300	85.26956666666602	31.47975630695927
301	85.26953333333269	31.479848344333114
302	85.26953333333269	31.479848344333114
303	85.26949999999935	31.4799397460772
304	85.26949999999935	31.4799397460772
305	85.26946666666602	31.48003220639316
306	85.26943333333269	31.480124772289038
307	85.26943333333269	31.480124772289038
308	85.26943333333269	31.480124772289038
309	85.26943333333269	31.480124772289038
310	85.26939999999935	31.48021977326905
311	85.26929999999935	31.480499374109872


==> rock_sim_files/rock_mem1_fwd.tex <==
% $\mathrm{Opt. \ FSC \  on \ POMDP, \ M=10, N=10}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.29143333333332416	2.6306114521576145
4	-0.1523999999999809	6.916945441450216
5	0.21620000000000075	10.752357767485051
6	1.2272666666667098	15.624102849835266
7	5.450399999999713	25.679961315650488
8	10.478866666666955	33.06442005210728
9	16.96876666666603	39.461428692824775
10	23.342999999999943	43.88885884823079
11	29.065599999999627	46.744391713231906
12	34.48930000000072	48.62378974168282
13	40.284066666665886	49.87632036142546
14	44.91430000000084	50.33667892809416
15	48.69190000000012	50.38900578886166
16	52.1854999999988	50.15623390716293
17	55.479499999999256	49.657415187293985
18	58.375000000000135	49.00452620251844
19	60.64990000000085	48.40337378038118
20	63.503766666666635	47.44718624406356
21	65.69439999999892	46.594565297968536
22	67.79916666666556	45.61803440130759
23	69.85650000000041	44.5194056311403
24	71.31266666666733	43.66552377130329
25	72.5648666666666	42.941672366698754
26	73.98383333333238	41.992778132740305
27	75.01199999999892	41.28138655617087
28	76.20220000000026	40.449082253618684
29	77.3647000000004	39.53960862953338
30	78.49759999999989	38.62407428327536
31	79.49933333333259	37.76789191304628
32	80.158999999999	37.16180439196505
33	81.33323333333347	36.04200538555296
34	82.11333333333351	35.27626438398604
35	82.99176666666644	34.260940182841274
36	83.67236666666597	33.52744546982692
37	84.34973333333254	32.67972602795541
38	84.79916666666662	32.124579934564295
39	85.27340000000011	31.567702679162444
40	85.99239999999978	30.585698546433953
41	86.63983333333275	29.730892070463604
42	86.99169999999933	29.19504320559689
43	87.5413666666666	28.419756839193557
44	88.15976666666664	27.456890658124895
45	88.47436666666638	26.966892904675245
46	88.92276666666622	26.170776291101603
47	89.23686666666617	25.677699809670457
48	89.59146666666652	25.045679344926622
49	89.9167666666666	24.435414235876664
50	90.3077999999998	23.641779103104742
51	90.6660999999997	22.911192478568218
52	91.0232333333329	22.17234636987163
53	91.18309999999994	21.822606269416983
54	91.47806666666652	21.146782393441125
55	91.73593333333308	20.55722035673978
56	91.89673333333303	20.166835547392058
57	92.02556666666626	19.867191791465885
58	92.2518666666665	19.27420235744028
59	92.44639999999981	18.748972070667474
60	92.71046666666642	17.99591760508164
61	92.90273333333303	17.43213505365555
62	92.99786666666625	17.156804154102275
63	93.12636666666648	16.784250200675892
64	93.18953333333307	16.601002694081163
65	93.2528666666664	16.421841911984835
66	93.41366666666646	15.931863248081118
67	93.47586666666635	15.74537109488233
68	93.53806666666654	15.54778154364431
69	93.59776666666644	15.361566489529096
70	93.62946666666645	15.245666872335304
71	93.69456666666643	15.01624077942133
72	93.72499999999967	14.833706268720139
73	93.82089999999982	14.461611477402242
74	93.95026666666644	13.965694872158023
75	93.9489333333331	13.975838634188946
76	94.01436666666645	13.728427814777502
77	94.07983333333303	13.465522516370804
78	94.14269999999986	13.19800439624616
79	94.17359999999978	13.086430492689747
80	94.20583333333315	12.941871424651932
81	94.23683333333314	12.82656618008978
82	94.26783333333304	12.699883279209908
83	94.3001666666665	12.559663609039147
84	94.33126666666645	12.406799039057363
85	94.3637333333331	12.228640891866185
86	94.39486666666645	12.092682373329001
87	94.39399999999974	12.100493543653478
88	94.49059999999982	11.616125500355112
89	94.5231999999998	11.434457067419801
90	94.58916666666646	11.10190100713485
91	94.62186666666646	10.934236226133455
92	94.65459999999976	10.763185967608916
93	94.68733333333317	10.576376169978483
94	94.68539999999982	10.597471090154805
95	94.71683333333314	10.44631130936761
96	94.74829999999982	10.253228943931116
97	94.7464333333331	10.273859414985631
98	94.74459999999983	10.294633108566828
99	94.74276666666647	10.314360911477886
100	94.74223333333315	10.320146947220346
101	94.74169999999982	10.325934878256774
102	94.77319999999978	10.141453960190661
103	94.80609999999984	9.937471817486276
104	94.80566666666647	9.942404532550917
105	94.80519999999981	9.947691505738076
106	94.80473333333316	9.95298033734397
107	94.83763333333313	9.716189602868427
108	94.8692666666665	9.544560167737258
109	94.8675999999998	9.564668851559901
110	94.8672666666665	9.568662142408174
111	94.86689999999982	9.5730257001988
112	94.86386666666644	9.610208168863403
113	94.8968666666665	9.389747432646363
114	94.9298999999998	9.192175440195552
115	94.92959999999982	9.195965628469937
116	94.92929999999983	9.19975750640559
117	94.9289999999998	9.203551071914202
118	94.92869999999984	9.20734632290974
119	94.92839999999981	9.211143257308855
120	94.9267666666665	9.231267169005271
121	94.9264666666665	9.235075140402943
122	94.92483333333314	9.255196376750883
123	94.92453333333317	9.259015324656406
124	94.92423333333315	9.262835927091762
125	94.92263333333315	9.282549455773946
126	94.92099999999981	9.303812426455456
127	94.91939999999981	9.325217261454704
128	94.9524666666665	9.091463427242559
129	94.95219999999982	9.094991029498987
130	94.98529999999981	8.853856442816333
131	94.9850666666665	8.857049376751961
132	94.98349999999982	8.878010911797718
133	94.98326666666651	8.881215382042159
134	94.98303333333317	8.88442131667686
135	94.9814666666665	8.906583511587828
136	94.98123333333317	8.909800473573418
137	94.98099999999982	8.913018886250999
138	94.97943333333318	8.93577418837091
139	94.9778666666665	8.956717597175643
140	94.97763333333317	8.95995664417836
141	94.97743333333315	8.962702387053152
142	94.97589999999983	8.983793696985696
143	94.97566666666651	8.98704481771155
144	95.00879999999984	8.675852843380904
145	95.00863333333317	8.678231509485238
146	95.04179999999984	8.401881104451112
147	95.04163333333315	8.404357798124071
148	95.0414666666665	8.406835741360869
149	95.07466666666652	8.102941331530321
150	95.07453333333316	8.10499834148997
151	95.07306666666649	8.127453143239654
152	95.07293333333315	8.129523606105257
153	95.07283333333318	8.131093733659384
154	95.07269999999984	8.13316613482517
155	95.07256666666649	8.135239644834579
156	95.10579999999983	7.834226596161232
157	95.10569999999981	7.835861418929417
158	95.1042666666665	7.859396189416964
159	95.10283333333318	7.882895532240799
160	95.10273333333316	7.884557852466348
161	95.1026666666665	7.885666715982573
162	95.10256666666649	7.887330563138715
163	95.1024666666665	7.888995325698266
164	95.13573333333316	7.5387335228729855
165	95.13566666666651	7.539897074157473
166	95.13559999999983	7.541061329370929
167	95.13419999999984	7.565848951703997
168	95.13413333333318	7.567028583415176
169	95.13273333333316	7.591785595555821
170	95.13269999999984	7.592383071868811
171	95.13263333333316	7.593578321991728
172	95.13256666666649	7.5947742612199525
173	95.1658666666665	7.206923170273303
174	95.16583333333318	7.2075545533064895
175	95.16579999999983	7.208186343318287
176	95.16576666666649	7.208818540201656
177	95.16573333333316	7.209451143849709
178	95.16569999999983	7.210084154155225
179	95.16566666666651	7.210717571011172
180	95.16563333333316	7.211351394310372
181	95.16559999999983	7.21198562394575
182	95.16423333333316	7.238337567809029
183	95.16419999999984	7.2389887663954635
184	95.16416666666652	7.239640366681861
185	95.16413333333317	7.240292368559595
186	95.16409999999982	7.240944771920276
187	95.1640666666665	7.241597576655458
188	95.16403333333317	7.242250782656527
189	95.16399999999985	7.2429043898149015
190	95.1639666666665	7.243558398022043
191	95.16393333333315	7.244212807169317
192	95.16389999999983	7.244867617148015
193	95.16386666666651	7.245522827849573
194	95.16383333333317	7.246178439165157
195	95.16379999999984	7.2468344509861655
196	95.16376666666649	7.2474908632037645
197	95.16239999999983	7.274747159867478
198	95.1623666666665	7.275420290188672
199	95.16233333333318	7.2760938162053765
200	95.16229999999983	7.276767737807786
201	95.16226666666648	7.277442054885917
202	95.16223333333316	7.2781167673299185
203	95.16219999999984	7.27879187502979
204	95.16216666666651	7.279467377875631
205	95.16213333333317	7.280143275757396
206	95.16209999999982	7.280819568565068
207	95.16206666666649	7.281496256188615
208	95.16203333333317	7.2821733385179845
209	95.16199999999985	7.282850815443069
210	95.1619666666665	7.2835286868537805
211	95.16193333333315	7.28420695264
212	95.16189999999983	7.284885612691533
213	95.1618666666665	7.2855646668981935
214	95.16183333333318	7.286244115149819
215	95.16179999999983	7.2869239573361755
216	95.1617666666665	7.287604193347018
217	95.16173333333316	7.288284823072037
218	95.16169999999984	7.288965846400981
219	95.1616666666665	7.28964726322352
220	95.16163333333317	7.290329073429339
221	95.16159999999982	7.291011276908019
222	95.1615666666665	7.291693873549212
223	95.16153333333317	7.292376863242593
224	95.16149999999985	7.2930602458775535
225	95.1614666666665	7.293744021343844
226	95.16143333333315	7.294428189530787
227	95.16139999999983	7.295112750328159
228	95.16136666666651	7.2957977036251895
229	95.16133333333318	7.296483049311414
230	95.16129999999983	7.297168787276345
231	95.16126666666649	7.29785491740935
232	95.16123333333316	7.298541439599788
233	95.16119999999984	7.299228353737142
234	95.16116666666652	7.299915659710663
235	95.16113333333317	7.300603357409746
236	95.16109999999982	7.30129144672367
237	95.1610666666665	7.301979927541725
238	95.16103333333317	7.302668799753221
239	95.16099999999985	7.303358063247345
240	95.1609666666665	7.3040477179133685
241	95.16093333333315	7.3047377636405155
242	95.16089999999983	7.305428200317908
243	95.16086666666651	7.306119027834761
244	95.15949999999984	7.334778098211271
245	95.1594666666665	7.335485240633753
246	95.15943333333315	7.3361927691109425
247	95.15939999999983	7.336900683531174
248	95.1593666666665	7.337608983782711
249	95.1593666666665	7.337608983782711
250	95.15933333333318	7.338317669753918
251	95.15929999999983	7.339026741332942
252	95.15926666666648	7.3397361984080955
253	95.19259999999983	6.840077867977835
254	95.19259999999983	6.840077867977835
255	95.19259999999983	6.840077867977835
256	95.19259999999983	6.840077867977835
257	95.19259999999983	6.840077867977835
258	95.19259999999983	6.840077867977835
259	95.19259999999983	6.840077867977835
260	95.19259999999983	6.840077867977835
261	95.19259999999983	6.840077867977835
262	95.19259999999983	6.840077867977835
263	95.19259999999983	6.840077867977835
264	95.19259999999983	6.840077867977835
265	95.19259999999983	6.840077867977835
266	95.19259999999983	6.840077867977835
267	95.19259999999983	6.840077867977835
268	95.19259999999983	6.840077867977835
269	95.19259999999983	6.840077867977835
270	95.19259999999983	6.840077867977835
271	95.19259999999983	6.840077867977835
272	95.19259999999983	6.840077867977835
273	95.19259999999983	6.840077867977835
274	95.19259999999983	6.840077867977835
275	95.19259999999983	6.840077867977835
276	95.19259999999983	6.840077867977835
277	95.19259999999983	6.840077867977835
278	95.19259999999983	6.840077867977835
279	95.19259999999983	6.840077867977835
280	95.19259999999983	6.840077867977835
281	95.19259999999983	6.840077867977835
282	95.19259999999983	6.840077867977835
283	95.19259999999983	6.840077867977835
284	95.19259999999983	6.840077867977835
285	95.19259999999983	6.840077867977835
286	95.19259999999983	6.840077867977835
287	95.19259999999983	6.840077867977835
288	95.19259999999983	6.840077867977835
289	95.19259999999983	6.840077867977835
290	95.19259999999983	6.840077867977835
291	95.19259999999983	6.840077867977835
292	95.19259999999983	6.840077867977835
293	95.19259999999983	6.840077867977835
294	95.19259999999983	6.840077867977835
295	95.19259999999983	6.840077867977835
296	95.19259999999983	6.840077867977835
297	95.19259999999983	6.840077867977835
298	95.19259999999983	6.840077867977835
299	95.19259999999983	6.840077867977835


==> rock_sim_files/rock_mem1_trajsize10mdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.09999999999999991	9.71445146547012e-17
2	-0.19999999999999982	1.942890293094024e-16
3	-0.2683666666666539	2.612105663806302
4	1.1785999999999395	14.853285002763869
5	7.364066666666703	28.686770042341962
6	10.401933333333414	32.774963863629516
7	14.639299999999777	36.97648449366193
8	20.32613333333293	40.87336203097959
9	23.4516999999997	42.52377041659574
10	25.248799999999775	43.42531003796408
11	26.44649999999983	43.97603538007947
12	27.17796666666654	44.31057832164793
13	27.909799999999887	44.6408928819006
14	28.47499999999991	44.90701587725491
15	28.93976666666661	45.10662407317667
16	29.437799999999935	45.32234001564067
17	29.835599999999992	45.482702418685214
18	30.664366666666684	45.81698942821952
19	31.296133333333362	46.05068524697058
20	31.761366666666706	46.21764003926282
21	32.426666666666705	46.43774458586746
22	32.89233333333339	46.58251168148343
23	33.19100000000007	46.67979276232162
24	33.656466666666745	46.828454720560245
25	33.9217000000001	46.91236346398029
26	34.520633333333436	47.103659704941116
27	34.68603333333343	47.15108660747486
28	35.18496666666679	47.29631455690304
29	35.683900000000136	47.427328803725175
30	35.916133333333455	47.49211492148516
31	36.18156666666677	47.56210876540582
32	36.58043333333344	47.66623116853511
33	37.01260000000012	47.76129682675445
34	37.37830000000013	47.85526936270107
35	37.610566666666784	47.90252705594554
36	38.009766666666806	47.99111592727967
37	38.342400000000154	48.06626268919485
38	38.57516666666681	48.11678023280676
39	38.80760000000016	48.157872553785765
40	38.97340000000016	48.192054176735134
41	39.20586666666682	48.23389837291743
42	39.571900000000156	48.30717234935211
43	39.904666666666834	48.36531813419806
44	40.0041333333335	48.382542611795394
45	40.23690000000017	48.424935192419284
46	40.469800000000156	48.4659941398095
47	40.53576666666684	48.4758052098719
48	40.76846666666683	48.512939912793115
49	40.93440000000017	48.539973870065296
50	41.26723333333351	48.59736868403722
51	41.40006666666684	48.61993589734807
52	41.566366666666845	48.644516430928796
53	41.73243333333352	48.66590406104552
54	41.865266666666855	48.68428918650858
55	41.93120000000019	48.69520770288134
56	42.13063333333352	48.72309491673908
57	42.36333333333353	48.75455187865961
58	42.42933333333354	48.761854895901095
59	42.59533333333353	48.78565169755878
60	42.861566666666874	48.81621608521987
61	43.09456666666687	48.84153744999119
62	43.26103333333354	48.85994519984908
63	43.360900000000214	48.87259642366072
64	43.427400000000205	48.88094621192749
65	43.4605000000002	48.882429935680065
66	43.49350000000021	48.88405521657039
67	43.559766666666874	48.88957521406996
68	43.65946666666688	48.89856109384887
69	43.792466666666876	48.908473055108054
70	43.95896666666686	48.92472046861581
71	43.99210000000021	48.92866597667193
72	44.0586000000002	48.93614301011762
73	44.09170000000021	48.93991705254534
74	44.191533333333545	48.95068166003676
75	44.25780000000022	48.955376339002584
76	44.32400000000021	48.96277651440942
77	44.45703333333357	48.97411905485257
78	44.49006666666691	48.97776204219877
79	44.62316666666692	48.98246155484828
80	44.68960000000026	48.988874163834936
81	44.75600000000027	48.98977788613979
82	44.88916666666693	48.99408895610665
83	44.95566666666693	49.00033565758052
84	45.02216666666691	49.00649411359209
85	45.02186666666691	49.006778121489326
86	45.08820000000024	49.01300664884748
87	45.15446666666692	49.018934505442786
88	45.22073333333359	49.022327533436616
89	45.42050000000025	49.0332092540347
90	45.55360000000028	49.04135119508884
91	45.620066666666965	49.04400409151876
92	45.653200000000304	49.046619826718675
93	45.71956666666698	49.05181920322175
94	45.78593333333364	49.05693103047626
95	45.85236666666697	49.05631275448174
96	45.985600000000304	49.06600662345869
97	46.05213333333365	49.067876274764174
98	46.08533333333365	49.070132513464536
99	46.08516666666698	49.070293491129235
100	46.151700000000325	49.07216125710554
101	46.21826666666699	49.076487917625755
102	46.218166666666995	49.076583146196704
103	46.217966666666996	49.07677346633144
104	46.28450000000032	49.08104178889575
105	46.317666666666995	49.083239989724824
106	46.384166666667	49.08754308347714
107	46.417366666667	49.089642170205984
108	46.48393333333365	49.091030088964
109	46.55050000000032	49.09477195265647
110	46.55040000000032	49.094870945684065
111	46.61700000000033	49.09577182405819
112	46.650266666666994	49.097580862967014
113	46.65016666666698	49.09767971407157
114	46.65006666666699	49.09777876844917
115	46.683300000000315	49.0969472008529
116	46.71653333333366	49.09874356826492
117	46.783166666666986	49.10224088544467
118	46.78313333333365	49.102275801115816
119	46.78306666666699	49.102342916900895
120	46.81636666666699	49.10128914260355
121	46.81623333333365	49.10142041202976
122	46.849400000000315	49.10319351094465
123	46.84923333333365	49.103360028402506
124	46.94913333333365	49.108421876994385
125	46.98243333333365	49.10732614806275
126	46.98236666666699	49.107393527507824
127	47.01563333333365	49.10630481176105
128	47.01550000000031	49.10643681246554
129	47.01533333333364	49.106601235362014
130	47.11526666666698	49.11115135006426
131	47.14850000000031	49.109869046353516
132	47.148400000000315	49.10996610437982
133	47.2150000000003	49.11304214089529
134	47.248266666666964	49.11458137521097
135	47.2482000000003	49.11464910553672
136	47.28143333333363	49.11606789309276
137	47.314666666666966	49.11481458333705
138	47.31453333333363	49.11494995194618
139	47.381100000000295	49.11226764047848
140	47.4477000000003	49.11502785682481
141	47.44766666666697	49.11506043182915
142	47.44763333333364	49.11509307465719
143	47.480966666666966	49.116338908068265
144	47.480966666666966	49.116338908068265
145	47.480966666666966	49.116338908068265
146	47.480966666666966	49.116338908068265
147	47.48093333333364	49.116371369047435
148	47.480900000000304	49.11640389784976
149	47.48086666666697	49.11643649447284
150	47.514166666666966	49.117762869511495
151	47.51413333333363	49.11779820237162
152	47.514100000000305	49.117833603048176
153	47.54743333333364	49.11631969191978
154	47.54743333333364	49.11631969191978
155	47.54743333333364	49.11631969191978
156	47.54743333333364	49.11631969191978
157	47.54743333333364	49.11631969191978
158	47.54743333333364	49.11631969191978
159	47.54743333333364	49.11631969191978
160	47.54743333333364	49.11631969191978
161	47.54743333333364	49.11631969191978
162	47.54743333333364	49.11631969191978
163	47.5474000000003	49.11635233375225
164	47.54736666666697	49.11638504340684
165	47.54733333333363	49.11641782088285
166	47.580666666666964	49.117528095601806
167	47.580666666666964	49.117528095601806
168	47.58063333333363	49.11756055559191
169	47.580600000000295	49.117593083402184
170	47.58056666666696	49.11762567903271
171	47.613900000000285	49.1189169613572
172	47.613900000000285	49.1189169613572
173	47.61386666666696	49.11894964656989
174	47.61380000000029	49.119017731356664
175	47.61373333333362	49.11908595168367
176	47.64703333333362	49.12018659572537
177	47.68036666666695	49.118582544683214
178	47.68036666666695	49.118582544683214
179	47.68036666666695	49.118582544683214
180	47.68036666666695	49.118582544683214
181	47.68036666666695	49.118582544683214
182	47.68036666666695	49.118582544683214
183	47.68036666666695	49.118582544683214
184	47.68036666666695	49.118582544683214
185	47.68036666666695	49.118582544683214
186	47.68036666666695	49.118582544683214
187	47.68036666666695	49.118582544683214
188	47.68036666666695	49.118582544683214
189	47.680333333333614	49.11861513949939
190	47.68030000000028	49.11864780213314
191	47.68026666666695	49.118680532585394
192	47.713600000000284	49.11983626845657
193	47.713600000000284	49.11983626845657
194	47.713600000000284	49.11983626845657
195	47.713600000000284	49.11983626845657
196	47.713600000000284	49.11983626845657
197	47.713600000000284	49.11983626845657
198	47.713600000000284	49.11983626845657
199	47.713600000000284	49.11983626845657
200	47.713600000000284	49.11983626845657
201	47.713600000000284	49.11983626845657
202	47.713600000000284	49.11983626845657
203	47.713600000000284	49.11983626845657
204	47.713600000000284	49.11983626845657
205	47.713600000000284	49.11983626845657
206	47.713600000000284	49.11983626845657
207	47.713600000000284	49.11983626845657
208	47.713600000000284	49.11983626845657
209	47.713600000000284	49.11983626845657
210	47.713600000000284	49.11983626845657
211	47.713600000000284	49.11983626845657
212	47.713600000000284	49.11983626845657
213	47.713600000000284	49.11983626845657
214	47.713600000000284	49.11983626845657
215	47.713600000000284	49.11983626845657
216	47.713600000000284	49.11983626845657
217	47.713600000000284	49.11983626845657
218	47.713600000000284	49.11983626845657
219	47.713600000000284	49.11983626845657
220	47.713600000000284	49.11983626845657
221	47.713600000000284	49.11983626845657
222	47.713600000000284	49.11983626845657
223	47.713600000000284	49.11983626845657
224	47.713600000000284	49.11983626845657
225	47.713600000000284	49.11983626845657
226	47.713600000000284	49.11983626845657
227	47.713600000000284	49.11983626845657
228	47.713600000000284	49.11983626845657
229	47.713600000000284	49.11983626845657
230	47.713600000000284	49.11983626845657
231	47.713600000000284	49.11983626845657
232	47.713600000000284	49.11983626845657
233	47.713600000000284	49.11983626845657
234	47.713600000000284	49.11983626845657
235	47.713600000000284	49.11983626845657
236	47.713600000000284	49.11983626845657
237	47.713600000000284	49.11983626845657
238	47.713600000000284	49.11983626845657
239	47.713600000000284	49.11983626845657
240	47.713600000000284	49.11983626845657
241	47.713600000000284	49.11983626845657
242	47.713600000000284	49.11983626845657
243	47.713600000000284	49.11983626845657
244	47.713600000000284	49.11983626845657
245	47.713600000000284	49.11983626845657
246	47.713600000000284	49.11983626845657
247	47.713600000000284	49.11983626845657
248	47.713600000000284	49.11983626845657
249	47.713600000000284	49.11983626845657
250	47.713600000000284	49.11983626845657
251	47.713600000000284	49.11983626845657
252	47.713600000000284	49.11983626845657
253	47.713600000000284	49.11983626845657
254	47.713600000000284	49.11983626845657
255	47.713600000000284	49.11983626845657
256	47.713600000000284	49.11983626845657
257	47.713600000000284	49.11983626845657
258	47.713600000000284	49.11983626845657
259	47.713600000000284	49.11983626845657
260	47.713600000000284	49.11983626845657
261	47.713600000000284	49.11983626845657
262	47.713600000000284	49.11983626845657
263	47.713600000000284	49.11983626845657
264	47.713600000000284	49.11983626845657
265	47.713600000000284	49.11983626845657
266	47.713600000000284	49.11983626845657
267	47.713600000000284	49.11983626845657
268	47.713600000000284	49.11983626845657
269	47.713600000000284	49.11983626845657
270	47.713600000000284	49.11983626845657
271	47.713600000000284	49.11983626845657
272	47.713600000000284	49.11983626845657
273	47.713600000000284	49.11983626845657
274	47.713600000000284	49.11983626845657
275	47.713600000000284	49.11983626845657
276	47.713600000000284	49.11983626845657
277	47.713600000000284	49.11983626845657
278	47.713600000000284	49.11983626845657
279	47.713600000000284	49.11983626845657
280	47.713600000000284	49.11983626845657
281	47.713600000000284	49.11983626845657
282	47.713600000000284	49.11983626845657
283	47.713600000000284	49.11983626845657
284	47.713600000000284	49.11983626845657
285	47.713600000000284	49.11983626845657
286	47.713600000000284	49.11983626845657
287	47.713600000000284	49.11983626845657
288	47.713600000000284	49.11983626845657
289	47.713600000000284	49.11983626845657
290	47.713600000000284	49.11983626845657
291	47.713600000000284	49.11983626845657
292	47.713600000000284	49.11983626845657
293	47.713600000000284	49.11983626845657
294	47.713600000000284	49.11983626845657
295	47.713600000000284	49.11983626845657
296	47.713600000000284	49.11983626845657
297	47.713600000000284	49.11983626845657
298	47.713600000000284	49.11983626845657
299	47.713600000000284	49.11983626845657
300	47.713600000000284	49.11983626845657
301	47.713600000000284	49.11983626845657
302	47.713600000000284	49.11983626845657
303	47.713600000000284	49.11983626845657
304	47.713600000000284	49.11983626845657
305	47.713600000000284	49.11983626845657
306	47.713600000000284	49.11983626845657
307	47.713600000000284	49.11983626845657
308	47.713600000000284	49.11983626845657
309	47.713600000000284	49.11983626845657
310	47.713600000000284	49.11983626845657
311	47.713600000000284	49.11983626845657


==> rock_sim_files/rock_mem1_trajsize10pomdp_irl.tex <==
% $\mathrm{Learned \ policy, \ |n|=1}$
x	y	err
0	0.0	0.0
1	-0.10133333333333362	0.07301750170716209
2	-0.20133333333333353	0.07301750170716209
3	-0.2615333333333272	2.606907551529619
4	-0.1963999999999849	9.650301914448038
5	0.6717333333333316	15.586613519156556
6	2.0855333333332835	19.990336766770664
7	5.014866666666639	25.807285773250584
8	10.529866666666784	32.95807965657088
9	16.06749999999971	37.932838900922505
10	19.881233333333043	40.597685457164864
11	22.734433333333055	42.29082348467829
12	25.259799999999853	43.58021742289372
13	27.086333333333144	44.42995828517322
14	28.247233333333217	44.9216499290217
15	29.274899999999857	45.35041396345425
16	30.83716666666656	45.98941025176961
17	31.899433333333246	46.37806187209881
18	33.12923333333328	46.79963185836933
19	33.99279999999993	47.07028951288338
20	35.02333333333328	47.371568782222965
21	35.954099999999904	47.6216679309255
22	36.38513333333326	47.73060205272445
23	37.24953333333326	47.92959927277613
24	37.813899999999954	48.06354526516599
25	38.244433333333276	48.158484081335
26	39.108766666666625	48.33633270959059
27	39.77323333333327	48.462561772418724
28	40.50469999999995	48.587510753724885
29	40.8693666666666	48.64570407479133
30	41.23413333333328	48.703402908991315
31	41.83219999999992	48.79154424515226
32	42.36359999999995	48.860345220229355
33	42.72813333333326	48.90447888672589
34	43.126066666666624	48.951652480063274
35	43.791033333333274	49.0099839107523
36	44.45616666666667	49.06709870478975
37	44.654399999999995	49.08496016065748
38	45.15256666666666	49.12514719311848
39	45.4840666666666	49.14508269191915
40	45.848966666666634	49.17395596857044
41	46.44736666666658	49.20189271155006
42	46.9127333333333	49.213652081465376
43	47.37819999999994	49.22428666921789
44	47.67683333333329	49.22757370931029
45	47.87529999999997	49.23529452107191
46	48.27386666666667	49.24019858864172
47	48.605533333333334	49.24094220648315
48	49.170666666666655	49.232432327571644
49	49.43576666666665	49.230923250319826
50	49.667266666666634	49.22630186389746
51	50.36576666666665	49.199944831393964
52	50.63099999999999	49.18386014741056
53	50.89626666666661	49.17158677592398
54	51.42843333333329	49.138257683929425
55	51.7271333333333	49.11964451332649
56	52.02593333333329	49.096996386020415
57	52.191399999999916	49.08551068669171
58	52.55723333333325	49.05727517584792
59	52.856333333333254	49.03131189918849
60	53.222199999999944	48.994640528259296
61	53.32129999999994	48.98467879153611
62	53.553699999999964	48.9632220444763
63	53.88619999999995	48.9253419973737
64	54.08523333333326	48.90428098451335
65	54.3508999999999	48.875727846481446
66	54.44979999999988	48.863205243072905
67	54.54863333333319	48.85062078894751
68	55.04793333333316	48.78807411375142
69	55.21379999999985	48.76852471516177
70	55.413133333333185	48.741072285245735
71	55.57906666666651	48.719912990434835
72	55.77843333333319	48.69158734537426
73	55.97783333333319	48.66170121672257
74	56.11039999999984	48.64070529751803
75	56.309699999999864	48.60969439569984
76	56.47576666666653	48.58547693922802
77	56.641799999999854	48.55515536747874
78	56.941433333333165	48.49739951735089
79	57.00769999999984	48.484304718571856
80	57.10739999999987	48.46556714383254
81	57.17373333333321	48.45504346018973
82	57.27336666666653	48.43851450377273
83	57.306299999999865	48.4335022855394
84	57.40573333333319	48.41735694764397
85	57.57183333333317	48.384207995022024
86	57.70459999999984	48.35641507432086
87	57.83739999999983	48.32791982460394
88	57.97023333333317	48.29899699385324
89	58.13663333333318	48.26026835122478
90	58.20293333333318	48.24555853197502
91	58.269133333333166	48.233642276412
92	58.33529999999984	48.221952786844476
93	58.53489999999986	48.18440756084915
94	58.634466666666526	48.162835382158825
95	58.73416666666652	48.14386069520087
96	58.800499999999865	48.13075049366399
97	58.90009999999988	48.10835218535361
98	58.96633333333322	48.09263214418181
99	59.03253333333321	48.079911275385
100	59.13209999999987	48.056706777063276
101	59.298399999999866	48.01957376015209
102	59.43149999999987	47.988854446458426
103	59.53126666666654	47.967787202061
104	59.56436666666653	47.96102814020496
105	59.664199999999866	47.939310435451944
106	59.697433333333194	47.93187029606587
107	59.73066666666653	47.9246144086965
108	59.730533333333206	47.92478281344149
109	59.797066666666545	47.90997541983197
110	59.83029999999987	47.90285605865993
111	59.86336666666654	47.89557420053439
112	59.896433333333206	47.88861977490639
113	59.92956666666653	47.88120935341523
114	60.029399999999875	47.859047096378056
115	60.06246666666654	47.84897983498595
116	60.09559999999986	47.84179679568928
117	60.1287333333332	47.834241163928674
118	60.22859999999988	47.80866513551685
119	60.261766666666524	47.80096646385751
120	60.294933333333205	47.79345562935948
121	60.36146666666654	47.77810316294371
122	60.3946333333332	47.770664651006115
123	60.4277333333332	47.76042326929515
124	60.52759999999986	47.73432459883199
125	60.560799999999865	47.723712450171725
126	60.56063333333319	47.72393194473311
127	60.59383333333319	47.71623167545337
128	60.62689999999987	47.70833183407294
129	60.6933333333332	47.68968556080969
130	60.72643333333319	47.68194911367289
131	60.82619999999986	47.65230291979586
132	60.89266666666653	47.63610968815786
133	60.92579999999986	47.62782682102285
134	61.02569999999986	47.60056452231808
135	61.05889999999986	47.59251384538653
136	61.092133333333194	47.58404499530863
137	61.0920333333332	47.58417481893383
138	61.158666666666534	47.56764774040859
139	61.19199999999985	47.55918512057699
140	61.19199999999985	47.55918512057699
141	61.19196666666652	47.55922839434558
142	61.191933333333196	47.55927173813959
143	61.19189999999986	47.55931515195865
144	61.19179999999985	47.55944553321318
145	61.19169999999985	47.55957584381216
146	61.22499999999985	47.55106190542291
147	61.25829999999985	47.54273324540084
148	61.25819999999984	47.54286612549402
149	61.258066666666515	47.543042550186655
150	61.2578666666665	47.54330893808532
151	61.35773333333317	47.515135415243385
152	61.39093333333317	47.5067733885973
153	61.42416666666652	47.49560350852363
154	61.5241333333332	47.46726911864884
155	61.52409999999986	47.467312569002324
156	61.52406666666653	47.46735608951568
157	61.55733333333319	47.45898713158062
158	61.55726666666653	47.459074515441074
159	61.55719999999986	47.459162039519136
160	61.5571333333332	47.459249703813455
161	61.590366666666526	47.45061907427746
162	61.590266666666516	47.45075024270472
163	61.6235333333332	47.44219169525036
164	61.62346666666653	47.44227948411493
165	61.65673333333319	47.43355543630353
166	61.69003333333319	47.42469220422577
167	61.689999999999856	47.42473595076693
168	61.72333333333319	47.41608519854374
169	61.723266666666525	47.416173246360565
170	61.72319999999986	47.41626361379942
171	61.72309999999986	47.416397758475824
172	61.756333333333195	47.40771617808866
173	61.75623333333319	47.407850979335485
174	61.78949999999986	47.399241763450206
175	61.82279999999986	47.38753619704944
176	61.822766666666524	47.38758070435982
177	61.822699999999855	47.38766950775944
178	61.85596666666652	47.37830323821474
179	61.85586666666652	47.378435308153406
180	61.8891333333332	47.36974775017863
181	61.922433333333196	47.36042771568057
182	61.95576666666653	47.35160159289378
183	61.95576666666653	47.35160159289378
184	61.95573333333319	47.35164615718826
185	61.95573333333319	47.35164615718826
186	61.95573333333319	47.35164615718826
187	61.95573333333319	47.35164615718826
188	61.95573333333319	47.35164615718826
189	61.95573333333319	47.35164615718826
190	61.95573333333319	47.35164615718826
191	61.95573333333319	47.35164615718826
192	61.95569999999986	47.3516929036688
193	61.955666666666524	47.35173972047422
194	61.95563333333319	47.351786607605675
195	61.95556666666653	47.35187770665023
196	61.95549999999985	47.351968946215166
197	61.95539999999985	47.35210432677022
198	62.02203333333319	47.33104123650991
199	62.02196666666653	47.33112965197668
200	62.055266666666526	47.32213138615897
201	62.08859999999986	47.31299317706838
202	62.08859999999986	47.31299317706838
203	62.08859999999986	47.31299317706838
204	62.08859999999986	47.31299317706838
205	62.08859999999986	47.31299317706838
206	62.08856666666652	47.31304005534729
207	62.08853333333319	47.31308700400841
208	62.08853333333319	47.31308700400841
209	62.08853333333319	47.31308700400841
210	62.08853333333319	47.31308700400841
211	62.08853333333319	47.31308700400841
212	62.08853333333319	47.31308700400841
213	62.08853333333319	47.31308700400841
214	62.08853333333319	47.31308700400841
215	62.08853333333319	47.31308700400841
216	62.08853333333319	47.31308700400841
217	62.08853333333319	47.31308700400841
218	62.08853333333319	47.31308700400841
219	62.08853333333319	47.31308700400841
220	62.08853333333319	47.31308700400841
221	62.08853333333319	47.31308700400841
222	62.08853333333319	47.31308700400841
223	62.08853333333319	47.31308700400841
224	62.08853333333319	47.31308700400841
225	62.08853333333319	47.31308700400841
226	62.08853333333319	47.31308700400841
227	62.08853333333319	47.31308700400841
228	62.08853333333319	47.31308700400841
229	62.08853333333319	47.31308700400841
230	62.08853333333319	47.31308700400841
231	62.08853333333319	47.31308700400841
232	62.08853333333319	47.31308700400841
233	62.08853333333319	47.31308700400841
234	62.08853333333319	47.31308700400841
235	62.08853333333319	47.31308700400841
236	62.08853333333319	47.31308700400841
237	62.08853333333319	47.31308700400841
238	62.08853333333319	47.31308700400841
239	62.08853333333319	47.31308700400841
240	62.08853333333319	47.31308700400841
241	62.08853333333319	47.31308700400841
242	62.08853333333319	47.31308700400841
243	62.08853333333319	47.31308700400841
244	62.08853333333319	47.31308700400841
245	62.08853333333319	47.31308700400841
246	62.08853333333319	47.31308700400841
247	62.08853333333319	47.31308700400841
248	62.08853333333319	47.31308700400841
249	62.08853333333319	47.31308700400841
250	62.08853333333319	47.31308700400841
251	62.08853333333319	47.31308700400841
252	62.08853333333319	47.31308700400841
253	62.08853333333319	47.31308700400841
254	62.08853333333319	47.31308700400841
255	62.08853333333319	47.31308700400841
256	62.08853333333319	47.31308700400841
257	62.08853333333319	47.31308700400841
258	62.08853333333319	47.31308700400841
259	62.08853333333319	47.31308700400841
260	62.08853333333319	47.31308700400841
261	62.08853333333319	47.31308700400841
262	62.08853333333319	47.31308700400841
263	62.08853333333319	47.31308700400841
264	62.08853333333319	47.31308700400841
265	62.08853333333319	47.31308700400841
266	62.08853333333319	47.31308700400841
267	62.08853333333319	47.31308700400841
268	62.08853333333319	47.31308700400841
269	62.08853333333319	47.31308700400841
270	62.08853333333319	47.31308700400841
271	62.08853333333319	47.31308700400841
272	62.08853333333319	47.31308700400841
273	62.08853333333319	47.31308700400841
274	62.08853333333319	47.31308700400841
275	62.08853333333319	47.31308700400841
276	62.08853333333319	47.31308700400841
277	62.08853333333319	47.31308700400841
278	62.08853333333319	47.31308700400841
279	62.08853333333319	47.31308700400841
280	62.08853333333319	47.31308700400841
281	62.08853333333319	47.31308700400841
282	62.08853333333319	47.31308700400841
283	62.08853333333319	47.31308700400841
284	62.08853333333319	47.31308700400841
285	62.08853333333319	47.31308700400841
286	62.08853333333319	47.31308700400841
287	62.08853333333319	47.31308700400841
288	62.08853333333319	47.31308700400841
289	62.08853333333319	47.31308700400841
290	62.08853333333319	47.31308700400841
291	62.08853333333319	47.31308700400841
292	62.08853333333319	47.31308700400841
293	62.088499999999854	47.31313176856934
294	62.08846666666652	47.31317660351627
295	62.08846666666652	47.31317660351627
296	62.08846666666652	47.31317660351627
297	62.08846666666652	47.31317660351627
298	62.08846666666652	47.31317660351627
299	62.08846666666652	47.31317660351627
300	62.08846666666652	47.31317660351627
301	62.08846666666652	47.31317660351627
302	62.08846666666652	47.31317660351627
303	62.08846666666652	47.31317660351627
304	62.08846666666652	47.31317660351627
305	62.08846666666652	47.31317660351627
306	62.08846666666652	47.31317660351627
307	62.08846666666652	47.31317660351627
308	62.08846666666652	47.31317660351627
309	62.08846666666652	47.31317660351627
310	62.08846666666652	47.31317660351627


==> sup_mat.tex <==
\inpu
